SkyStore: Cost-Optimized Object Storage Across Regions and Clouds

Modern applications span multiple clouds to reduce costs, avoid vendor lock-in, and leverage low-availability resources in another cloud. However, standard object stores operate within a single cloud, forcing users to manually manage data placement across clouds, i.e., navigate their diverse APIs and handle heterogeneous costs for network and storage. This is often a complex choice: users must either pay to store objects in a remote cloud, or pay to transfer them over the network based on application access patterns and cloud provider cost offerings. To address this, we present SkyStore, a unified object store that addresses cost-optimal data management across regions and clouds. SkyStore introduces a virtual object and bucket API to hide the complexity of interacting with multiple clouds. At its core, SkyStore has a novel TTL-based data placement policy that dynamically replicates and evicts objects according to application access patterns while optimizing for lower cost. Our evaluation shows that across various workloads, SkyStore reduces the overall cost by up to 6x over academic baselines and commercial alternatives like AWS multi-region buckets. SkyStore also has comparable latency, and its availability and fault tolerance are on par with standard cloud offerings. We release the data and code of SkyStore at https://github.com/skyplane-project/skystore.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> figures/tex_files/plot.tex <==
\begin{tikzpicture}[scale=0.9]
    \begin{axis}[
        height=6.0cm,
        xlabel={\large\textbf{K}},
        ylabel={\large\textbf{Pass @ K}},
        xmin=0, xmax=11,
        ymin=0.15, ymax=0.55,
        xtick={1, 2, 3, 4, 5, 6, 7, 8, 9, 10},
        xticklabels={1, 2, 3, 4, 5, 6, 7, 8, 9, 10},
        ytick={0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7},
        legend pos=south east,
        ymajorgrids=true,
        grid style=dashed,
        line width=1pt
    ]
    
    \addplot[color=edgeblue,mark=square]
        coordinates {
        (1, 0.211) (2, 0.307) (3, 0.364) (4, 0.403) (5, 0.432) (6, 0.456) (7, 0.475) (8, 0.492) (9, 0.506)
        (10, 0.518)
        };
​
    \addplot[color=red,mark=square]
        coordinates {
        (1, 0.302) (2, 0.391) (3, 0.43) (4, 0.453) (5, 0.468) (6, 0.479) (7, 0.488) (8, 0.495) (9, 0.501)
        (10, 0.506)
        };
​
    \addplot[color=edgegreen,mark=square]
        coordinates {
        (1, 0.407) (2, 0.456) (3, 0.474) (4, 0.484) (5, 0.491) (6, 0.496) (7, 0.5) (8, 0.503) (9, 0.505)
        (10, 0.506)
        };
​
    \legend{\texttt{GPT3.5}, \texttt{GPT3.5-API}, \texttt{GPT3.5-API-CS}}
    
    \end{axis}
\end{tikzpicture}

==> sections/1_introduction_new.tex <==
\section{Introduction}
In the rapidly evolving landscape of cloud computing, applications increasingly span multiple regions and clouds. Organizations adopt multi-cloud software to reduce costs, avoid vendor lock-in, improve fault tolerance, increase the availability of specific capabilities beyond a single region or cloud, or support geo-distributed services~\cite{jain2022skyplane,cloudcast,skypilot}.
For instance, using multiple clouds to deploy a model serving service reduces monetary costs by up to 50\% on low-availability resources (e.g., GPUs) compared to a single cloud~\cite{sky-serve}.
% For instance, deploying a model serving service across clouds can reduce monetary costs by up to 50\% on low-availability resources (e.g., GPUs) compared to using a single cloud~\cite{sky-serve}. 
To manage vast amounts of data, today, applications rely on object storage services (e.g., Amazon S3, Google Cloud Storage, Azure Blob Storage, and IBM Cloud Object Store. \cite{aws-s3,gcp-storage,ms-azure-blob,ibm-cloud-storage}).
% for a reliable and cost-effective solution. 

% \natacha{These two sentences are somehwat confusing. You first say that users manually place objects across clouds, and then you say that they store everything in one region. Which one is it?  I think this all paragraph could be made much shorter by simply saying "Current solutions cluster around two extremes: store all data locally, which sgiicantly increases egress expenses (give example), or replicate data to multiple regions, as multiple commercial systems do. 
% I also don't think you need to give so many numbers right at the intro} 

% As a result, users manually manage data placement across regions and clouds, which is neither convenient nor cost-efficient -- we need a solution that is both.
% \natacha{These two sentences are somehwat confusing. You first say that users manually place objects across clouds, and then you say that they store everything in one region. Which one is it?  I think this all paragraph could be made much shorter by simply saying "Current solutions cluster around two extremes: store all data locally, which sgiicantly increases egress expenses (give example), or replicate data to multiple regions, as multiple commercial systems do. 

% I also don't think you need to give so many numbers right at the intro}
% Many users simply store all their data using one service in a single cloud and region. While this approach simplifies management and may reduce storage costs, it significantly increases egress expenses when data is frequently accessed from different regions or clouds. Indeed, data transfers within the same cloud provider across regions cost about \$0.19 per GB, and moving data between clouds can cost 23$\times$ more~\cite{cloudcast,aws-pricing,azure-pricing,gcp-pricing}. A popular alternative used by several commercial services~\cite{aws-replication, gcp-multi-region-bucket, minio, microsoftDataRedundancy} is to replicate data to multiple regions. 
% % While this approach lowers network (egress) expenses for repeated accesses
% However, this approach complicates data management and increases storage expenses as data is now replicated at many locations.
%  For example, replicating 500GB data onto 10 AWS S3 Standard Storage buckets costs up to \$200 per month. \shu{storage - cost too low?}


% MODIFIED BELOW?
However, existing object stores operate within their respective clouds and typically limit their operations to specific regions.
As a result, users manually handle data placement across clouds or regions, and their solutions cluster around two extremes: store locally or replicate everywhere. While storing all data in a single cloud region simplifies data management and reduces storage costs, it increases egress expenses when data is accessed from another cloud region~\cite{cloudcast,aws-pricing,azure-pricing,gcp-pricing}. 
% Indeed, data transfers across regions within a cloud cost about \$0.19 per GB, while moving data across clouds costs 23$\times$ more! 
On average, data transfers across clouds costs 23$\times$ more compared to transfers within the same cloud.
On the other hand, replicating data to multiple regions and clouds~\cite{aws-replication, gcp-multi-region-bucket, minio, microsoftDataRedundancy}
% , like most commercial systems~\cite{aws-replication, gcp-multi-region-bucket, minio, microsoftDataRedundancy}, 
may reduce network access fees but can significantly increase storage expenses. 
For example, storing the training data for a Llama3 model with 15 trillion training tokens ($~$60 TB in size)~\cite{}
    across AWS S3, GCS, and Azure Blob standard storage buckets in different regions costs up to \$300K per month~\cite{}.\souj{Fix two missing citations}
% For example, Llama3 model is trained on 15 trillion training tokens (around 60 TB)\cite{}. Storing this training data across AWS S3, GCS, and Azure Blob standard storage buckets in different regions costs up to \$300K per month~\cite{}. \souj{Fix two missing citations}
% \shu{storage - cost too low?}

% AWS: 34, GCP: 40, Azure: 60 
% 500GB * 10 REGION --> $200 per month 
% 10TB * 34 region --> 200 * 20 * 3.4 
% AWS + GCP = 74 region --> 200 * 20 * 7.4
% All regions: 134 --> 200 * 20 * 13.4 

 
% As a result, users manually manage data placement across regions and clouds, which is neither convenient nor cost-efficient -- we need a solution that is both.
% \natacha{These two sentences are somehwat confusing. You first say that users manually place objects across clouds, and then you say that they store everything in one region. Which one is it?  I think this all paragraph could be made much shorter by simply saying "Current solutions cluster around two extremes: store all data locally, which sgiicantly increases egress expenses (give example), or replicate data to multiple regions, as multiple commercial systems do. 

% I also don't think you need to give so many numbers right at the intro}
% Many users simply store all their data using one service in a single cloud and region. While this approach simplifies management and may reduce storage costs, it significantly increases egress expenses when data is frequently accessed from different regions or clouds. Indeed, data transfers within the same cloud provider across regions cost about \$0.19 per GB, and moving data between clouds can cost 23$\times$ more~\cite{cloudcast,aws-pricing,azure-pricing,gcp-pricing}. A popular alternative used by several commercial services~\cite{aws-replication, gcp-multi-region-bucket, minio, microsoftDataRedundancy} is to replicate data to multiple regions. 
% % While this approach lowers network (egress) expenses for repeated accesses
% However, this approach complicates data management and increases storage expenses as data is now replicated at many locations.
%  For example, replicating 500GB data onto 10 AWS S3 Standard Storage buckets costs up to \$200 per month. \shu{storage - cost too low?}
% For example, replicating 

% \souj{However, a key challenge that exacerbates the
% complexity of designing a cost-efficient multi-region and multi-cloud object store
% is the sheer diversity of application workloads}.
% Furthermore, the sheer diversity of application workloads exacerbates the challenges of designing a cost-effective multi-region and multi-cloud data replication system. 
% \natacha{This is the place where I would introduce the sentence "We need a solution that is most cost-effective and convenient. The key challenge there is that cloud workloads are highly diverse. Request patterns often vary across ...}
% \natacha{Suggestion above to shorten this sentece. Quite verbose rn}

Consequently, there is a need for a multi-region, multi-cloud data placement solution that 
minimizes the total monetary cost for various cloud applications.
However, the key challenge in developing such as system is that cloud applications are highly diverse and their data access patterns vary across several dimensions: object size, location distribution, data access recency, and access frequency.
% For instance, a machine-learning application can be trained in a cloud region and later deployed in another region~\cite{skypilot},
% a typical satellite imagery application generates data across cloud regions and analyzes this data centrally in a specific region~\cite{googleLandsatData}.
For applications that perform repeated reads, like model training, it is cost-effective to 
    replicate data to multiple regions as this avoids additional network costs for subsequent reads.
% For instance, model training applications often perform repeated reads---as a result, replicating data to local regions reduces network fees that would otherwise occur, making this technique cost-effective.
% making data replication across regions cost-effective since its reduction in network fees outpaces resulting storage costs. 
In contrast, for applications that read infrequently, like satellite imagery,
    it is cost-effective to occasionally pay for network transfers.  
% In contrast, satellite imagery is accessed infrequently. %, making long-term caching expensive and unnecessary. 
% In this case, paying for occasional network transfers is more efficient. 
\shu{what is it about diversity that makes simple solution not an option - a sentence about why workload diversity makes it a problem (forward reference evaluation): most of the commercially available solutions work well in others but poorly on others}

% Thus, we need a cross cloud, cross region data placement solution that is the most convenient and cost-effective. The key challenge there is that, cloud workloads are highly diverse: request patterns often vary across multiple dimensions, such as object size, location, and access recency and frequency. % \accheng{suggest to remove: (reads and writes)}
% For example, a machine learning model might be trained in \texttt{aws:us-east-1} (N. Virginia) region and later deployed ad-hoc in regions like \texttt{azure:east-asia} (Hong Kong), depending on where serving instances are available \cite{skypilot}.
% In contrast, satellite imagery typically generates data across geo-distributed regions but then analyzes the data centrally (e.g., in the US \cite{googleLandsatData}). 
% % \shu{Describe a bit more here on trade-offs}
% \souj{Implications are not clear; end seems abrupt} \shu{Should we discuss how to describe these applications better? i.e. hotspots impact storage or network cost} \shu{Peter: Connect this to storage of the model parameters, otherwise this reads like an argument for provisioning compute resources. You can also emphasize that models are rapidly becoming larger (e.g., LLMs with 100s of billions of parameters which take 100s of GBs to store).}

\accheng{why is this paragraph here? we should move it up and merge it with the 2nd paragraph since there's repeat info?}
Over the past decade, a plethora of storage solutions have been proposed to address challenges in multi-region and multi-cloud settings.
Commercial systems, such as AWS and GCP, support multi-region buckets\cite{aws-access-point}. However, these services only operate within their respective clouds, and users must manually configure regions for replication.
Geo-distributed systems~\cite{volley, nomad, pileus} handle data replication across cloud regions to minimize latency but ignore transfer costs, which become prohibitive across multiple clouds. 
The most relevant work in this area is SPANStore~\cite{spanstore}, a multi-cloud storage system that considers cost and latency tradeoffs. However, it ignores replication costs and assumes access patterns do not change over time, which limits its practical applicability. 

% assumes access patterns do not change over time, which limits its practical applicability. 

% \shu{shall we move it up to third paragraph? but spanstore limitation is about the workload}


% Over the past decade, a plethora of storage solutions were proposed to address other challenges with data management across clouds and regions. Geo-distributed systems~\cite{volley, nomad, pileus} handle data replication to minimize latency but ignore transfer costs, which are crucial in a multi-cloud setup. Commercial systems like AWS and GCP multi-region bucket\cite{aws-access-point} need manual configurations and only operate within their respective clouds. The most relevant work in this area is SPANStore~\cite{spanstore}, a multi-cloud storage system that considers cost and latency tradeoffs. However, it ignores replication costs and assumes access patterns do not change over time, which limits its practical applicability. \shu{shall we move it up to third paragraph? but spanstore limitation is about the workload}

% \natacha{Not a major thing, but it read a bit strange for you to split the related work in two halfs, where you first talk about what people currently do (the single version vs always replicate), talk about the need for something different, and then go back to related work}
% \accheng{Joey's suggested rewrite: The closest work in this area is SPANStore~\cite{spanstore}, a multi-cloud storage system that considers cost and latency tradeoffs. However, it assumes access patterns do not change over time, its optimizer has limited scalability, which limiting its practical applicability.}
% The closest work is... more explicit: cost, scalability
%Existing multi-cloud systems, such as SPANStore \cite{spanstore}, address cost and latency considerations but assume that access patterns do not change over time, limiting their practical applicability.

In this paper, we present \sys,
    a cost-optimized multi-cloud object store that adapts to diverse workloads and their dynamic access patterns.
\sys provides a single uniform API
    that emulates a local object store while 
    transparently managing data across
    clouds and regions to minimize cost.
In a nutshell, \sys provides an \emph{overlay} cloud service on top of existing cloud object stores that operate in multiple regions and clouds. It decides where an object should be stored and to which locations it should be replicated, if at all, while consistently managing these data copies.
    
% In a nutshell,
% \sys provides an \emph{overlay} cloud service on top of existing cloud object stores that operate within specific regions or clouds.
% It decides where an object should be stored, to which
%     locations it should be replicated, if at all,
%     while managing these data copies consistently.

% In this paper we aim to design a service that provides a single consistent API emulating a local object store, while dynamically managing data placement across regions and clouds to minimize costs. To this end, we present \sys, a cost-optimized, multi-cloud object store that is highly adaptable to diverse workloads. 
% In a nutshell, \sys provides an \emph{overlay} cloud service on top of existing cloud object stores that operate in multiple regions and clouds.
% The system decides where each object should be stored and at which locations it should be replicated, if any.

% Shu
%\sys operates in two modes (Section~\ref{section 2?}), one that allows replicas to be \ion{what does "freely placed and removed" mean?} freely placed and removed, while the others keep a base region in which the replica never gets removed. 
% , and replicas may be created and evicted elsewhere to fit workloads, but the base is never evicted. 
% Danny: too long 
% \sys offers two modes of operation: The first is a free placement mode in which each object can be placed in any region or cloud, adding and removing replicas to fit workload needs and assuring only that at least one replica stays alive at all times. The second mode is a fixed base mode in which each object is assigned a base region, and replicas may be created and evicted elsewhere to fit workloads, but the base is never evicted.   
%Existing commercial services \cite{aws-replication, gcp-multi-region-bucket, minio, microsoftDataRedundancy} focus on improving data reliability via replication and often rely on replicating data manually. Early geo-distributed systems \cite{volley, nomad, pileus} optimize latency but ignore network (egress) costs crucial in a multi-cloud setup. Multi-cloud systems like SPANStore \cite{spanstore} address cost and latency but assume the access frequency does not change over time, which limits their applicability in practice. \shu{This paragraph feels out of place right now}
%At a high level, \sys addresses a caching problem:

% Introduce in S2 right before talking in policy for space 
% \shu{keep 1-1.5 sentence is enough} \sys offers two modes of operation: The first is a free placement mode in which each object can be placed in any region or cloud, adding and removing replicas to fit workload needs and assuring only that at least one replica stays alive at all times. The second mode is a fixed base mode in which each object is assigned a base region, and replicas may be created and evicted elsewhere to fit workloads, but the base is never evicted.
% % \accheng{suggested rewrite of above:
% At a high level, \sys addresses a caching problem: it needs to ``cache'' (i.e., replicate objects from different regions into the region from which they are accessed) and ``evict'' (i.e., if an object is unlikely to be accessed from a particular region again, remove this copy to save storage costs) objects depending on usage patterns.}
% \natacha{Suddenly started using the word we. Minor but good to change}
%it needs to ``cache'' (i.e., stores objects from different regions in the region from which they are accessed) and ``evict'' (i.e., if an object is unlikely to be accessed from a particular region again, remove this copy to save storage costs) objects depending on usage patterns. 


At a high level, \sys addresses a caching problem: it decides to ``cache'' (i.e., replicate objects to their accessed cloud region) and to ``evict'' (i.e., remove object copies from cloud regions if they are unlikely to be re-accessed) based on application access patterns. Unlike traditional caches that optimize for performance and have a finite capacity, \sys optimizes for monetary costs since its capacity is virtually unlimited. However, caching objects incur non-trivial charges associated with network and storage.
% TOO COMPLICATED
% its capacity is an artifact of the non-trivial transfer and storage costs in this multi-cloud environment.
% but transferring and storing data objects in the cache incurs non-trivial monetary costs.

Accordingly, \sys needs to make two decisions: (i) when to cache (i.e., replicate) an object? and (ii) when to evict an object? 
\sys addresses the first with a copy-on-write replication policy. 
% \natacha{Technically not a question, you were talking about decisions earlier}
When a user writes an object, \sys stores it in the local region to minimize cost and latency. If a user reads this object from another cloud region, 
% Suppose a user reads this object from another cloud region where it is not available locally. In that case, 
\sys replicates it from an available region with the lowest transfer fees and ensures that network costs are only incurred for objects that are accessed. 
% (if the object is available in multiple regions).
% This approach ensures that we only incur network costs for replicating objects to locations in which they will be accessed.
% \natacha{This is sufficiently basic that I'm not sure it needs to be in the intro, or take up so much real-estate}
% , which is significant when workloads are unpredictable.   

Second, \sys leverages a novel adaptive Time-To-Live (TTL)-based eviction policy that balances the cost of storing and transferring the object if accessed again.
% Our policy reduces costs by adapting the TTL assigned to replicas based on the current workload and attempts to learn the optimal TTL for each replica. 
% To do so, \sys captures the workload access pattern via a weighted histogram, which describes the distribution of time between object re-reads in each bucket and region. %\accheng{unclear what "time distance between object re-reads" is}. 
% Periodically, the policy estimates what TTL setting would have minimized cost up to this point and adjusts the current TTL setting going forward. This computation is based on the histogram and the ratio between the storage costs and network costs at the various locations. 
% %the best TTL \accheng{what does "best" mean?} based on this histogram for each object. 
% Our policy can adapt to the workload at hand and proves more robust to workload variance than other caching-based methods (Section~\ref{s:eval}). 
Our policy reduces costs by adapting the TTL assigned to objects based on the current workload and attempts to learn the optimal TTL for each replica. \sys captures past workload access patterns to estimate TTL costs and periodically updates these values, providing robustness to workload variance compared to traditional caching-based methods (Section~\ref{s:eval}). \accheng{should add other section refs as well}
We also show how latency considerations can be integrated into our cost-centric framework, making it applicable for clouds with no explicit egress costs, such as the R2 service~\cite{cloudflare-r2} or in a hybrid cloud setting using an on-premise object store (such as ~\cite{ceph-RGW, minio}). 

% We build a prototype of
We implement \sys to seamlessly integrate with existing clouds (e.g., Azure Blob, AWS S3, and GCS).
% while ensures consistency, and provides fault tolerance. 
\sys offers a \textit{virtual bucket} and \textit{virtual object} abstraction via a standard S3-compatible API, allowing users to manage data as if all data were in a single region.  
% data plane and control plane discussion
% Under the hood, \sys consists of a data plane and a control plane.
% The data plane contains stateless web proxies serving the AWS S3 wire protocol that communicate with the control plane and the different object store services. The control plane manages metadata about the objects stored across regions and executes \sys's policies.
\sys provides the same consistency guarantees~\cite{aws-consistency, gcp-consistency, azure-consistency} as its underlying object stores and similar fault tolerance guarantees as existing services. We evaluate \sys on various workloads retrieved from IBM object store traces in the Storage Networking Industry Association (SNIA). 
Our results show that \sys achieves up to 6$\times$ cost savings and has comparable latency relative to the state-of-the-art systems. To summarize, our contributions are as follows: 
\vspace{-0.211em}
\begin{enumerate}
    \item We design a novel cost-optimized data replication policy that can adapt to diverse workload patterns in the multi-region, multi-cloud setting. 
    \item We implement \sys, a cost-efficient multi-cloud storage system that provides virtual object and bucket abstractions, seamlessly integrating with S3, GCS, and Azure Blob Storage as storage backends. 
    \item We evaluate against state-of-the-art policies, showing that \sys's policy can substantially reduce cost by up to 6$\times$ over SNIA object store traces \cite{snia-ibm-object-store-trace} compared to TTL-based policies\cite{TTLbasedCC2019}, SPANStore, and commercial systems like AWS Multi-Region Replication\cite{aws-access-point} and JuiceFS\cite{}. \shu{Note: I think disaster recovery is not a good example here: then the cache replica might never get evicted, we need some places to write about it}
\end{enumerate}
% \michael{In the intro do we want to be more explicit about performance relative to alternatives?  This is mentioned in the paragraph above the bullets but nowhere else. --> be explicit on what are the alternatives}



==> sections/1_outline.tex <==

\section{Outline}
\begin{table*}[t]
\centering
\begin{tabular}{ccccccccc}
\hline
 & AWS / GCP Multi-Region & MinIO & FUSE-based (Rclone, etc.) & Alluxio & Delta Sharing \\ \hline
Data Type & Blob & Blob & Blob & Blob & Database \\


% Compute Type & Web & Web & Real Time & Web & Real Time \\ 

% Consistency & Eventual & Eventual & Eventual & Eventual & $\times$ \\

Multi-Cloud & $\times$ & \checkmark & \checkmark & \checkmark & \checkmark \\
Workload Optimized & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\



\hline \\ 
\end{tabular}

\caption{An overview of industry baselines. }
\label{table:overview}
\end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{ccccccccc}
\hline
 & Volley & Nomad & Pileus / Tuba & SPANStore & Iridium & Akkio & SkyStore\\ \hline
Data Type & File & Database & Blob & Blob & Blob & Database & Blob\\

% Consistency & N/A & Strong/Eventual & 6 Types & Strong/Eventual  & N/A & Strong & RAW/Eventual \\

Multi-Cloud & $\times$ & $\times$ & $\times$  & \checkmark  & $\times$ & \checkmark & \checkmark  \\

Latency/Bandwidth Optimized & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark  \\

Cost Optimized & $\times$ & $\times$ & $\times$ & \checkmark & \checkmark & \checkmark  & \checkmark  \\

Workload Optimized & $\times$ & $\times$ & $\sim$ & $\sim$ & $\times$ &  $\sim$ & \checkmark  \\ 
\hline \\ 


\end{tabular}

\caption{An overview of academic baselines}
% \simon{I think we are missing Scalability here. Ideally, for us SPANStore will not scale beyond X queries per second for read etc... And S3 is famous for ``infinite scalability''. But it could also distract us.}}
\label{table:overview}
\end{table*}

\subsection*{Section 1: Introduction}

% \shu{We should say the workload first (read-heavy), bc there are lots of cases which are not read-heavy, when you don't read after a long time. We should stress the importance and make it clear, not all the workloads are the same - important workloads which are read heavy, i.e. containers, popular contents (pictures, etc.)} .}

\textbf{Why? The world is multi-region and multi-clouds}
\begin{itemize}
    \item The world is already multi-region, and even multi-cloud. 
    
    % \item Driven by market, technological, and regulatory forces, large organizations are rapidly adopting a geo-distributed and multi-cloud technology stack. 
    \item Different clouds provide heterogeneous resource availability, pricing tiers, and services. 
    \item To reduce vendor lock-in, drive down cost (cheaper storage in a specific cloud), and improve performance of applications with specialized resources (cloud specific hardware), organizations are rapidly adopting a geo-distributed and multi-cloud technology stack. \ion{You should give a numerical example here illustrating cost reduction or something else.} 
    \item Example: spot applications and geo-distributed serving tiers turn into multi-region and even multi-cloud to gain access to low availability resources like GPU.\ion{Of course we need citations.}
    \natacha{Definitely need one or two examples that confirm this is true and not niche}
    \item Acquisitions and mergers of organizations, along with data sovereignty policies also enforce organizations to manage customer data in the regions, and cloud providers of their customers
    % \item Stronger data sovereignty policies also force organizations to manage customer data in the regions, and cloud providers of their customers 
\end{itemize}

% \simon{A paragraph on: How has object storage evolved over the last 18 years (2006). Historical context is important here to motivate this is a new and novel problem. Overtime, the feature set of object storage systems have evolved to include strong consistency, multipart/block level file management, tiering, and versioning.}

\textbf{Workloads?}

\begin{itemize}
    \item As a result, data is living in different places (e.g. containers, models, satellite data \cite{}, etc.) . 
    \natacha{Not clear where the "as a result" comes from is. Result of multicloud? It doesn't seem true that the reason why data lives in models/satellites/containers is multicloud}
    \item Most of the workloads use object store for storage \cite{}
    \natacha{Need a citation for this. There was a Materialize blog post that talks about this, there's also articles that describe how geo-science and satellite data is now hosted on S3.}
    \natacha{Also important to say why that is (but I think you should be brief). Low cost, reliability,scalability. API standardised on S3?}
    \begin{enumerate}
        \item \simon{A paragraph on: How has object storage evolved over the last 18 years (2006). Historical context is important here to motivate this is a new and novel problem. Overtime, the feature set of object storage systems have evolved to include strong consistency, multipart/block level file management, tiering, and versioning.}
    \end{enumerate}
\item Workloads are highly variable
\begin{itemize}
    \item Pattern: read and write from different regions and clouds 
    \item Data size: mix size for containers, can be large objects (i.e. model, data) 
    % \item R/W patterns: read-heavy, highly concurrent reads, write few (e.g. 10x R/W ratio) 
    \item R/W patterns: different recency and frequency distribution 
\end{itemize} 
and have requirements in terms of 
\begin{itemize}
    \item Performance: fast repeated reads, fast write 
    \item Consistency: matches the application tolerable consistency level provided by S3, GCP, Azure (e.g. read-after-write and eventual consistency)
    \item Cost: minimize cost 
\end{itemize}
\end{itemize}


\textbf{Challenges: managing multi-region multi-cloud data can be complex, expensive, low-performance}


Unfortunately, managing data associated with a multi-region and multi-cloud technology stack can be expensive and operationally complex. 
\natacha{Flow of the intro was a bit confusing until now because you talk about multicloud -> then object stores->then multicloud}


Typically, users manually manage the placement and movement of data and reason about a patchwork of localized name spaces. (human resources). The challenges are: 
\begin{itemize}
    \item Each provider has different APIs and storage and network (egress) offerings with a wide range of performance, cost trade-offs. 
    \begin{enumerate}
        \item Cross-region storage cost up to 2X cost difference
        \item Cross-region egress cost: 19X
        \item Cross-region data transfer rate: 80X \ion{Need also to say how the egress cost relate to storage cost.}
    \end{enumerate}
    \item Workloads are changing over time, manual management is even harder  
    \item Optimally navigating this complex trade-off space requires understanding application usage patterns.
\end{itemize}

\textbf{Existing Work}
While existing tools can replicate data across regional bucket (e.g. AWS S3 replication, GCP multi-region bucket, Rclone, Alluxio, Delta Sharing) or on-prem (e.g. MinIO), these features are either 1) not supporting multi-cloud, or 2) does not make intelligent placmenet decisions, users need to manually manage.  \shu{Change this to "users need to manually manage"...}

Early academic systems (e.g. Volley, Nomad, Pileus) focus on optimizing placement in geo-distributed applications to minimize client access latency or optimize consistency, but it is not multi-cloud, and pricings under the cloud setup (e.g. bandwidth) is not considered. Systems like SPANStore, Iridiumsupport multi-cloud, but they assume some knowledge of the workloads (e.g. SPANStore - access set, Iridium - complete knowledge on workloads), and thus are less workload-adaptive. Akkio targets facebook-specific workloads (low read-write ratio), and it focues on database, and many of the datasets accessed by their services require strong consistency; while in the object store case it is not. 

\textbf{Examples: why naive management can be expensive and low performance} 
\begin{itemize}
    \item Naively storing data in one centralized place, read and write from it can be 1) high cost, due to the egress price of transferring data across regions and clouds, and 2) low performance, due to the high data access latency across regions and clouds
    \item Replicating data everywhere is a way to address the data access latency, by replicating data upon write. However it can also incur 1) high cost due to the storage fees of storing multiple replicas of the data, and 2) low performance if frequent writes (need to maintain data consistency between replicas) 
\end{itemize}

\textbf{SkyStore - What we do, restate the problem}

\sys is a storage solution that aim to solve the data management problem in multi-region, multi-cloud setting. \shu{Start with the requirements, and state the solutions}
\begin{enumerate}
    \item \textbf{Usability}: s3-compatible API, unified namespace via virtual bucket and object abstraction . \ion{Need to justify this. Maybe say this is the de-facto standard API for cloud storage and provide some citations.}
    \item \textbf{Workload Assumptions} 
    \begin{itemize}
        \item Make no pre-assumption about the workloads \ion{Too vague. Maybe: We consider a general workload that includes (1) small and large objects, (2) both read and write heavy, and (3) both read-after-write and eventual consistency semantics}
        \item \shu{Reactive caching makes sense (opportunistic) when dealing with workload variability, if we don't have the workload knowledge; if perfectly optimal, perfect knowledge on workloads, forever to compute \cite{SkyPie}}
    \end{itemize}
    
    \item \textbf{Performance: Fast repeated reads, Fast writes}
    \ion{Split requirements from solution. First list requirements, and then say how you satisfy these requirements.}
    \begin{enumerate}
        \item Write policy: write local
        \item Read policy: Latency-aware (orthogonal: use skyplane for large data exchange) fetch
        \item Cache policy 
        \begin{enumerate}
            \item Admission: pull-based replication 
            \item Eviction: garbage collections
        \end{enumerate}
    \end{enumerate}
    \item \textbf{Consistency: read-after-write and eventual}
    \begin{enumerate}
        \item Cache coherence policy (consistency): version control 
        \begin{enumerate}
            \item Single region: read-after-write
            \item Multi region: eventual consistency, read local if possible
        \end{enumerate}
    \end{enumerate}
    \item \textbf{Low operational cost}: for reads and writes  
     \begin{enumerate}
        \item Data placement
        \begin{enumerate}
            \item Caching: replicate only when needed 
            \item Eviction: lower storage cost if no access 
        \end{enumerate}
        \item Data transfer: egress pricings-awareness 
    \end{enumerate}
    \item \textbf{Other characteristics} 
    \begin{enumerate}
        \item Scalability: separation of control and data plane, scale each one individually 
        \begin{enumerate}
            \item Control plane: metadata state management 
            \item Data plane: stateless, request translation and execution 
        \end{enumerate}
        \item Fault tolerance and availability model: metadata replication 
    \end{enumerate}
\end{enumerate}

% \sarah{We should have an explanation of why Spanstore/MinIO don't solve the problems we are looking at -- reviewers are very likley to compare/contrast to Spanstore.}

\subsection*{Section 2: Multi-cloud Storage Problem Setup}
\textbf{Problem Statement} \\
For variable workload patterns, minimize \textbf{the cost} and \textbf{latency} for read and write, while maintaining consistency required by the applications \\ \\
\textbf{Solution Space: Questions to Address}
\begin{enumerate}
    \item Besides the traditional problem on read and write 
    \begin{enumerate}
        \item Where to write 
        \item Where to read from 
    \end{enumerate}
    \item Another dimension - Caching
    \begin{enumerate}
        \item Cache admission: when and what to cache 
        \item Cache eviction: when and what to evict from cache 
        \item Cache coherence: how to maintain the consistency between cache copies
    \end{enumerate}
\end{enumerate} 
\textbf{Existing systems}  
\begin{enumerate}
    \item Commercial systems: minIO, AWS, GCP multi-region replication 
    \begin{enumerate}
        \item Users manually define buckets of replication (read and write from these buckets) 
        \item Cache admission: write propagated to other buckets 
        \item Cache eviction: none, high storage cost 
        \item Cache coherence: maintained by provider or replication protocol (eventual consistency)
    \end{enumerate}
    \item Academic systems 
    \begin{enumerate}
        \item SPANStore: high egress and storage when workload is variable 
        \begin{enumerate}
            \item Read / Write: cost and latency-aware 
            \item Cache admission: push-based, propagate upon write, prefetch  
            \item Cache eviction: none 
            \item Cache coherence: strong and eventual consistency
        \end{enumerate}
        \item Volley, Nomad, Pileus: not egress or storage cost-aware 
        \begin{enumerate}
            \item Read and cache admission: latency optimized, but not cost aware 
            \item Cache eviction: none 
        \end{enumerate}
    \end{enumerate}
\end{enumerate}

\textbf{Towards a new approach} 
To reduce egress cost and unnecessary storage as much as possible, cache admission policy should be reactive instead of push-based (e.g. SPANStore). Differ than the traditional cache setting 
\begin{enumerate}
    \item Miss on cache not only brings latency penalty but also monetary cost 
    \item Different object at different region has different miss penalties depending on where other cache copies reside 
    \item There is no fixed cache size: pay as much as you want to store more
    \item Cache eviction goal is to bring down the storage cost
    \begin{enumerate}
        \item Eviction: not compare object with each other to evict, can make individual eviction decision 
    \end{enumerate}
\end{enumerate}

To address caching in the object store setup, we must address the challenge: (1) formalize caching in the object store context, including cost-optimally analysis (2) adapt to the workload patterns dynamically. 

\accheng{Could possibly add a subsection giving an overview of the challenges and / or of the paper (see S2.3 of https://www.usenix.org/system/files/osdi23-cheng.pdf)}

% \accheng{I would including existing systems here and what they address / don't address. maybe make a table with the columns showing the features desired and where things like minIO, spanstore, etc. fall, and skystore should have all the features} 

% \shu{Problem statement (need to redefine it), solution space, and discussion on related works in the context of the solution space (to say what choices they make in the design space), unify with the existing system, and say what is our trace; or solution statement, design space, what traces you make in the design space and then how are the other different}

% \shu{R/W: minimize the cost and latency; build a storage system that minimize these (multi-cloud storage system); in order to solve this, the solution space is where to read, when to read, when to cache, how to evict from cache; some trade-offs (if you want about the challenges, explain the trade-offs in the context of the solutions); what are our choicse or our solution, write-local, cost-aware latency of read, and say what is the related works} 
% \textbf{Challenge 1: Cloud Variability}
% \begin{enumerate}
%     \item Cost, bandwidth heterogeneity: egress, storage, put/get (request) cost;  difference in bandwidth and latency for cross-region, cross cloud transfer 
%     % \item Fault tolerance and availability: managing the locations and ensuring availability of objects in face of network and component failures (and consistency) 
%     \item Storage API heterogeneity: different semantics (put, get, multipart-upload, versioning, etc.) 
% \end{enumerate}
% \textbf{Challenge 2: Workload Variability}
% \begin{enumerate}
%     \item Extract 94 IBM bucket traces: different size, recency and frequency CDF \shu{Within the same workload or across different workloads; making sure to explain it clearly}
%     % \item \shu{Assume variability; important one is gonna impact the design - is it a characteristics (a large number of objects read only once), don't say it. If you have many objects, number of read only objects (talk about it) the fraction of read-only is different across different workloads, different policies on caches; if read only once then don't cache}
%     % \item \shu{Do we need requirement variability here? or shall we stress the importance on workload characteristics? i.e. read-heavy, etc.}
% \end{enumerate} 

% \textbf{Overview on solutions}
% \begin{enumerate}
%     \item Write local
%     \item Cost- and latency-aware read 
%     \item Pull-on-read (cache), garbage collection policy (eviction)
%     \item Coherence: versioning, read-after-write consistency and eventual consistency 
% \end{enumerate}

% \shu{Tight the setup with the workloads (multi-site object, read-heavy); region, cost, workload types, this are the solutions}
% \textbf{Overview on Solutions}
% \begin{enumerate}
%     \item Write local
%     \item Read according to latency and cost trade-offs
%     \item Reactive approach: reactive workloads 
%     \item Cache coherence or consistency model 
%     \begin{enumerate}
%     \item Single Region, read-after-write consistency --> What S3 does, and what we are going to do 
%     \item Between regions, availability with eventual consistency --> if there is a local version, it doesn't make sense you cannot return the local version 
% \end{enumerate}
% \end{enumerate}


\subsection*{Section 3: \sys Solution}
% \accheng{need a different section name, this section is addressing performance and cost? why not put this after you've described the system?}
\begin{enumerate}
    \item Write policy --> Where to write and when to cache?
    \begin{enumerate}
        \item First write: write local 
        \item Cache admission: reactive pull-on-read 
    \end{enumerate}
    \item Read policy --> Where to read and how to maintain cache coherence? 
    \begin{enumerate}
        \item Latency and cost trade-offs 
        \item Cache coherence (consistency) 
        \begin{enumerate}
            \item Read-my-write: always read the latest version 
            \item Eventual consistency: can read from local if there is one  
        \end{enumerate}
    \end{enumerate}
    \item Cache eviction --> When to evict from cache? 
    \begin{enumerate}
        \item Basic eviction policy: two-region, storage v.s egress trade-offs 
        \item Optimal policy and break-even time (proof) 
        \item Choosing the eviction time
        \item Expand this model to multi-region, distributed cache eviction 
        \item Add latency considerations in cache eviction 
    \end{enumerate}
\end{enumerate}

\subsection*{Section 4: System Architecture}
\textbf{Architecture Overview}
\begin{enumerate}
    \item A collection of client VMs (data plane: client libraries) 
    \item A set of DB deployed in each clouds (control plane)
    \item Show the architecture diagram here (or explain how get / put works in such setup) 
\end{enumerate}
\textbf{API} 
\begin{enumerate}
    \item S3 compatible operations: buckets and objects 
    \item additional interface (i.e. allowing prefetch, register existing buckets) 
\end{enumerate}
\textbf{Control Plane and Data Plane}
\begin{enumerate}
    \item Control plane: store-server 
    \begin{enumerate}
        \item Server configuration and database integration 
        \item Metadata abstraction: logical and physical for object and bucket 
        \item Metadata layer functionality 
        \begin{enumerate}
            \item Maintain necessary data location information
            \item Data transfer and placement policies 
            \item Concurrency control and metadata updates 
            \item Speed up metadata-related operations (list, head) 
        \end{enumerate}
    \end{enumerate}
    
    \item Data plane: s3-proxy 
    \begin{enumerate}
        \item design: client-side library, stateless, can scale horizontally 
        \item functionality: operations supported, how it communicates with server 
        \item implementation details: LoC, s3s 
    \end{enumerate}
    
\end{enumerate}

\textbf{Fault Tolerance on Control Plane}
% \accheng{why do we have only fault tolerance as a separate section?}

\begin{enumerate}
    \item Fault tolerance and resiliency model 
    \begin{enumerate}
        \item Data plane failure, what we want 
        \item Control plane failure, what we want (failure in single region server, failure on region) 
    \end{enumerate}
    \item Metadata replication explain 
    \begin{enumerate}
        \item Backup server in single region, sync replicate
        \item Backup server in replicated region, async 
    \end{enumerate}
\end{enumerate}
\subsection*{Section 5: Evaluation}
% \accheng{I would add the 3 high-level eval questions that a lot of systems papers have. The eval will also probably be structured by workload rather than by academic vs. commerical baselines?}\\

\textbf{Eval questions}
\begin{enumerate}
    \item How does using \sys compared to object store in terms of latency and throughput? 
    \item How does \sys algorithm behave in face of different workload patterns? (algorithm ablation) 
    \item How does \sys compare with academic baselines on geo-distributed replication?
    \item How does \sys compare with commercial baselines like the provider's offerings?
\end{enumerate}
\textbf{Eval Plans}
\begin{enumerate}
    \item \textbf{System Ablation}
    \begin{enumerate}
        \item Single region object store
        \begin{enumerate}
            \item Benchmark SkyProxy v.s naive object store (i.e. AWS, GCP, Azure) for object operation latency (e.g. put, get, list, head, delete) 
            \item Benchmark scalability of SkyProxy v.s naive object store for download and upload operations with variable number of threads 
        \end{enumerate}
       \item Repeat experiments for dual-region 
    \end{enumerate}
    \item \textbf{Algorithm ablation}
    \begin{enumerate}
        \item Workloads
        \begin{enumerate}
            \item One hit wonder objects
            \item Lots of repeated read objects 
            \item Synthetic mimic of the real object store traces 
            \item Real object store traces (sample from 96 buckets) 
        \end{enumerate}
    \end{enumerate}
    \item \textbf{Comparison to academic baselines: prototype, simulation}
    \begin{enumerate}
        \item Baselines 
        \begin{itemize}
            \item Store in one place 
            \item Replicate everywhere
            \item Oracle: know-future algorithms 
            \item SPANStore, Iridium, Akkio
        \end{itemize} 
    \end{enumerate}
    \item \textbf{Comparison to commercial baselines: prototype, simulation}
    \begin{enumerate}
        \item Baseline 
        \begin{itemize}
            \item AWS / GCP Multi-Region Replications: more expensive on service fee, manual configured replication (basically without eviction) 
            \item FUSE-based replication baselines: same as above 
            \item \shu{CDN baseline? a huge line of works}
        \end{itemize}
    \end{enumerate}
\end{enumerate}

\subsection*{Section 6: Related Works}
\accheng{this is a section we can write out now (without any of the results) and will help us make sure we've covered all our bases}
\begin{enumerate}
    \item Geo-distributed storage work: SPANStore, Tuba, Volley, Nomad, etc. 
    \item Data transfer work: skyplane, skyplane-multicast  
    \item Multi-cloud related work: skypilot, skyplane, etc. 
\end{enumerate}

% \textbf{Key: } building a unified global object store that brings additional benefits on cost and performance, without losing guarantees for scalability, availability, and fault tolerance as the object store inherently provides

% \todo{A key topic sentence? building a unified global object store that brings additional benefits on cost and performance, without losing guarantees for scalability, availability, and fault tolerance as the object store inherently provides} \newline

% \joey{I think we want to make a stronger claim that the world is already multi-region and even multi-cloud.  SkyStorage is about addressing the present problem of being multi-region and multi-cloud -- not enabling it.}

% \gvernik{exactly...PBs of data  located in different regions and clouds. Example is the USGS or NATO with their Earth Science use cases, where all kind of satellites and sensors write data into different buckets in different regions and clouds. Then a single workload need to access that distributed data. Also 
% all kind of acquisitions, like IBM with IBM Cloud Object Storage, but  acquired The Weather Company that was using Amazon S3.}

% \textbf{Key Question}
% Technical statement for the question
% Can we architect an \textbf{high-performance} and \textbf{low-cost} global object storage backend that exposes a unified interface across providers and automates data management decisions underneath according to the workloads?

% \subsection{What should the metadata look like}
%     \begin{enumerate}
%         \item Global namespace map
%         \item Policies (e.g. cache copy lifetime)
%         \item Access statistics
%         \item Status, migration/copy plans (in transit, etc…)
%     \end{enumerate}
% \subsection{What should the metadata layer do}
%     \begin{enumerate}
%         \item Maintains necessary data locations information 
%         \item Consists of data transfer and placement policies 
%         \item Concurrency control (and locking) 
%         \item Speed up metadata-related operations (e.g. List operations)
%     \end{enumerate}
% \subsection{What storage medium do store metadata}
%     \begin{enumerate}
%         \item Persistent store
%         \item In-memory cache 
%         \item Object store backend 
%     \end{enumerate}
%     \begin{enumerate}
%         \item Decentralized: Distributed across regions (i.e. maybe close to where the data source is), hash decentralization 
%         \item Centralized: single region DB
%     \end{enumerate}


% \begin{enumerate}
%     \item Setup 
%     \begin{enumerate}
%         \item The world is heading multi-region and multi-cloud
%         \item Driven by market, technological, and regulatory forces, large organizations are rapidly adopting a geo-distributed and multi-cloud technology stack. 
%         \begin{itemize}
%             \item Market: organizations grow and merge with other organizations, forced to merge multiple independent cloud technology stacks. To reduce vendor lock-in, mix multiple cloud providers for the same services.
%             \item Workload: data can be already distributed 
%             \item Technology: turn to multi-region spot applications, geo-distributed serving tiers, and multiple cloud providers to gain access to low-\textbf{availability} resources (e.g. GPUs) (or higher data availability), \textbf{reduce latency}, and drive down \textbf{cost}. 
%             \item Regulatory: stronger data sovereignty policies forces organizations to manage customer data in the regions, and cloud providers of their customers 
    
%     \end{itemize}
        
%     \end{enumerate}
%     \item Example workload 
%     \begin{enumerate}
%         \item Typical object store workloads (IBM traces) 
%         \item Container (model, image) sharing across regions and clouds, upload once, read multiple times 
%         \item Size: mixture of sizes, heavy read, little write 
%     \end{enumerate}
%     \item Challenges: complexity in data management 
%     \begin{enumerate}
%         \item Complexity: dealing with different storage APIs across cloud vendors, navigating the trade-offs between cost, performance, and consistency 
%         \item Performance: achieve fast repeated reads, and fast writes 
%         \item Cost: storage, request, egress  
%         \item Workload patterns: access patterns can be not so predictable (try this and make unrealistic assumption) 

        
%     \end{enumerate}
%     \item Contributions 
%     \begin{enumerate}
%         \item Reduce data management complexity via virtual bucket/object abstraction
%         \item Improve performance and cost via runtime- and cost-aware reactive placement and access policy 
%         \item "Zero-overhead" in system design (separation of control and data plane, simple replication and backup model on metadata) \shu{(what system are we comparing against; changes nothing, can crash, can recover) (challenges to do it across multi-cloud, want to preserve all the properties) (minimal cost and all the benefits)}
%     \end{enumerate}
% \end{enumerate}

% \begin{enumerate}
%     \item API design: S3-compatible operations - talk about each cloud implementation in detail 
%     \begin{enumerate}
%         \item Virtual bucket and object abstraction 
%         \item Object implementations: put, get, copy, multipart, delete, head 
%         \item Bucket implementation: create, delete, list 
%         \item Versioning support
%         \item Interface: register, warmup  
%     \end{enumerate}
%     \item Data plane: s3-proxy 
%     \begin{enumerate}
%         \item stateless
%         \item client-side library 
%     \end{enumerate}
%     \item Control plane: store-server 
%     \begin{enumerate}
%         \item Metadata 
%         \begin{enumerate}
%             \item Logical bucket and physical bucket abstraction 
%             \item Logical object and physical object abstraction 
%         \end{enumerate}
%         \item Metadata layer functionality 
%         \begin{enumerate}
%             \item Maintain necessary data location information
%             \item Data transfer and placement policies 
%             \item Concurrency control and metadata updates 
%             \item Speed up metadata-related operations (list, head) 
%         \end{enumerate}
%         \item Metadata availability/resiliency model
%         \begin{enumerate}
%             \item \sys should provide availability and resiliency that
%             are on par with a solution that does not use \sys
%             but rather places objects in separate buckets in different
%             regions or clouds.
%             \item In such a solution, a client will have
%             access to all objects as long as the corresponding object storage is up and there is network connectivity to the
%             respective region or cloud.
%             \item A network
% failure between two clouds may render objects residing
% solely on the remote cloud inaccessible but should not
% affect the availability of local objects
%             \item Location catalog cached in each cloud and region, updates are synchronized with the centralized DB periodically
%             \item Upon writing an object, the DB at the region
%             in which the object was written should be updated first.
%             This information should then be propagated to the other
%             DB instances
%             \item Look up and listing can fall back to centralized DB if the object not yet appear in the local DB instance 
%         \end{enumerate}
%     \end{enumerate}
% \end{enumerate}

% \item \shu{simple policy, reactive, create a copy upon request (get or warmup request); eviction: focus on cost, the performance aspect of it (discussion points, positive correlation between cost and performance, egress cost is much higher than storage cost, if store object and save egress cost, also saving latency; read: closest replica, lowest latency and cost; )}

% \begin{itemize}
    %     \item Market:  To reduce vendor lock-in, mix multiple cloud providers for the same services. \shu{Booking: data lake, reference for that; Taboola Outbrain: analytics, collecting from each country; start with the vendor lock-in, reduce the cost, and improve performance} organizations grow and merge with other organizations, forced to merge multiple independent cloud technology stacks. \shu{this is the secondary reasons, don't categorize these reasons}
    %     \item Workload: data can be already distributed 
    %     \item Technology: turn to multi-region spot applications, geo-distributed serving tiers, and multiple cloud providers to gain access to low-\textbf{availability} resources (e.g. GPUs) (or higher data availability), \textbf{reduce latency}, and drive down \textbf{cost}. 
    %     \item Regulatory: stronger data sovereignty policies force organizations to manage customer data in the regions, and cloud providers of their customers 
    % \end{itemize}

==> sections/1_sosp_old_introduction.tex <==
\section{Introduction}
% \shu{Lmk if there are any modifications except grammar, leave comments on large modifications will be great!} 
% \shu{Do we want to talk about customer single endpoint first? virtual bucket abstraction, after talking about this, talking about the actual challenges -- The organization would ideally work with a service that looks local but underneath the hood spans object sores in multiple clouds and regions. We aim at providing such a service that will decide how best to choose...}
% \newline 
In the rapidly evolving landscape of cloud computing, applications are increasingly multi-region and multi-cloud. Organizations are adopting a multi-cloud software stack to prevent vendor lock-in, reduce costs, improve fault tolerance, improve the availability of specific capabilities at a single site or cloud, or simply to support geo-distributed services \cite{jain2022skyplane,cloudcast}. 
% \accheng{I think we still need some citations here} 
For instance, deploying a model serving service across regions and clouds can reduce costs by up to 50\% on low-availability resources (e.g., GPUs) compared to using a single region or cloud~\cite{sky-serve}. 

% \accheng{object store is a central component but not designed for multi-region/cloud}
% A central component of virtually any cloud provider is the object storage service 
Most applications running in the cloud rely on an object storage service (e.g., Amazon S3, Google Cloud Storage, Azure Blob Storage, and IBM Cloud Object Store \cite{aws-s3,gcp-storage,ms-azure-blob,ibm-cloud-storage}), which provides a reliable and cost-effective solution for managing vast amounts of data. 
% \shu{the topic sentence a bit repetitive on the however sentences?}
However, existing object stores are not designed to support multi-region and multi-cloud workloads: they operate only in their respective clouds and typically confine operations to specific regions within each cloud. These limitations complicate data management. 
% \natacha{"in the multi-region/cloud setting -> can remove sentence if short on space}

% Currently, organizations often need to navigate various storage and network options to develop cost-effective object storage strategies.

% While Object storage APIs allow remote access to objects, this is a pricey operation that also carries high latency with it. 

% \accheng{change prev sentence to: }
% Object store APIs allow remote access to objects and it is tempting to 
% As a result, organizations often need to navigate various storage and network options to develop cost-effective object storage strategies. 
As a result, users need to manually decide where to store data objects, which is neither convenient nor cost-efficient.
% \accheng{change prev sentence to: As a result, users need to manually decide where to store data objects, a task that is neither convenient nor cost efficient.}
%As a result, object store users need to decide where to place data manually, and existing policies are often not cost-efficient. 
Many users simply store all the data using one service in a single cloud and region. While this minimizes storage costs and simplifies management, it significantly increases egress expenses when data is frequently accessed from different regions or clouds. Indeed, data transfers within the same cloud provider across regions cost up to \$0.19 per GB, and moving data between clouds can cost 23$\times$ more~\cite{cloudcast,aws-pricing,azure-pricing,gcp-pricing}. A popular
alternative used by several commercial services~\cite{aws-replication, gcp-multi-region-bucket, minio, microsoftDataRedundancy} is to replicate data to multiple locations. This can potentially lower network (egress) expenses, but it complicates data management, as data must be replicated at the locations where it is accessed. While this approach reduces the transfer costs when the data object is accessed repeatedly at the same location, it can result in higher storage costs.
% it increases the cost of storing the replica at that location. \accheng{change prev sentence to: it can result in higher storage costs}
%This approach, of course,  can escalate storage costs significantly in some cases. 
For example, replicating 500GB data onto 10 AWS S3 Standard Storage buckets costs up to \$200 per month. 
%\accheng{we should still mention these systems}
%While some geo-distributed systems \cite{volley, nomad, pileus}  use replication to minimize latency, they ignore transfer costs, which are crucial in a multi-cloud setup. 
% \natacha{This paragraph is a lot of "while X ..., this. Yuo have two/three in a row. I'd remove the comment about geo-replication for readability}

% Existing approaches to multi-region and multi-cloud object storage fall short of application needs. \accheng{we should make clear cost is the main concern early on (if it is our main focus)}
% Many organizations simply choose to store all of the data using one service in a single cloud and region. \accheng{would add some citations for this} This minimizes storage costs and simplifies management. However, it significantly increases egress expenses when data is frequently accessed from different regions or clouds. Indeed, data transfers within the same cloud provider across regions costs up to \$0.19 per GB, and moving data between clouds is up to 23$\times$ more. As an alternative, some commercial services~\cite{cloudcast,aws-pricing,azure-pricing,gcp-pricing} \accheng{does this reflect recent changes in cloud policy that removed egress costs?} enable applications to manually replicate data to multiple locations~\cite{aws-replication, gcp-multi-region-bucket, minio, microsoftDataRedundancy}. This has the potential to lower egress expenses, but it complicates data management: it is only worthwhile to replicate data that will be accessed in other locations. This approach can escalate storage costs significantly (in the AWS regions, the storage pricing ranges from \$0.021 to \$0.041 per GB per month for S3 standard storage\cite{s3-pricing}). \accheng{maybe give an example of storage cost increase given X amount of data rather than just the storage pricing numbers}
% On the research side, early geo-distributed systems~\cite{volley, nomad, pileus} optimize for latency but ignore data egress costs crucial in a multi-cloud setup. Multi-cloud systems, such as SPANStore \cite{spanstore}, address cost and latency concerns but assume that access patterns do not change over time, which limits their applicability in practice. \accheng{is spanstore the only multi-cloud system relevant to us?}

Furthermore, the sheer diversity of application workloads exacerbates the challenges of designing a cost-effective multi-region and multi-cloud data replication system. Request patterns often vary across multiple dimensions, such as object size, location, and access frequency. % \accheng{suggest to remove: (reads and writes)}
For example, a machine learning model might be trained in \texttt{aws:us-east-1} (N. Virginia) region and later deployed ad-hoc in regions like \texttt{azure:east-asia} (Hong Kong), depending on where serving instances are available \cite{skypilot}.
In contrast, satellite imagery typically generates data across geo-distributed regions but then analyzes the data centrally (e.g., in the US \cite{googleLandsatData}). 

Over the past decade, a plethora of storage solutions have been proposed to address various challenges in multi-region and multi-cloud settings. Geo-distributed systems~\cite{volley, nomad, pileus} use replication to minimize latency but ignore transfer costs, which are crucial in a multi-cloud setup. The most relevant work in this area is SPANStore~\cite{spanstore}, a multi-cloud storage system that considers cost and latency tradeoffs. However, it only optimizes for access costs, ignores replication costs, and assumes access patterns do not change over time, which limits its practical applicability.
% \accheng{Joey's suggested rewrite: The closest work in this area is SPANStore~\cite{spanstore}, a multi-cloud storage system that considers cost and latency tradeoffs. However, it assumes access patterns do not change over time, its optimizer has limited scalability, which limiting its practical applicability.}
% The closest work is... more explicit: cost, scalability
%Existing multi-cloud systems, such as SPANStore \cite{spanstore}, address cost and latency considerations but assume that access patterns do not change over time, limiting their practical applicability.

In this paper we aim to design a service that provides a single consistent API emulating a local object store, while dynamically managing data placement across regions and clouds to minimize costs. To this end, we present \sys, a cost-optimized, multi-cloud object store that is highly adaptable to diverse workloads. 
In a nutshell, \sys provides an \emph{overlay} cloud service on top of existing cloud object stores that operate in multiple regions and clouds.
The system decides where each object should be stored and at which locations it should be replicated, if any.

% Shu

%\sys operates in two modes (Section~\ref{section 2?}), one that allows replicas to be \ion{what does "freely placed and removed" mean?} freely placed and removed, while the others keep a base region in which the replica never gets removed. 
% , and replicas may be created and evicted elsewhere to fit workloads, but the base is never evicted. 
% Danny: too long 
% \sys offers two modes of operation: The first is a free placement mode in which each object can be placed in any region or cloud, adding and removing replicas to fit workload needs and assuring only that at least one replica stays alive at all times. The second mode is a fixed base mode in which each object is assigned a base region, and replicas may be created and evicted elsewhere to fit workloads, but the base is never evicted.   
%Existing commercial services \cite{aws-replication, gcp-multi-region-bucket, minio, microsoftDataRedundancy} focus on improving data reliability via replication and often rely on replicating data manually. Early geo-distributed systems \cite{volley, nomad, pileus} optimize latency but ignore network (egress) costs crucial in a multi-cloud setup. Multi-cloud systems like SPANStore \cite{spanstore} address cost and latency but assume the access frequency does not change over time, which limits their applicability in practice. \shu{This paragraph feels out of place right now}
%At a high level, \sys addresses a caching problem:

% Introduce in S2 right before talking in policy for space 
% \shu{keep 1-1.5 sentence is enough} \sys offers two modes of operation: The first is a free placement mode in which each object can be placed in any region or cloud, adding and removing replicas to fit workload needs and assuring only that at least one replica stays alive at all times. The second mode is a fixed base mode in which each object is assigned a base region, and replicas may be created and evicted elsewhere to fit workloads, but the base is never evicted.
% % \accheng{suggested rewrite of above:
% At a high level, \sys addresses a caching problem: it needs to ``cache'' (i.e., replicate objects from different regions into the region from which they are accessed) and ``evict'' (i.e., if an object is unlikely to be accessed from a particular region again, remove this copy to save storage costs) objects depending on usage patterns.}
% \natacha{Suddenly started using the word we. Minor but good to change}
%it needs to ``cache'' (i.e., stores objects from different regions in the region from which they are accessed) and ``evict'' (i.e., if an object is unlikely to be accessed from a particular region again, remove this copy to save storage costs) objects depending on usage patterns. 
At a high level, \sys addresses a caching problem: it needs to ``cache'' (i.e., replicate objects from different regions into the region from which they are accessed) and ``evict'' (i.e., if an object is unlikely to be accessed from a particular region again, remove this copy to save storage costs) objects depending on usage patterns. However, unlike traditional caching policies, which focus on optimizing performance given a finite cache capacity, \sys focuses on optimizing for monetary costs in an environment in which the cache (i.e., cloud object store) capacity is virtually unlimited, but transferring and storing data objects in the cache incurs non-trivial monetary costs.
% These differences lead to novel %varying 
% tradeoffs and solutions for \sys.
% \natacha{Last sentence doesn't add much IMO, would remove}

% for organizations would be a service that mimics the API of a local object store with a single consistent API, yet behind the scenes handles actually interacting with the various object store services as well as choosing where to place data and when to move it or replicate it in a way that minimizes costs. This is exactly what \sys aims to provide. To this end, in this paper, we focus on how can we best choose when, and where to create and delete data replicas across regions to minimize monetary costs associated with cloud storage and networks.  
 %nd is only beneficial if you replicate data that is bound to be accessed. %, especially for a large number of objects with a long tail of rarely accessed data. %\ion{Give some numbers for storing data as well.}
%\danny{The effect of store everywhere is actually more painful for network than storage. You are sending to objects to locations they might never be accessed in... }
% \tiemo{This last sentence does not connect. May drop.} \shu{Ion: just put it here, but not sure the numbers are good enough} \michael{In Sao Paulo it is \$0.0405 per GB }


% For example, on an object store workload in AWS, it is up to 7$\times$ more expensive to replicate data than re-fetching data over the network upon access. 
% For example, maintaining 500 GB of data across 10 AWS regions using standard S3 storage costs could average \$115 per month. 
% Storage, on the other hand, is more affordable in comparison. As an example, AWS average storage pricing per month (i.e. \$0.024 per GB per month) in a single region costs 2.3$\times$ less than a single network transfer cost (i.e. \$0.056 per GB). Thus, creating multiple data replicas in various regions becomes a strategic approach that may lower egress expenses. However, excessive data copies can still escalate storage costs, especially for infrequently accessed objects.

% \natacha{Had a hard time following the argument you wanted to make in this paragraph. Maybe a simpler either/or structure would work? 1) Single region -> high egress fee 2) multi region -> gets expensive when you have a large number of objects and a long tail} \shu{shall we stress the difference between storage and network fees?}\natacha{given you end up trading off between them, it wasn't clear to me why we needed to stress the difference}

% but it raises storage expenses over time. 

% The storage cost also varies across regions and clouds: for example, standard storage in \texttt{gcp:southameria-east1} region costs \$$0.035$ per GB per month, which is $1.75\times$ more expensive than storing data in S3 standard bucket in \texttt{aws:us-east-1}. 

% For example, maintaining 500 GB of data across 10 AWS regions using standard S3 storage costs could average \$115 per month \shu{Put per GB for storage as well, so what is the difference}. 

% The challenges of designing a cost-effective multi-region or multi-cloud data replication system are exacerbated by the sheer diversity of workloads that vary across different dimensions, such as object size, location, and access frequency (both reads and writes).
%---a diversity in the number and size of objects as well as the origin and frequency of accesses. 
%which vary in how frequently they access each object and where from. 
% \natacha{which vary in how frequently they access each object and where from? thought that it was a bit hard to read}. 
% For example, a machine learning model might be trained in \texttt{aws:us-east-1} (N. Virginia) region and later deployed ad-hoc in regions like \texttt{azure:east-asia} (Hong Kong), depending on where serving instances are available \cite{skypilot}.
% In contrast, satellite imagery typically generates data across geo-distributed regions but then analyzes the data centrally, e.g., in the US \cite{googleLandsatData}.
%Applications like satellite systems have a different operational cycle: image data is typically generated monthly in \texttt{aws:eu-north-1} (Stockholm) and transmitted to US regions for one-time data analysis. 
% \natacha{are you talking about diversity across workloads or within a workload} \shu{more like across}

% To address these complexities, it is crucial to carefully analyze the design space, and strategically decide when and where to create or delete data replicas according to the workload. The goal is to optimize monetary costs, particularly related to cloud storage and egress charges. 
% \danny{Perhaps say something like earlier in the paper? The organization would ideally work with a service that looks local but underneath the hood spans object sores in multiple clouds and regions. We aim at providing such a service that will decide how best to choose...}
%danny - move the following earlier
%To this end, in this paper, we focus on how can we best choose when, and where to create and delete data replicas across regions to minimize monetary costs associated with cloud storage and networks. % \natacha{I would be more direct: This paper asks, how can we best choose to create/data replicas to ensure good performance while minimizing monetary costs (cloud storage, egress charges)} 
% (e.g., AWS S3\cite{aws-replication}, GCP Multi-region Bucket \cite{gcp-multi-region-bucket}, Minio \cite{minio}, and Microsft Azure \cite{microsoftDataRedundancy}) 
% Existing commercial services \cite{aws-replication, gcp-multi-region-bucket, minio, microsoftDataRedundancy} focus on improving data reliability via replication, and often rely on replicating data manually. Early geo-distributed systems \cite{volley, nomad, pileus} optimize latency but ignore data egress costs crucial in a multi-cloud setup. Multi-cloud systems like SPANStore \cite{spanstore} address cost and latency but assume the access frequency does not change over time, which limits their applicability in practice. 
%their adaptability to changing workloads.
% \natacha{Are you saying they only look at it weekly?} \shu{yeah they use this week to predict next week}

% \shu{Key question: when you access the data, whether you are going to make a copy of it locally or not; second question: when to delete that copy, these questions are similar in the context of caching. Caching trying to optimize performance given the finite capacity of the cache, in this case we want to minimize the cost because capacity is infinite}

% In this paper we present \sys, a cost-optimized virtualization layer on top of multiple object stores. It is simple to use and highly adaptable to diverse workloads.
% We present \sys, a cost-optimized multi-cloud object store that 
% is highly adaptable to diverse workloads, including workloads that change over time. In a nutshell, \sys provides an \emph{overlay} cloud service over existing cloud object stores that run in multiple regions and clouds.
% It decides where the object should be stored, and potentially replicates objects in multiple locations. 
% \sys draws inspiration from traditional caching mechanisms in that it caches objects that are stored in one region when accessed from a different region, and evicts the cached objects depending on usage patterns. 
%: it treats object stores at each region of each cloud as caches, creates on-demand replicas, and strategically evicts data depending on usage patterns. 
% However, unlike traditional cache mechanisms which focus on optimizing performance given a finite cache capacity, in our case we focus on optimizing for monetary costs in an environment in which the cache (i.e., cloud object store) capacity is virtually unlimited, but transferring and storing data objects in the cache incurs non-trivial costs.
%caching but incurs costs both on access (i.e., data transfer) and ongoing costs based on usage. 
% \simon{virtually unlimited but incur ongoing cost based on usage.}
% These differences lead to different tradeoffs and solutions for caching policies. 

% In the remainder of this paper, we use "caching" and "replication" interchangeably, as well as "cache" and "region" (where the object is being replicated).  \shu{Why do we clarify the notion here? shouldn't it be done in the background or wherever the concept is setup}
%\danny{Should add the two modes of fixed base and free placement somewhere here. The free placement is another differentiator from standard caches} 
%This shift enables \sys to move beyond space management to cost optimization. 

% In response to these challenges, we propose \sys, a cost-effective storage system that is easy to use and highly adaptable to diverse workloads. \sys casts the data management as an on-demand caching problem in the context of multi-cloud. Unlike traditional cache which is limited by predetermined sizes, cloud cache capacity is virtually unlimited but costs money. This shift enables \sys to move beyond space management to cost optimization. 

% \shu{The main difference is that, in our case, there is no space limitation, is budget limitation (?) Performance of cache --> infinite, storing and moving data cost moeny} 


% Like traditional caching systems, 
Similar to conventional caching systems, \sys makes two decisions: (i) when to cache (i.e., store) an object? and (ii) when to evict an object? 
\sys answers the first question by implementing a read-driven replication policy.
When a user writes a data object, \sys stores it in the local region to minimize both cost and latency. When an object is read, if the object is not in the local region, \sys creates a local replica by copying it from the region that minimizes the transfer cost (if the object is available in multiple regions). This approach ensures we only incur network costs for replicating objects to locations in which they will be accessed.
% , which is significant when workloads are unpredictable.   

For eviction, \sys leverages a novel Time-To-Live (TTL)-based policy. The goal of the TTL is to balance the cost of storing the object and the cost of transferring the object if accessed again.
% Our policy reduces costs by adapting the TTL assigned to replicas based on the current workload and attempts to learn the optimal TTL for each replica. 
% To do so, \sys captures the workload access pattern via a weighted histogram, which describes the distribution of time between object re-reads in each bucket and region. %\accheng{unclear what "time distance between object re-reads" is}. 
% Periodically, the policy estimates what TTL setting would have minimized cost up to this point and adjusts the current TTL setting going forward. This computation is based on the histogram and the ratio between the storage costs and network costs at the various locations. 
% %the best TTL \accheng{what does "best" mean?} based on this histogram for each object. 
% Our policy can adapt to the workload at hand and proves more robust to workload variance than other caching-based methods (Section~\ref{s:eval}). 
Our policy reduces costs by adapting the TTL assigned to replicas based on the current workload and attempts to learn the optimal TTL for each replica. \sys captures past workload access patterns to estimate TTL costs and periodically updates these values, providing robustness to workload variance compared to caching-based methods (Section~\ref{s:eval}).
We also show how latency considerations can be integrated into our cost-centric framework, making it applicable for clouds with no explicit egress costs, such as the R2 service~\cite{cloudflare-r2} or in a hybrid cloud setting using an on-premise object store (such as ~\cite{ceph-RGW, minio}). % citation as :(https://ceph.io/en/discover/technology/#object) 


% ~\cite{ceph-RGW (https://ceph.io/en/discover/technology/#object), minio}).  
%\danny{Please do not edit the section above unless you fully understand what our method does}
%what would have been the best TTL setting up to this point and adjusts the current TTL setting going forward. This computation is based on the histogram and on the ratio between the storage costs and network costs at the various locations. 
% We compare our eviction policy to other TTL based eviction policies and show that it manages to adapt to variable workloads whereas other methods are not robust to workload variance.  

% Shu's version
%\sys eviction policy further reduces costs by assigning TTL for data replicas in each cloud region, adapting to diverse workload patterns. At a high level, TTL determines the duration data should remain stored before eviction. This balances the storage costs against potential egress expenses of fetching data over the network. \sys eviction policy employs a weighted histogram that collects how frequent and recent objects are re-read per bucket in each cloud region. By periodically analyzing this histogram, the policy attempts to learn the optimal TTL to ensure that data is stored just long enough to be cost-effective, minimizing the expected total cost. \shu{We also design a variance of \sys strategy to provide the best-effort latency improvement for repeated reads?}
% \shu{Does this work? I think high-level explain why TTL mechanism, what is the trade-offs here are pretty important}
% \danny{Intuition is good but we need to be very accurate and not misleading. "determines the optimal TTL" is not true. rather "attempts to learn the optimal TTL" - I chose the wording carefully to be correct. }

% %time to remove replicas based on workload access patterns and cloud service pricing.
% %This method employs a weighted histogram of access time at the bucket level in each region to inform TTL decisions.
% For each replica, it captures the access pattern and compares the expected cost of storing the replica versus transferring it anew,
% %With this information, \sys's eviction policy compares the expected cost of storing a replica until its next access against the cost of transferring it anew,
% choosing the cheaper option. \danny{This describes the clairvoyant strategy, not what we do}
% Unlike traditional caching systems where objects compete for limited cache space, \sys allows for individual TTL decisions tailored to each object access pattern, further enhancing cost efficiency.\danny{This is also not what we do. This is what EWMA does which works very poorly. The fact that cache is unlimited is needed to make TTL work even with same TTL for all, not for separate TTLs.} 
% %Additionally, \sys incorporates a strategy variation to incorporate latency considerations into the cost-driven framework. 
% Additionally, \sys allows to tie in latency consideration into its cost-driven policies.

% Moreover, \sys policy makes individual TTL decisions for objects based on their replica location, in contrast to traditional cache eviction where objects compete with each other to stay in the cache. We also design a variance of \sys strategy to provide the best-effort latency improvement for repeated reads. 

We build a prototype of \sys that seamlessly integrates with existing clouds (e.g., Azure Blob, AWS S3, and GCS).
% while ensures consistency, and provides fault tolerance. 
\sys offers a \textit{virtual bucket} and \textit{virtual object} abstraction via a standard S3-compatible API, allowing users to manage data as if all data were in a single region.  Under the hood, \sys consists of a data plane and a control plane.
The data plane contains stateless web proxies serving the AWS S3 wire protocol that communicate with the control plane and the different object store services.
% Under the hood, \sys consists of a data plane and a control plane.
% The data plane is a proxy implemented as a fully compatible web server that communicates to various storage providers.
The control plane manages metadata about the objects stored across regions and executes \sys's policies.
Furthermore, our system ensures the same consistency as its underlying object stores: \textit{read-after-write} and \textit{eventual consistency}~\cite{aws-consistency, gcp-consistency, azure-consistency}. 
It also provides the same fault tolerance guarantees as existing services through the stateless proxy and fault-tolerant database.
% a replicated metadata architecture. %\shu{Audrey: is it sound better than primary-seconedary metadata architecture?}

% We implement multiple replication policies in \sys and run end-to-end system evaluations for comparison. 
We evaluate \sys on various workloads generated from IBM object store traces in the Storage Networking Industry Association (SNIA). 
Our results show that \sys can achieve up to 69.5\% cost savings while maintaining latency comparable to the state-of-the-art systems. To summarize, \sys's contributions are as follows: 
\vspace{-0.211em}
\begin{enumerate}
    \item We design a novel cost-optimized data replication policy that can adapt to diverse workload patterns in the multi-region, multi-cloud setting. 
    \item We build \sys, a cost-efficient multi-cloud storage system that provides virtual object and bucket abstractions, seamlessly integrating with S3, GCS, and Azure Blob Storage as storage backends. 
    \item We implement and evaluate various state-of-the-art policies, showing that \sys's policy can substantially reduce cost by up to 69.5\% on 31 SNIA object store traces \cite{snia-ibm-object-store-trace} compared to TTL-based policies and SPANStore. 
\end{enumerate}
% \michael{In the intro do we want to be more explicit about performance relative to alternatives?  This is mentioned in the paragraph above the bullets but nowhere else. --> be explicit on what are the alternatives}


%%%%%%%%%%%%%%%%
% \shu{the last two sentences are weird, also, is this descriptive enough? shall we provide an example?}

% Like caching solutions, our strategy provides the best-effort latency improvement for repeated reads, and its effectiveness is workload-dependent. 

%\sys employs an adaptive eviction policy to determine when to evict data based on workload access patterns and the service pricing at different regions and clouds. 

%he policy compares the costs of storing data against the cost of network transfer to decide whether maintaining a replica is more cost-effective than re-transferring it when next needed. The policy collects access recency histograms at the bucket level to reflect common patterns and trends within a particular workload and calculates the time-to-leave (TTL) for individual objects within the bucket. Differ from traditional caching where objects compete with each other for eviction, \sys cache can make independent decisions on each object within the bucket, depending on their replica locations. 

% \shu{need to improve this, how to frame it? being more precise, the question is about whether to cache or copy, and when to evict; the question about when to evict: predict when to access the next time, see whether it is cheaper to keep it or cheaper to copy it again. }
% \begin{enumerate}
%     \item Time-based eviction is used by \sys to navigate the cloud's cost dynamics - storage is billed per GB per month, and network cost is per GB transferred.
%     \item The insight in TTL-based eviction lies in its ability to minimize overall storage and network cost by determining when data should be evicted based on its likelihood of future access.
%     \item Unlike traditional capacity-constrained caching where objects compete for space, \sys leverages the virtually unlimited capacity of the cloud to make cost-optimized eviction decisions for each object individually.
%     \item By collecting a histogram of access patterns for each bucket, \sys can dynamically adjust TTL to minimize the total expected cost. 
% \end{enumerate}

 % The insight of time-based eviction lies in its ability to balance these costs by intelligently determining when data should be evicted based on its likelihood of future access.  By collecting a histogram of access patterns for each bucket, \sys can dynamically adjust TTL to minimize the total expected cost that accounts for both storage and network. \shu{This needs improvement, how to frame it better?} 

% At the core of \sys cost-aware strategy is an adaptive TTL-based eviction policy, designed to judiciously balance storage costs and egress costs of retrieving data that is not locally available. \sys eviction policy adapts to real-world usage patterns, learning from workload through the collection of a weighted histogram of access statistics. \shu{need to update this} Like caching solutions, our strategy provides the best-effort latency improvement for repeated reads, and its effectiveness is workload-dependent. 


% \begin{itemize}
%     \item When to store: initially, written data is stored locally to minimize write latency and costs.
%     \item When to replicate: for subsequent reads, the policy finds the most cost-effective data sources to read and creates replicas only where needed.
%     \item When to evict: \sys eviction policy prevents storage costs from exploding by storing too many replicas. It balances the trade-offs between storage expenses and potential egress costs from cache misses according to the actual usage patterns. 
%     % \item There are some existing works (dynamic TTL, To-keep-or-not-keep) that frame cloud caches as a cost-centric model similarly, but they do not consider network egress cost across multi-region and clouds, and their policies make strong assumptions about workload distributions. \shu{is it enough to address these sets of related work? --> this circles back to the related work again, should change it}
%     \item Like caching solutions, our strategy provides the best-effort latency improvement for repeated reads, and its effectiveness is workload-dependent. \shu{Latency goals}
% \end{itemize}   

 % \begin{itemize}
 %    % \item Satellite-based systems often generate vast amounts of image data in one location and transmit it to other locations for analysis at different points in times. \accheng{is there a concrete example you have here? reads too general right now} \shu{Probably wants to stress that at some points, data is not needed anymore}
 % \end{itemize}
 
% \ion{If possible I'd first talk about the design space: decide where to store, decide when to cache, decide when to evict. Goal: provide good performance while minimizing the cost in a multi-cloud environment.}

% Essential to these modern cloud-native applications are object store services, which serve as the backbone for reliable, available, and affordable data storage in the cloud. However, existing services such as Amazon S3, Google Cloud Storage (GCS), and Azure Blob Storage typically operate within a single region or cloud, presenting challenges in a multi-region, multi-cloud environment. 
% \begin{itemize}
%     \item 
%     % \natacha{Two separate points here? Geo distribution does not reduce vendor lock-in?}
%     \item . 
%     % An m5.8x large instance costs only \$0.22 in AWS Asia Pacific (Melbourne) region, which is 5$\times$ more expensive than AWS South America region. \accheng{I would add some specific examples and / or actual numbers to make the problem more concrete}
% \end{itemize}

% Object stores, for example, Amazon S3, Google Cloud Storage (GCS), and Azure Blob Storage, are serving as the backbone for data storage for cloud-native applications. \shu{Cost-efficient storage}
% \begin{enumerate}
%     \item They provide scalable, reliable, and cost-efficient storage solutions, offering easy access to vast amounts of unstructured data through REST APIs.
% \end{enumerate}


% \danny{right around here we should present object stores and explain that they are our focus. We need to explain that:
% 1. Object store serve as the back bone for storage for most modern cloud native applications.
% 2. Object store give a REST API for writing immutable objects. They provide highly reliable, available and relatively cheap storage. 
% 3. Our work focuses on using object stores across multi-cloud and multi-regions.}

% Today, services such as Amazon S3, Google Cloud Storage, and Azure Blob Storage form the foundation of data storage for most modern cloud-native applications \cite{}. They provide highly reliable, available, and cheap storage for large amount of data. However, these services typically do not offer intelligent geo-distribution of data that spans multiple regions and cloud providers.

% These cloud-native applications rely heavily on services like Amazon S3, Google Cloud Storage, and Azure Blob Storage for reliable, available, and affordable data storage. However, these services lack intelligent geo-distribution across multiple regions and cloud providers, making data mangement highly complex and expensive in multi-region and cloud setup.
% However, managing data across different regions and clouds can be highly expensive. 
% users often face the daunting task of navigating different storage and network options to determine data placement.


% Moreover, the cost of storage can vary up to 2$\times$ depending on the storage locations.

% \begin{enumerate}
%     \item Centralizing data in a single cloud region may seem straightforward and minimize storage costs. Yet, it increases data egress costs and slows down access speeds for geo-distributed accesses. 
%     \begin{enumerate}
%         \item Transferring data across regions costs \$0.01 - \$0.19 per GB in the same cloud.  Moving data across cloud providers incurs even higher costs, ranging from \$0.08 to \$0.23 per GB. \cite{cloudcast} \shu{Transform this into full text, a bit hard to follow, English text; operationally straightforward, and minimize storage cost. But when considering data access, can be up to 8x cost increase 0.08 to 0.01}
%     \end{enumerate}
%     \item On the other hand, replicating data across multiple locations improves access speeds and reduces data transfer costs, yet it also elevates storage costs over time. 
%     \begin{enumerate}
%         \item For example, maintaining 500 GB of data across 10 AWS regions using standard S3 storage costs could average \$115 per month. Moreover, the cost of storage can vary up to 2$\times$ depending on the storage locations. \accheng{same comment as above, add some numbers to show the magnitude of the problem} \shu{is this number a bit too small?}
%     \end{enumerate}
% \end{enumerate}
 % \natacha{Trying to both talk about multi region and multicloud at the same time feels a bit confusing at times. Could you start with one (or the other), and briefly say that many of the same concerns apply to the second?}
 % These challenges underscore the need for a multi-cloud storage solution that can navigate this complexity. However, developing such a system is particularly challenging because of the inherent unpredictability of multi-cloud workloads. 
 % \natacha{The arguments that you're making below seem to strongly argue that workloads are geo-distributed or multicloud, but they don't necessarily make the point that workloads are "unpredictable"? Why not just say that they are geo-distributed and accesses change over time? (your examples are great exmaples of geo-distirubution)}

% The data placement problem is more challenging due to the diversity of access patterns for geo-distributed workloads. It is often hard to predict the location, frequency, and recency of workload operations.

==> sections/2_background.tex <==
\section{Background}
\label{s:background}

    

We first provide an overview of the pricing models and workload variability in the cloud to place our cost-optimized replication and eviction policies in context of multi-cloud and multi-region environments. 
% , which involves deciding (i) When and where to store or create object replicas in each region and (ii) When to evict object replicas from each region,
% We also discuss framing latency considerations into our setup in Section\ref{sec:latency}. \shu{shall we include this sentence if we have not done much?} 


\subsection{Cloud Pricing Models}
Cloud pricing consists of data storage, network, and operational charges \cite{gcp-pricing}. Most cloud vendors charge storage per GB per month based on the geographic region, provider, and storage class. For example, standard storage in \textit{gcp:southamerica-east1} costs $1.75\times$ more than S3 standard storage in \textit{aws:us-east-1}. The cloud provider also charges network (egress) costs based on the volume of data moved out of a particular cloud region \cite{aws-pricing}. This can differ by up to 15$\times$ within the same cloud and 19$\times$ between different clouds. Operations made to the cloud storage service are also charged: this cost is usually much cheaper than storage and network charges, with an average of 0.04 cents per thousand requests. Thus, we will mainly consider storage and network pricing in our discussion. 
% \shu{wordings ok?} Navigating various price offerings across regions and clouds to decide on data replication is often complex. \joey{This last sentence sort of feels out of place (starting a new thought at the end of a paragraph).}
% \newline
% Operations made to the cloud storage service are also charged: this cost is usually much cheaper than storage and network charges, with an average of 0.04 cents per thousand requests. 

\subsection{Workload Variability}
Cloud object stores exhibit diverse access patterns in terms of object size, access frequency, and burstiness \cite{6546109}. For instance, IBM object store traces (details in Section~\ref{eval:trace}) show a wide range of object sizes, from small ($<$1KB) to medium (1MB–1GB), and occasionally large (>1GB). Access frequencies can vary significantly, with some objects being one-hit wonders, while others experience cold (1-10), warm (10-100), hot (100-1000), or even super hot (>1000) accesses. Access patterns can also fluctuate: some traces show repeated reads early on, while others have a more uniform distribution. Recency is another critical factor, with intervals between accesses from hours to months. These variations make it difficult for a single simple policy to work cost-effectively across workloads.

% Cloud object stores often demonstrate diverse access patterns regarding object sizes, access frequencies, recency of accesses, and burstiness of accesses\cite{6546109}. Across IBM object store traces (detail in Section~\ref{eval:trace}), object sizes range from predominantly predominantly tiny ($<$1KB) to medium (1MB–1GB) or even large (>1GB) in some traces. Access frequencies also differ widely: workloads can have one-hit wonders, cold (1-10), warm (10-100), hot (100-1000), and even super hot (>1000) accesses, sometimes with a mix of them spread across objects.  Burstiness patterns vary, with certain traces having repeated reads appearing mainly at the beginning half of the trace, whereas others might have a more uniform distribution. Recency also plays a key role: some access intervals span within a few hours, while others span across days or months. These patterns impact the end-to-end placement costs and often make manual placement and eviction hard to be fully cost-effective. 


% We consider two modes of operation for object replication and eviction. First, there is the \textbf{\textit{Fixed Base}} mode, where each object has a fixed base (primary) storage region in which its replica never gets removed. Additional replicas may be created or removed in other regions as needed. Second, the \textbf{\textit{Free Placement}} mode allows for dynamic placement of replicas in any cloud region. The only requirement is that at least one replica is always present. \shu{in following section: say \sys allow configuring fixed base region that never gets evict, etc.}
% \shu{This section reads awkward here}
% The management of multi-cloud storage lies in deciding (i) When and where to store or create object replicas in each region and (ii) When to remove object replicas from each region, according to the workloads. 
% \newline 
% \textbf{Cost Objective} These design questions mimic the tradi tional caching paradigm, where decisions on replication and eviction are made in the cache based on access patterns. However, unlike traditional caches like CDNs, which are mostly latency-driven\cite{ms-cdn-paper, cdn-latency-aware}, object stores have unlimited capacity but incur costs based on usage (charged per GB per month). Therefore, in a multi-cloud environment, the placement policy must carefully balance two key expenses: the storage cost incurred for maintaining replicas and the network egress cost for fetching data from a remote region in the event of a cache miss. Unlike latency-driven systems such as CDNs, the focus here is minimizing these costs. We ignore operational costs typically negligible for this analysis and aim to optimize the total cost incurred from storage and network egress across regions and clouds.


% However, object stores differ from traditional caches since they have unlimited capacity but are charged by usage (per GB per month). Thus, a multi-cloud object store placement policy needs to carefully balance the storage expenses of using a cloud object store as a cache and the network egress expenses to fetch from the other region in case of a cache miss, compared to traditional caches like CDNs, which are mostly latency-driven\cite{ms-cdn-paper, cdn-latency-aware}. 
% \newline

% \newline 

% \subsubsection{System Design} To build a multi-cloud storage system, we need to design \shu{??}
% Traditional cache eviction policies are largely latency-driven, focusing on maintaining frequently accessed items to reduce miss rates and the associated time penalties. However, the context of cloud-based object stores introduces a critical additional dimension: cost. Cloud providers typically charge users based on the amount of data stored, measured in cost per gigabyte (\$/GB). This pricing model shifts the focus of eviction strategies from managing space and latency towards optimizing cost. 

% \subsection{Toy Example}
% \shu{Will it be helpful to have some sort of toy example demonstration here?}

% \subsection{\sys Overview}
% We first describe \sys placement policies in Section
% ~\ref{s:policies}.

% \subsubsection{A motivating example} An example of the challenges that workloads can pose for eviction can be seen in trace 009. It consists of bursts of GETS to the same object. Each burst consists of 2-8 GETs in sequence with less than 10 minutes between adjacent GETs. After the burst this object is never accessed again and the trace moves on to a different object. 
% Methods trying to learn this pattern for each object separately (e.g. \cite{tokeep2014, EWMA}) are bound to fail as will methods that assume the objects are accessed in a Poisson like distribution \cite{tokeep2014, TTLbasedCC2019}. The only hope is to observe this pattern at a bucket level and learn from it. Our challenge is to find a method that collects succinct yet useful information about the workload at a wide scope and devise an eviction strategy according to it. Our method ends up choosing a TTL of around 10 minutes for the entire trace which ensures the local replica will remain available as long as the burst is ongoing, but will be evict shortly after. 
% \subsection{Questions}
% \begin{enumerate}
%     \item Move TTL-based eviction from S3.2.1 discussion here?
%     \item Move the S3.3.1 discussion here about storage and network cost? 
%     \item Shall we use two-site as an introductory example here, or introduce high-level overview from 3.2.2 in this section?
% \end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \subsection{Key Questions}
% In light of the outlined challenges, the following questions become central to our problem setup:

% \begin{enumerate}
% \item Where should data be written?
% \item From which locations should data be read? 
% \item When to cache? 
% \item When should the cache be cleared? 
% \item How to maintain the consistency model (cache coherence) across cached copies? 
% \end{enumerate}

%%%%%%%%%%%%%
% Effective management of data across diverse cloud providers presents several challenges. These challenges are rooted in the variability of workloads and the inherent heterogeneity of cloud services. 

% \shu{Describe the design space: have copies of reads, introduce consistency issues to be addressed for multiple reads}

% \shu{Model monthly trace: don't have data, could assume IBM workloads stay as it is; do the simulation (and tell how the simulation is done), make this up, i.e. how quickly a particularly key dies; randomly sample subset of keys and rename them (every week sample 10\% of the keys), cloud workloads, create a new key (rename of the key), scheme to justify (i.e. 10\% of the rewrite, or 15\% rewrite rate, how does that change the workloads). Start the section of: don't have annual workloads, simulate the workloads have changing access patterns}




==> sections/2_background_outline.tex <==
\section{S2 and S3 outline}

==> sections/3_overview_scratch.tex <==
\newpage
\section{\sys Placement Policies} \label{s:policies}
This section outlines \sys's cost-optimized replication and eviction policies.


\subsection{On-Demand Replication Policy}
\sys operates with an on-demand principal, deploying a simple \textit{write-local} policy for data storage and a \textit{read-driven} policy for data replication. For data storage, \sys stores data in the region where the write request originates. This minimizes write latency and reduces egress costs for write operations, ensuring data is immediately available in the local region. In the fixed base mode, we set the base region of the object to the initial write location. Consecutive write to the objects creates a new object with an updated version in its write location, where versioning is managed by \sys control plane (see Section~\ref{s:arch-control-plane}). \newline 
\textbf{Replicate on Read} 
Upon read request, \sys selects the cheapest region where the replica resides to retrieve the data and creates a local replica to optimize future reads. 
This method reduces future egress costs and is coupled with a replica eviction policy described in Section~\ref{s:evict} to keep storage costs in check. 
Replicate-on-read contrasts with proactive replicate-on-write methods used in AWS Multi-Region bucket and SPANStore \cite{aws-access-point, spanstore}, which pushes all data to a predicted set of regions upon write operations. Unless the prediction is very accurate, such a model can lead to high egress costs and storage charges (Section~\ref{s:eval}). 
 % and the workload does not change significantly over time



\subsection{\sys Replica Eviction Policy}\label{s:evict}

\subsubsection{TTL-based eviction.}
\sys uses the following approach to manage replicas cost-effectively.
Each replica (i.e., a copy of an object) is assigned a TTL (Time To Live) value. If the replica is not accessed within this time frame, it will be evicted as long as it is not the sole remaining replica. 
In the fixed base mode, the replica is evicted as long as it is not in the base location.  

There are two popular methods of TTL-based eviction.
The first, often used in Content Delivery Networks (CDNs)~\cite{ttl-cdn}, invalidates a cached object after TTL to ensure data is not stale. This happens no matter how frequently an object is accessed during the TTL time. 
In the second approach which \sys uses, TTL is reset every time the object is accessed. This method is geared towards reducing network costs, not evicting frequently accessed objects.

The overall eviction policy is straightforward: \sys periodically scans over all objects and evicts ones 
that have not been accessed within $\tev$ time, as long as they are not the sole replica of the object.
The crux of this method is how to set this TTL for various object replicas. \sys eviction policy for object $o$ at region $R$ is as follows: 
%\remove{
\[ Policy(o, R) = \left\{
  \begin{array}{ll}
    \text{evict :} &  \text{time since last access} > \tev(o, R) \\
    & \ \& \text{ not sole copy}\\
    \text{keep :} &  \text{otherwise}
  \end{array}
\right.
\]
%}
%\michael{The fact that the TTL is per object, per region needs to be explained.  This is not obvious. This also seems inconsistent with the paragraph below which says it defined for a pair of regions in a directed graph.}

\subsubsection{Choosing adaptive TTLs.} % - high-level overview

\begin{figure}
    \centering
    \includegraphics[width=.85\linewidth]{figures/TTL_figure.pdf}
    % https://docs.google.com/presentation/d/1c8WAbqHgEdVLjG0NdVunE_q2ph9oxC1v_7ilpXN8q-g/edit#slide=id.g2cc2bb5414f_0_126
    \vspace{-1em} % Adjust this value as needed
    \caption{The multi-cloud setting as a directed graph with a TTL assigned per each directed edge.}
    \label{fig:ttl}
\end{figure}

We tackle the multi-region setting by breaking the problem into a pairwise problem and setting the TTL for each pair of source target sites. Namely, we view the multi-region setting as a fully directed graph where each node is a region, and for each directed edge, we compute a TTL corresponding to this edge (as shown in Figure~\ref{fig:ttl}).
The TTL assigned to an object at a specific region is then deduced from the TTLs of the edges directed at this region. 
We denote $\tev(R_i,R_j)$ as the chosen TTL value for the edge from region $R_i$ to region $R_j$ and $\tev(o, R_j)$ as the TTL assigned to an object $o$ at region $R_j$. The eviction TTL of an object depends on the relevant regions that hold a replica of the object $o$. The TTL of the object at each region is then chosen to be the minimal TTL of edges from all the relevant regions.  Namely: 
$$\tev(o, R_j)= \min_{i | o \in R_i} \tev(R_i,R_j) $$

The TTL of an edge is assigned as a function of the incoming network cost, so the cheaper the cost, the lower the TTL. Since we use the cheapest available source in case of a cache miss, this corresponds to the minimal TTL.  

Our method for calculating an edge's TTL values is inspired by solving a two-region caching problem with a source and a target. To compute the TTL for each edge, we take the storage cost at the target, the network cost from the source to the target, and a statistics histogram of the workload in each region as input. 
This final component is what makes our choice of TTLs adaptive. As time goes by, we learn from the access patterns of the workloads and change the associated TTLs accordingly.
% assuming bucket-level statistics have some stability over time and can be expected to maintain their behavior in the future (at least in the near future). 
% \shu{need more algorithm support} We show evidence that this approach is effective in Section~\ref{sec:future}. 
% \accheng{suggest to remove, repeated content: TTLs are adapted periodically as statistics are accumulated; hence, this solution can also adapt to changes in workload behavior.} % \michael{There is also an implicit assumption that there is similarity in the access pattern within a bucket.  Do we have evidence for this?  How sensitive is our approach to this assumption, e.g., if we partition the objects in a bucket into multiple equivalence sets wrt access patter.}\danny{We have some evidence but all in the 1-week trace. Is it worth bringing it up?}


%The TTL of an object at a target is defined as the lowest TTL of all the potential sources for this object. Namely the minimum TTL of all the edges from regions that hold a replica of this specific object. This is described more formally in Section~\ref{s:multi}.

%In the following we describe how we set a TTL for an edge.  
%The eviction policy in \sys is a critical component for effective data management. This policy is responsible for making informed decisions on whether to retain or evict data objects in a specific region. The rationale behind implementing an eviction policy is to balance the trade-offs between cost and performance. We want to ensure high availability and quick access to data, but also want to minimize unnecessary storage and egress expenses by intelligently decides what data should stay.

% users can choose to pay additional costs for improved performance. 

\subsection{The Two-Region, Base and Cache Problem}
\label{s:problem-twosite}

As mentioned before, we approach the two-site TTL problem as a caching problem between a source base site and a target cache site. We start by presenting a clairvoyant algorithm that serves as a baseline and introduces concepts to build up to our method.  
% Yet our setting  differs from traditional cache settings in the following ways:
% \paragraph{Unlimited Cache Size} Traditional caching approaches typically manage a fixed-size cache, where the decision to evict items is driven by the need to make room for new ones when the cache is exhausted. The decision on which items to evict typically involves comparing objects against each other to determine which are the least likely to be needed soon \cite{}.
% In contrast, our setting assumes an unlimited cache size - namely, the local object store is considered to be large enough to host all of the objects accessed in a region. 
% As such, our system can evaluate each object independently instead of comparing them to decide which to remove.
% \paragraph{Cost Objective} Traditional cache eviction policies are largely latency-driven, focusing on maintaining frequently accessed items to reduce miss rates and the associated time penalties. However, the context of cloud-based object stores introduces a critical additional dimension: cost. 

% Cloud providers typically charge users based on the amount of data stored, measured in cost per gigabyte (\$/GB). This pricing model shifts the focus of eviction strategies from managing space and latency towards optimizing cost, i.e. storage expenses. 


\subsubsection{The Clairvoyant Greedy Policy and Break Even Time}
\label{sec:clairvoyant}
We measure ourselves against a policy that is given access to an {\em oracle} that knows exactly when an object will be read in the future (if at all). This is akin to Belady cache eviction algorithm \cite{belady} but adapted to our problem setting. 
This clairvoyant algorithm is the optimal policy for the case of a two-site base and cache setting. 
To understand this policy, we define the following notations: 

We denote $S$ as the storage cost (\textbf{\$/GB*Month}) in the baseregion and $N$ as the egress cost (\textbf{\$/GB}) for moving an item over the network between the base region and the cache region.
In a multi-region setting, these parameters may change between every pair of regions, but for this discussion, we consider only two sites: base and cache. 
A read miss means that an object needs to be brought over the network, and this cost would amount to $\text{Size}(o) \times N$\footnote{For simplicity, we are ignoring the associated operation costs (e.g., cost for every PUT or GET) that are typically lower than the storage and egress costs.}. 

A key parameter in the clairvoyant strategy is the {\em break-even time}. This is the duration in which the cost of storing an object equals the cost of evicting it and fetching it again across the network (i.e., the storage cost equals the egress cost). We denote this as $\teven$, where:  
\begin{equation}
   T_{\text{even}} =  N  / S \label{eqn:teven}
\end{equation}

For example, we have $\text{Cost}_\text{storage} = \$0.026 \text{ per GB per month}$ for \texttt{aws:us-west1} and $\text{Cost}_\text{egress} = \$0.02 \text{ per GB}$ between \texttt{aws:us-east1} and \texttt{aws:us-west1}. Thus,  
    $T_{\text{even}} \approx 0.77 \text{ months}$ for the edge between these two regions.\footnote{Prices taken in Sept. 2023.}

Since the eviction of one object is independent of others, it is clear that the best one can do is cache an object as long as the cost of caching it is lower than the cost of bringing it again over the network. Every time an object is read, the clairvoyant policy accesses an oracle that returns the time duration until this object will next be read. We denote $T_{\text{next}}(o,i)$ as the time between the $i^{th}$ and ${i+1}$ reads of object $o$. The strategy then compares this with the break-even time $T_{\text{even}}$ and decides whether to evict the object. In summary, the clairvoyant policy upon the $i^{th}$ access to object $o$ is as follows:
\vspace{-0.2em}
\[Clairvoyant(o,i) = \left\{
  \begin{array}{lr}
    \text{evict :} &  T_{\text{next}}(o,i) > T_{\text{even}}\\
%        & \ \& \text{ not sole copy}\\
    \text{keep :} &  T_{\text{next}}(o,i) \leq T_{\text{even}}
  \end{array}
\right.
\]

\remove{
\begin{equation}
\text{Cost} = \text{storage cost} = ( T_{\text{next}}(o,r) ) \times \text{Size}(o) \times \text{Cost}\_\text{storage}(r)
\end{equation}

If an item is evicted, then its egress cost is paid for the next access,

\begin{equation}
\text{Cost} = \text{next access cost} = \text{Size}(o) \times \left( \frac{1}{m} \right) \sum_{j=1}^{m} \text{Cost}_\text{egress}(r_j, r)
\end{equation}

The break-even point is when the cost of evicting an object would be the same as storing it. It is defined by:  
\begin{equation}
   T_{\text{even}} =  \text{Cost}_\text{egress} / \text{Cost}_\text{storage}(r)
\end{equation}
}
\subsubsection{The $\teven$ Policy}
Before explaining our actual policy, we first consider another baseline: the simple policy that sets $\tev = \teven$, termed the $\teven$-policy. 
This simple policy has the following properties:
% makes sense because of the two facts relevant to the two-site caching problem. 
\begin{enumerate}
    \item The cost of the $\teven$-policy is at most double that of the clairvoyant policy.
    \item $\forall$ eviction policy $\exists$ a workload for which the policy costs twice as much as the clairvoyant policy. 
\end{enumerate}

% We provide the proofs for these two properties in the Appendix A. 
% \sum_{o, i| \tnext(o,i)
\paragraph{Proof.} The cost per byte for a single object in the optimal policy under this setup is:
$$ \sum_{i| \tnext(i) \leq \teven} \tnext(i) \cdot S + \sum_{i| \tnext(i) > \teven} N  + N $$
The last $N$ is the cost of the initial GET, whereas there is no cost after the last get as the object is evicted. The cost of the $\teven$-policy policy is:
$$ \sum_{i| \tnext(i) \leq \teven} \tnext(i) \cdot S + \sum_{i| \tnext(i) > \teven} 2N + 2N$$
The last $2N$ includes the cost of the initial GET and the cost of keeping the object around after the last GET. The first part is identical, whereas the second part is exactly double that of the optimal cost. 
Namely, the cost of the $\teven$ policy is bounded by $2\times$ that of the optimal algorithm. On the other hand we claim that for every eviction strategy there exists an (adversarially chosen) workload for which the cost amount to more than twice that of the optimal strategy. 
This can be shown for each object separately. It starts by reading the object once (therefore putting it in the cache). If the eviction policy P decides to evict the object after more than $\teven$ time, then the workload never asks for this object again. 
In such a case, the optimal strategy cost would be $N$ (just for the first GET), whereas the cost for policy $P$ would be greater than $N + \teven \cdot S = 2N$. 


 If, on the other hand, P decides to evict the object earlier, at time $t < \teven$, then the workload submits a GET after $t + \varepsilon$ time, subject to $t + \varepsilon<\teven$. 
 The $\co$ in this case is $N+(t+\varepsilon)\cdot S$ whereas for $\cp$ is $2N+t\cdot S$.
 Since the object is in the cache again, we recursively continue.
 After $k$ iterations we have $\co = N+(\sum (t_i+\varepsilon))S$ whereas $\cp = (k+1)N + (\sum t)S$.
 
 The difference between them is  $\cp - \co = kN + k\varepsilon$ since $\co <(k+1)N$ then choose $k$ to be large enough so that $k \varepsilon> N$ which will cause $\cp-\co > \co$ and give us a ratio $\geq 2$.  

These two properties demonstrate that if nothing is known apriori about the workload, then the $\teven$-policy is the safest strategy one could hope for.
However, distributions are not chosen adversarially in reality. Quite a bit can be learned about workload distribution, which should be used to reduce costs. 
Our designed eviction strategy learns the access distribution over time and tries to choose an optimal $\tev$ for the workload at hand. 
 
\subsubsection{Adaptive TTL}\label{s:tevict}
Our method chooses the $\tev$ at the bucket level. Bucket granularity is often a good indicator of access patterns, and the distribution of accesses in buckets remains more or less stable over time for most workloads. We find that statistics at an object level may be highly misleading and prohibitively expensive \shu{provide evidence: the motivating example should probably be moved here}. 
% \accheng{do we have evidence?}
%\michael{do we have evidence to support these assertions?  Prohibitively expensive is likely easy to support but what about the other aspects?}
The main statistic we use to adapt the eviction time is the time distribution between accesses of an object. In other words, what is the distribution of $\tnext$ in a bucket at a specific region?  
We collect a weighted histogram of various values that $\tnext$ can have. Each cell in the histogram corresponds to a time range, %The cells are chosen at a discrete  granularity (for example, each cell can refer to a 1 hour time window). 
and the weight in each cell in this histogram corresponds to the total size of all object GETs with a $\tnext$ in the cell's time range. Namely, how many bytes were re-read at a time difference that falls in the range of the cell. 
Note that such a histogram is collected per region and per bucket. 

\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{ m{7.5em}  m{16em}}
          \toprule
          {\bf Parameter} & {\bf Description}  \\
        %   \hline
            \midrule
          $range(j)$ & Time interval of the $j^{th}$ cell \\%\hline
      $t(j)$ & Maximum time in $range(j)$ \\%\hline
      $\widehat{t}(j)$ & Mean time in $range(j)$ \\%\hline
      $hist(j)$ & Bytes re-read after time $t \in range(j)$ \\%\hline
      $last(j)$ & Bytes not read in $t \in range(j)$ \\%\hline
      \bottomrule
      \end{tabular}
  }
  \vspace{0.5em}
    \caption{Eviction parameters.}
    \label{tab:notations}
\end{table}


We define our notation in Table~\ref{tab:notations}. According to these, the value in a histogram cell is:
$$ hist(j)  = \sum_{o, i| \tnext(o,i) \in range(j)} size(o)$$
The histogram accounts for all re-reads in the workload. However, it does not account for what happens to objects after their last access. 
% At every point in time, every object stored in a region has a time that has passed since its last access. \accheng{prev sentence unclear} 
We calculate a histogram called $last$ to account for the time of policy evaluation and latest access.
% We count the weight of these in an additional histogram called $last$.    
The crux of our method is that, given the histograms and a TTL value, we can compute the expected cost for this region.  
For each value, the expected cost for the $\tev$ is calculated as follows \shu{expected cost: add in base cost for initial reads}: 
% cost of re-read, the histogram does not include the initial reads; the histogram always talk about the interval between two reads
\begin{align*}
ExpectedCost(\tev) =&  
\sum_{\substack{j \in hist \\ t(j) \leq \tev}} hist(j)\cdot \widehat{t}(j) \cdot S \\
&+ \sum_{\substack{j \in hist \\ t(j) > \tev}} hist(j) \cdot (N+\tev \cdot S) \\
&+ \sum_{\substack{j \in last}}  last(j) \cdot \tev \cdot S
\end{align*}
\remove{
\begin{align*}
ExpectedCost(\tev) =  
\sum_{\substack{j \in hist \\ t(j) \leq \tev}} (hist(j) + last(j))\cdot t(j) \cdot S \\
+ \sum_{\substack{j \in hist \\ t(j) > \tev}} hist(j) \cdot (N+\tev \cdot S) + last(j) \cdot \tev \cdot S
\end{align*}
}
%\begin{align*}
%ExpectedCost(\tev) =  
%\sum_{\substack{j \in histogram \\ t(j) \leq \tev}} (hist(j) last(j))\cdot t(j) \cdot S / sum_{hist} \\
%+ \sum_{\substack{j \in histogram \\ t(j) > \tev}} (hist(j) + last(j)) \cdot (\tev \cdot S + N)/sum_{hist} \\
%\end{align*}
The first line accounts for hits -- objects that are re-read and exist in the region. The second accounts for misses -- objects that are evicted and then brought back in with network cost, and the third line accounts for storage costs of object instances that have not yet been re-read.
We now iterate all possible values of $\tev$ at the same granularity as the histogram. % where $0 \leq \tev \leq \teven$. 
Since we aim to minimize total cost, we choose the value $\tev$ with the lowest expected cost. 

The expected cost and the best TTL are influenced by the histogram of the specific workload, the network and storage costs, and the value of $\teven$ which is a ratio of these costs.  
Figure~\ref{fig:costhist} shows an example of the expected cost as a function of TTL for one of the SNIA traces with different pricing choices. A lower value of $\teven$ indicates that storage costs are higher (relative to the network costs) and means that shorter TTLs would fare better, as seen in the example.   
%\danny{I brought the figure back in here. I think it helps understand the policy and better shown here than in the evaluation section. It is simply an example.}

% \begin{figure}
%     \centering
%     \includegraphics[width=.85\linewidth]{figures/costhist029.png}

%     \vspace{-1em} % Adjust this value as needed
%     \caption{The expected cost as a function of TTL on Trace 029 with an hourly histogram. The dashed line represents the optimal (clairvoyant) policy cost, and the dot on each graph represents the minimal cost point.}
%     \label{fig:costhist}
% \end{figure}
% \vspace{-0.2em}

\paragraph{Histogram Size and Granularity}
The granularity of the histogram is directly related to our possible choices for setting the TTL. A more granular histogram gives us additional information and allows us to choose TTLs more accurately, achieving better cost savings. On the other hand, a large histogram burdens the memory and computation requirements of the system. Recall that the histogram should potentially cover a time duration of many months, yet at times, the best eviction policy calls for evicting objects within minutes or even seconds. 
To balance this tradeoff, we support a variable range to histogram cells, attempting to have high granularity for small TTL values and lower granularity for larger one. For the first minute, we use a per-second granularity (taking up 60 cells). Beyond that, we employ a logarithmic base granularity with a low base of $1.02$. This ensures that the time ratio between two consecutive potential TTL values is no more than 2\%. In turn, the difference in storage cost between two consecutive TTLs is also bounded at 2\% as the cost is linear in the time the replicas are stored. 
Using 740 cells at this log granularity covers $(1.02)^{740}$ minutes, which amounts to almost 2 years of time. An additional 60 cells cover the first minute, and we thus manage to cover nearly 2 years with an 800-cell histogram. 

In order to account for changing behavior over time, we opt to periodically start collecting a new histogram (while still keeping the previous histogram). Once the new histogram has a long enough history, the old histogram can be discarded. Our investigations indicate that the histogram should be longer than the $\teven$ time in order to be effective. 

\subsubsection{Latency Considerations}
\label{sec:latency}
Incorporating latency considerations in a cost-driven framework can be difficult. \shu{change this to latency SLOs and do ablation on it (simulation)}
Essentially, we need to put a price tag on object read performance. This price can vary depending on the application, the user, and the objects at hand. Nevertheless, we show that given a way to price performance, we can integrate it into our framework. 

% We consider two methods for price-latency considerations: the first is to add a price tag for cache misses, and the second puts a price on potential cache hits.

% \textbf{Pricing Misses.} This approach is also used in \cite{TTLbasedCC2019} to calculate the cost of a cache miss. In the framework above, we model the cost of a cache miss solely using the network egress cost associated with bringing the object over from a remote site. This can be generalized to also consider latency and model the price associated with waiting longer for objects. We focus on a cost for each {\em byte} read that is not in read locally (as opposed to pricing according to object misses). We incorporate this into our framework by replacing network cost (a per byte figure) with miss cost, which accounts for both the network cost and an additional monetary penalty for a read miss (also a per byte cost). 

%\michael{Since latency is often about time to first byte, which is independent of object size, can we justify a per byte charge other than it fits in better with the model?}

We show a potential method for price-latency considerations, i.e., to put a price on potential cache hits or to ask how much a customer is willing to pay for cache hits. Namely, if all things are equal, how much additional cost the user would be willing to pay for local latency and bandwidth? Say we denote this value as {\em user performance value}, denoted by $\uval$, a cost per byte.
We add this to the basic methodology of choosing a $\ttl$ as follows: After finding the value of $\ttl$ that achieves the lowest expected cost, check whether there is a higher $\ttl$ value for which the $\ uval$ bounds the average cost per additional hit. 

More formally, let $\ttl'$ stand for the eviction time, achieving the best expected cost. We choose the highest value $\ttl$ such that 
$$ \frac{ExpectedCost(\ttl) - ExpectedCost(\tev')}{\text{object byte count between $\tev$ and $\tev'$}} \leq \uval$$ 

For each cached object, the user pays the storage for this cache until the time $T$ of the next read or eviction. This amounts to $T \times \text{Size}(o) \times S$. 


% \accheng{forward reference eval?}

% Latency consideration section 
% \subsubsection{Latency Considerations}\label{s:latency}
% Incorporating latency considerations in a cost-driven framework can be difficult. 
% Essentially, we need to put a price tag on object read performance. This price can vary depending on the application, the user, and the objects at hand. Nevertheless, we show that given a way to price performance, we can integrate it into our framework. 
% We consider two methods for price-latency considerations: the first is to add a price tag for cache misses, and the second puts a price on potential cache hits. %\michael{This section hit me out of the blue. In the intro we should include a sentence about extending model to explicitly include latency via translating into \$ cost.}

% \textbf{Pricing Misses.} This approach is also used in \cite{TTLbasedCC2019} to calculate the cost of a cache miss. In the framework above, we model the cost of a cache miss solely using the network egress cost associated with bringing the object over from a remote site. This can be generalized to also consider latency and model the price associated with waiting longer for objects. We focus on a cost for each {\em byte} read that is not in read locally (as opposed to pricing according to object misses). We incorporate this into our framework by replacing network cost (a per byte figure) with miss cost, which accounts for both the network cost and an additional monetary penalty for a read miss (also a per byte cost). %\michael{Since latency is often about time to first byte, which is independent of object size, can we justify a per byte charge other than it fits in better with the model?}

% \textbf{Pricing Hits.}
% An alternative approach is to ask how much a customer is willing to pay for cache hits. Namely, if all things are equal, how much additional cost the user would be willing to pay for local latency and bandwidth? Given such a parameter, we show in Appendix B how our framework can be tweaked to account for this additional pricing consideration.

% Note that we considered per-byte pricing in both of the above approaches, which work well with the rest of our framework in which pricing is dominated by object size. It also avoids a need to differentiate between objects according to their size as part of the eviction policy. For example, if the main goal was object cache hits (irrespective of the object size), then it is obvious that achieving cache hits for small objects is cheaper than for large objects. This would then suggest varying the TTL according to object size, which we leave for future work.



%\shu{Take 24 hour T\_even, make some storage cost (price of hit is 0.056), same experiments --> pricing misses is the exact same experiments, makeup whatever we want on this, make the price of miss much lower than the network price, and can fit it into Teven, add the price of miss into the network cost; pricing hits are more problematic}

==> sections/4_1_fault_tolerance.tex <==
\section{Fault Tolerance}
\label{s:ft}
The cost of abstracting away location details of data placement is to have another layer of indirection keeping track of the logical to physical location mappings. The metadata layer needs to be consulted for every single access (read, write). This might be a related paper: https://dl.acm.org/doi/pdf/10.1145/3552326.3587443 


% \subsection{Model}

% \sys should provide availability and resiliency that are on par with a solution that does not use \sys but rather places objects in separate buckets in different regions or clouds. 
% In such a solution, a client will have access to all objects as long as the corresponding object storage is up and there is network connectivity to the respective region or cloud. In other words, a network failure between two clouds may render objects residing solely on the remote cloud inaccessible but should not affect the availability of local objects. 

% As a result, the location catalog cannot be centralized in a single region because a connectivity failure with this region would render all objects inaccessible (assuming that using solely the information in the underlying object stores would not be performant enough for standard operation).  
% A possible solution is to hold a local copy of the location database in each cloud. Updates to each database should be synchronized with the other database instances.
% \gvernik{Currently DB is located in the metadata server. Do you suggest to keep metadata server in each region? If so, that means each region will need to keep a dedicated VM for this - this will be very expensive to keep such server in each region.}
% In order to maintain the availability model defined above it is critical that a DB will be up to date about its local objects.  So upon writing an object, the DB at the region in which the object was written should be updated first. This information should then be propagated to the other DB instances. 
% \gvernik{if region local metadata server is down, but region still available, then SkyStore should continue to provide access to the data in this region. That means local DB need to backup to to other regions in such way that there is no data loss. This is not strait forward to achieve and since there are many local DB servers, the entire fault tolerance architecture will be too complicated. 
% I think for this paper is better keep a single MD server and explain how we sync it to other regions for the fault tolerance, etc. and you can mention that future work will consider local DB servers or some other DB sharding}

% Lookup and listing then become tricky as remote object may not yet appear in the local database instance.
% There are a number of ways to approach this: 
% \begin{enumerate}
% \item chuck it up to eventual consistency – ones the sync finishes everything will be fine. 
% \item First look up locally and if an object is not there then venture to remote DBs (potentially scanning all of them).
% \item Hold for each object a hash based authoritative location and make sure to sync with that location ASAP. This will help with lookup, less for listing. It also needs to overcome temporary timeout of an authoritative region. ( Should authoritative location be at a bucket or sub-bucket granularity?)
% \end{enumerate}

% Other options would include looking into distributed DBs (e.g.  CockroachDB). However, in CAP theorem terms we must use one that provides Availability at all cost (CockroacDB for instance ensures consistency over availability).    

\shu{A section to discuss the failure mode; need to have a separate section on this, what is the model }

\gvernik{I think it should be one bucket DB that contains metadata of all buckets, their physical locations, etc. And another DB should contain all object operations. Then we can have different policies how to protect them. At later point we can shard the objects DB to get better performance. Having per-bucket MD database might not be optimal, as with "virtual bucket" approach  users might create a single bucket and upload / link millions of objects into this bucket}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/metadata_server.png}
%     \caption{Cost}
% \end{figure}

Primary-secondary approach is a popular paradigm implemented by various distributed systems like HDFS [] to ensure fault tolerance and availability.  With this approach, the primary server handles all operations, while the secondary server is either updated periodically or always in full sync with the primary server. 

The straightforward approach is to update both primary and the secondary server for every operation, making both servers fully synchronized. Although this might not be optimal and affect the overall performance of the system, the benefit is the secondary server is always consistent with the primary.  In case the primary server becomes unavailable, the system can switch to secondary right away and there is no data loss. 

A different approach when the secondary server is periodically updated from the primary. While this reduces overload on the system, the main drawback is that in case of primary server failure, the secondary will have state based on the last sync and even with data recovery, still may result in some data loss. 

To address the fault tolerance of the metadata server in \sys, we decided to follow the hybrid version of the primary-secondary approach as follows. \sys will initiate a primary metadata server $P$ and a backup metadata server $A1$ in the same cloud region. In addition, \sys will initiate another metadata backup server $B1$, in a different region. Metadata servers $P$ and $A1$ will be in full sync inside a single region and thus maintain strong consistency between them. 
We configure PostgreSQL in the primary metadata server $P$ to synchronously replicate it's database to the secondary PostgreSQL metadata server $A1$ located in the same region.
Moreover, all bucket operations, like create or register bucket,  will be synchronously forwarded from $A1$ server into another region with $B1$ server. Once metadata servers fully process the requests, the primary metadata server will generate a response to the user. This ensures that if the primary metadata server is down, has network issues or other faults, \sys will continue to operate without disturbance by accessing secondary metadata server $A1$ located in the same region. 

This solution however does not cover the case when the entire cloud region is down and both primary and backup metadata servers located in that region become not available. To address this issue, \sys also keeps another metadata server $B1$ in a different region that is updated by $A1$ server. As opposed to $P$ and $A1$ that are updated synchronously for all operations, the $B1$ server is updated asynchronously for object related operations and synchronously for bucket related operations. This will assure that $B1$ is always aware what virtual buckets exists in the \sys. [to-do: update pic. In addition, $B1$ server will also dump its local metadata DB to the object storage bucket. ] The overall flow would be as shown in Fig. \ref{fig:metadata-backup}. 
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/backup_server.png}
    \caption{Metadata Backup}
    \label{fig:metadata-backup}
\end{figure}
In case the entire cloud region is down and both $P$ and $A1$ are not available, \sys will choose region $B$ as its primary region and choose $B1$ as a primary metadata server, which we name $P1$. To maintain fault tolerance of the $P1$, \sys will create a secondary metadata server $B2$ in the same region $B$ and create another metadata server $C1$ in a different region $C$. 
Similar to the previous semantics,  $B2$ will be synchronously updated by $P1$ for every operation. In addition metadata server $C$ will be updated synchronously by $B2$ for bucket related operations and updated asynchronously for object related operations.

$B1$ metadata server has the current state  of the \sys virtual buckets, but may not have the updated state of the object operations that were registered on the primary metadata server $P$. [will update soon ]


==> sections/5_method.tex <==
\section{Methodology} \label{s:method}


==> sections/6_evaluation.tex <==
\FloatBarrier
\section{Evaluation} \label{s:eval}



We compare \sys's cost-optimal replication policy with
other alternatives and answer the following questions: 
\begin{enumerate}[noitemsep=*,leftmargin=*]
    \item What are the cost savings in \sys from cost-optimal replication policy with two-region base and cache setting?
    \item How does \sys's cost-optimal replication policy adapt to multi-region and multi-cloud settings?
    \item How does \sys prototype perform in the real world with multiple clouds?
    \item What are the overheads and trade-offs in \sys?
\end{enumerate}



% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/nsdi/5_trace_new_analysis_14_65_78_79_95.pdf}
%     \caption{\textbf{Five Trace Analysis}: The frequency, size, recency, and distribution of GETs over time CDF of Trace 14, 65, 78, 79 and 95.}
%     \label{fig:5_trace_new_analysis}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=.65\linewidth]{figures/nsdi/trace_plot.pdf}
%     \caption{\textbf{Five Trace Analysis}: The PUTs and GETs ratio of Trace 14, 65, 78, 79 and 95. \shu{maybe less useful to keep this?}}
%     \label{fig:put_get_distribution}
% \end{figure}
\subsection{Workload Generation From Traces}  \label{s:workload-gen} 
% \shu{Ion: we are using this kind of base traces, and use these base traces to generate our workloads (by generalizing the traces in times, and across regions). Gives a head-up --> generate our workloads, extending the traces over time and over regions.}

We draw our experimental workloads from 98 IBM Object Store traces from the SNIA I/O Traces, Tools, and Analysis (IOTTA) repository~\cite{SNIA_TRACE}. Each trace represents a week of RESTful operations (e.g., GET, PUT, HEAD, DELETE) for a single bucket (one region) within the IBM object storage system, with additional metadata such as timestamps, object keys, and sizes ~\cite{LRUvsFIFO}. We pick five traces with distinct characteristics in recency, frequency, size, burstiness, and put and write distribution. We then use these base traces to generate our multi-region and multi-cloud workloads by expanding the traces over regions and times. We demonstrate our policy cost savings over these representative traces and show the complete results of 31 traces in Appendix~\ref{}. 
% \souj{All traces are just for a week?}
% \souj{Total of how many traces are in the repo?} \shu{Yes, look above}
% How do we pick traces? 


\textbf{Five-trace analysis.} Cloud object stores often demonstrate diverse access patterns in terms of object sizes, access frequencies, recency of accesses, and burstiness in accesses. We choose 5 out of 98 SNIA IBM Object Store traces which are diverse and representative of the workload patterns, as shown in Figure~\ref{fig:5_trace_new_analysis}. 

% \shu{Choose traces that exhibit the largest difference across these dimensions of object size, read and write ratios; have a table for these five traces, and show five columns on each dimension (5 traces, five dimensions, sub-columns; put the percentage)}

% Trace 15 (80\%), Trace 29 (56\%), Trace 78 (97\%), Trace 79 (40\%), Trace 65 (34\%),  between 1KB and 1MB.

\textit{Size} The Size CDF illustrates the distribution of objects across various traces. In Traces 29 and 65, 44\% and 31\% of the objects, respectively, are smaller than 1KB. In contrast, Traces 15, 78, and 79 have fewer than 0.5\% of their objects under 1KB. The majority of objects fall between 1KB and 1MB for Trace 15 (80\%), Trace 29 (56\%), and Trace 78 (97\%). For Traces 79 and 65, around 40\% and 34\% of objects, respectively, are within this range. In the large-size range (1MB to 1GB), more than 60\% of the objects in Trace 79 fall within this category. However, no objects in Trace 29 fall into this range, and the percentages are much lower for Trace 78 (2\%), Trace 15 (20\%), and Trace 65 (34\%).

% For Trace 14 and 78, 74\% and 97\% of objects are between 1KB and 1MB. Trace 65 has a more equal distribution (33\%) of objects below 1KB, between 1KB to 1MB, and larger than 1MB. While in Trace 79, more than 60\% of the objects are between 1MB and 1GB. \shu{Add more numbers in the same interval}

\textit{Access Frequency} The CDF of number of GET requests shows patterns in access frequency across the traces. Nearly half of the objects in Trace 15 are one-hit wonders, whereas the other traces have less than 20\% of objects with just one access. In the moderate frequency range (1-10 GETs), almost all objects in Trace 29 (98\%) fall into this category, with Trace 79 also showing a significant proportion (61\%). For higher frequency (10-100 GETs), over half of the objects in Trace 78 belong to this group, with 22\% in Traces 79 and 65. Traces 15 and 29 lack objects with more than 10 GETs. Trace 65 has 66.6\% of its objects accessed with even higher access frequency (100-1000 GETs), while Trace 78 only has 11\% and no other traces feature objects in this range.

% Trace 78 and Trace 65 have larger access frequency per object, where around 51\% of objects have between 10 to 100 GETs, and 67\% of objects have between 100 to 1000 GETs. 


\textit{Recency} The recency CDF illustrates the time between consecutive GET requests for each trace. In Traces 15 and 78, over 90\% of inter-arrival times are under one hour. In contrast, Traces 65 and 79 show about 10\% of GET intervals falling between one hour and one day. Trace 29 presents a different pattern, with approximately 80\% of recency values ranging from one hour to two days, and the remaining intervals exceeding two days.

\textit{Arrival Burstiness} We measure the fraction of GET requests over time to capture the burstiness in each trace. In Trace 78, a majority of objects (60\%) appear during the last two days (days 5 to 7), while the other traces show less than half in the same period. Trace 15 has an even distribution of accesses between the first four days and the final day, with no objects arriving between days 5 and 6. Traces 29, 65, and 79 exhibit nearly equal distribution of GETs across all days, with a noticeable spike on day 2, where 30\% of objects arrive in Traces 65 and 79.

\textit{Read and Write Ratio} We plot the number of PUTs and GETs in millions for each trace. As shown in the Figure~\ref{fig:5_trace_new_analysis}, Trace 65, 78, and 79 are read-dominated. Trace 15 and 29 are more write-heavy: around 42\% and 30\% of the accesses are write operations. Notably, Trace 29 is a large trace consists of more than 10 millions of requests compared to the others. 

% Trace 14 is a write-heavy workload, where 66\% of the operations are PUTs. Trace 95 is a read-and-write-balanced workload: around 59\% of the operations is the write operation, and 41\% of operations of the operations is read.


% For access frequency, the majority of objects in both Trace 06 and Trace 29 have fewer than 10 GETs, while
% more than 50\% of the objects in Trace 80 have more than 1,000 GETs. Lastly, the recency CDF reveals that Trace 36 typically features object accesses within a single day, in contrast to
% Trace 06, which displays a more distributed pattern with
% accesses extending beyond a week. In addition, in the multi-cloud settings, the provider locations of workload accesses add another variable to the equation. 

% For access frequency, the majority of objects in Trace 14, 20, and 89 have fewer than 10 GETs, while more than 50\% of the objects in Trace 36 has between 10 and 100 GETs, and more than half of the objects in Trace 65 has between 100 to 1000 GETs. The recency CDF reveals the duration distribution between consecutive GETs from each trace. For the GET that never sees any next GET, we count the interval as infinite. For example, Trace 14 shows close to 0\% of all consecutive GETs within 7 days, this means almost of all the traces objects are one-hit-wonder objects. The size CDF also shows the distribution of object sizes in each trace. For example, in trace 20, more than 50\% of the object is larger than 1MB, while 100\% of object accesses in trace 36 is smaller than 1MB. 

% \souj{Sample 31 out of how many remaining traces?}
% \souj{Say we pick 5 traces of 31 (results of all 31 traces are in appendix) and add graphs for the 5 traces we pick!}


\textbf{Workload expansion.}
% The available traces record operations in a week. However, we need longer traces to evaluate replication policies with real-world pricing structures for network and storage costs. For instance, on average, it takes about 2.33 months for the storage cost of an object to dominate its network cost. 
The available traces record operations only for a week. However, this snapshot is too short to capture the full lifecycle of objects in a cloud object store environment. Object storage systems are typically designed for long-term data retention, with many objects being stored for months or even years (e.g., the storage pricing is structured per GB per month) ~\cite{}. 
Therefore, we first expand traces to longer periods without modifying their inherent characteristics like frequency, recency, and the bytes that are read and written. We treat the weekly traces to represent monthly patterns by considering the observed access patterns in a day to be effective on roughly a month's timescale. 

% \shu{any way to reason about this? T\_even is larger so we extend the trace period to longer}
% \shu{In practice, taking a snapshot of 7 days doesn't make sense because of the pricing structure. People store these objects for months, storage patterns - people reason about it over month (cost structure: \$/GB), in practice people store it forever; our results are skew if it looks at shorter time. There exists trade-offs in practice}


\textbf{Single region to two-region base and cache.}
The available traces are collected from a single region (base region) within a cloud.
First, we use these traces to evaluate \sys's replication policy against alternatives where there is an additional site that can cache objects (cache region) within the same cloud.
In this setup, PUT operations are directed to the base region and GET operations are handled by the cache region.
This setup represents a popular approach~\cite{separate-compute} where data is already located in one region like for low storage cost, but the computation is run elsewhere like for resource availability and low compute cost like geo-distributed model serving service. 


\textbf{Two-region to multi-region, multi-cloud.} To the best of our knowledge, no multi-cloud workload traces are publicly available today. Therefore, we use available single-cloud traces to generate traces that capture multi-cloud workload patterns in best-effort synthetically. This approach is informed by our conversations with industry experts and their observations, which highlight the following patterns: 

% \shu{step process: step 1 - workload expansion, step 2- single region to two regions, step 3 - multi-region to multi-cloud}: 

\begin{enumerate}[noitemsep=*,leftmargin=*]
    \item \textit{Type A (Unpredictable Accesses)}: We distribute PUT and GET requests of objects randomly across regions and clouds.
    Workloads like networks of IoT sensors and e-commerce websites have this access pattern~\cite{razzaque2024analysisstatusupdatewireless}.
    % \souj{Add citations and references everywhere}
    \item \textit{Type B (Region-Based Accesses)}: 
    We dedicate PUT requests of objects to one region and get requests from another (both selected at random per each object). 
    Workloads like satellite image analysis~\cite{googleLandsatData}, disaster recovery~\cite{https://docs.aws.amazon.com/whitepapers/latest/disaster-recovery-workloads-on-aws/disaster-recovery-options-in-the-cloud.html}, and cloudburst~\cite{https://cloud.google.com/architecture/hybrid-multicloud-patterns-and-practices/cloud-bursting-pattern}, ingest data into one region and consume it from another. 
    \item \textit{Type C (Replicated Accesses)}: 
    Dedicate PUT requests to one region (selected at random per object)
    and distribute GET requests across other regions.
    CDN~\cite{la2021usecasecontentdelivery}, container registry~\cite{}, and similar applications~\cite{} typically write to a single region and read from multiple other regions.
    \item \textit{Type D (Aggregated Accesses)}: Dedicate PUT requests to multiple regions, allowing data to be ingested across various locations, but GET requests are concentrated in a single region. This pattern supports workloads like regional sales data aggregation~\cite{} and log aggregation~\cite{}, where data is collected from different regions and then accessed or analyzed in a central location.   
\end{enumerate}

We evaluate \sys's replication policy against alternative approaches for multi-cloud setup across AWS S3, Azure Blob Storage, and GCS. We run 3-region\footnote{\path{aws:us-east-1}, \path{azure:eastus}, \path{gcp:us-east1-b}}, 6-region\footnote{\path{aws:us-east-1}, \path{aws:us-west-2}, \path{azure:eastus}, \path{azure:westus}, \path{gcp:us-east1-b}, \path{gcp:us-west1-a}}, and 9-region\footnote{\path{aws:us-east-1}, \path{aws:us-west-2}, \path{aws:eu-west-1}, \path{azure:eastus}, \path{azure:westus}, \path{azure:wasteurope}, \path{gcp:us-east1-b}, \path{gcp:us-west1-a}, \path{gcp:europe-west1-b}} experiments where we select 1, 2, and 3 regions from each cloud in each setup. 

% \shu{This generates a total of however many traces: 3 * 5 * 4 * 7 = 420 configurations. Run this in simulation, we know what costs looks like in practice}

\textbf{Real-world evaluation}. 
Finally, we evaluate \sys prototype in the real world. The total size of object store operations averaging across the five traces we select is 6.7 TB per trace. With 5 traces, 4 types of trace adaptation methods (i.e., Type A-D), 8 different policies to run over 3 setups (i.e., 3, 6, and 9 regions), this generates in total 480 configurations. Considering the storage and network costs, this will cost close to 0.2 million dollars to run in real cloud setups. Since it is expensive to evaluate all settings, we combine Type A, B, C, and D workloads to Type E for each of the five traces we select and only run in the 9-region setups to show performance from \sys in the real world. 


% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=\textwidth]{figures/nsdi/output_relative_to_skystore_percentage_new.pdf}
%     \vspace{-2em}
%     \caption{\textbf{\sys Cost Savings (\%) on 2-Region, Fixed Base (FB)}: \sys achieves on average 10.1\%-57.6\% cost savings over 31 traces and 7 baselines.}
%     \label{fig:2sites}
% \end{figure*}
% \vspace{-0.5em}


% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=\textwidth]{figures/nsdi/output_relative_to_skystore_percentage_14_65_78_79_95.pdf}
%     \vspace{-2em}
%     \caption{\textbf{\sys Cost Savings (\%) on 2-Region, Fixed Base (FB)}: \sys achieves on average 10.1\%-57.6\% cost savings over 31 traces and 7 baselines.}
%     \label{fig:2sites}
% \end{figure*}

% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=\textwidth]{figures/nsdi/output_updated_vs_optimal_15_29_65_78_79.pdf}
%     \vspace{-2em}
%     \caption{\textbf{\sys Cost Relative to Optimal on 2-Region, Fixed Base (FB)}: \sys cost is within 13\% of clairvoyant greedy policy (CGP), which is cost-optimal in this setup. \shu{presentation format? Heatmap}}
%     \label{fig:2sites-optimal}
% \end{figure*}

% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=\textwidth]{figures/nsdi/output_relative_to_skystore_percentage_15_29_65_78_79.pdf}
%     \vspace{-2em}
%     \caption{\textbf{\sys Cost Savings (\%) on 2-Region, Fixed Base (FB)}: \sys achieves on average 15\% to 55\% cost savings across 5 traces, compared with 5 baselines.}
%     \label{fig:2sites}
% \end{figure*}



% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=\textwidth]{figures/nsdi/3_regions_type.pdf}
%     \vspace{-2em}
%     \caption{\textbf{\sys Cost Savings (\%) on 3-Region, Type A-D, Fixed Base (FB)}: . \shu{presentation format? Heatmap}}
%     \label{fig:2sites-optimal}
% \end{figure*}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/two_region_relative_to_opt_new.pdf}
%     \caption{\textbf{\sys v.s. Optimal on 2-Region, Fixed Base (FB)}: \sys cost is within 15\% of clairvoyant greedy policy (CGP), which is cost-optimal in this setup.}
%     \label{fig:opt}
% \end{figure}

\subsection{Baseline Policies}
\label{sec:baselines}
% We compare \sys against nine other baselines. \newline 

\textbf{Baseline policies} refer to the \textit{Always Evict} policy, where objects only reside in one storage location and there is no replication, and to the \textit{Always Store} policy, where replicas are created in regions where the read is initiated. 
\newline
% \textbf{TTL-based policies} refer to a set of static TTL policies, including $\tev=1$hr, and $\tev=12$hr, and $\tev=\teven$ (Section~\ref{eqn:teven}). We pick $1$ and $12$ hours as these values fit well for the duration of the trace. We also implement TTL-CC~\cite{TTLbasedCC2019}, a state-of-the-art baseline that dynamically adapts TTL with a stochastic approach based on the behavior of every new object entering the cache. 
\textbf{TTL-based policies} refer static and dynamic TTL policies. We evaluate $\tev=\teven$ (Section~\ref{eqn:teven}). We also implement TTL-CC~\cite{TTLbasedCC2019}, a state-of-the-art baseline that dynamically adapts TTL with a stochastic approach based on the behavior of every new object entering the cache. 
\newline
\textbf{Oracle Policy} refer to the clairvoyant greedy policy (CGP) described in Section~\ref{sec:clairvoyant}. Given the oracle's knowledge of the access times for each object, this policy decides on eviction per object. CGP is the optimal policy in the 2-region base and cache setting. \newline
\textbf{Per-object Prediction Policy}
In addition, we design a simple baseline policy that uses the Exponentially Weighted Moving Average (EWMA) 
% \cite{EWMA} 
to predict the next access time per object and choose what to evict or store accordingly. 
\newline
\textbf{Multi-cloud replication policy} is also evaluated: we measure the performance of SPANStore~\cite{spanstore}, which dynamically replicates objects per hour to minimize access costs. 
% SPANStore performs proactive replication on write, does not consider eviction and costs of replication, and requires the anticipated workload as input.
We run SPANStore in a best-case scenario where the actual workloads instead of predicted ones are fed into its solver. We evaluate it only in the free placement mode because SPANStore does not fix a storage region. 
\newline 
\textbf{Industrial baselines} consist of AWS multi-region bucket~\cite{} and JuiceFS multi-cloud replication~\cite{}. These platforms enable users to set up replication across two regions or clouds. Upon each PUT request, the data is asynchronously copied to the designated secondary region. 


\subsection{Experiment Setups}

\textbf{Cost Estimation.} We implement all policies described above with 1.9k lines of Python code. We calculate the cost of read and write operations for all traces based on our data collection regarding storage cost for the Standard Storage tier and the bidirectional egress cost between 9 AWS, GCP, and Azure regions.  
% \textbf{Simulation.} We implement all policies described above with 1.9k lines of Python code. Because running all traces over multiple regions and clouds is too expensive and slow (i.e., some of the traces contain millions of requests and GBs of object sizes), we built a simulator to simulate the cost and latency of read and write operations for all traces. The simulation numbers are based on our data collection regarding storage cost for the Standard Storage tier and the bidirectional egress cost between 9 AWS, GCP, and Azure regions.  
\newline 
\textbf{Prototype Implementation.} We build an open-source prototype of
 \sys as described in Section \ref{sec:Architecture}. \sys's metadata server is implemented
 in Python in 3.5K lines of code and can run on a SQLite or Postgres database\cite{postgres-replication}. The S3-proxy is implemented in Rust in about 9k lines of code, connecting to AWS S3~\cite{aws-s3}, Google Cloud Storage~\cite{gcp-multi-region-bucket}, and Azure Blob Storage~\cite{ms-azure-blob}. We host the metadata server for prototype benchmarks on \texttt{m5d.8xlarge} instance in \texttt{aws:us-east-1}. It contains 32 vCPUs, 128 GiB of memory, and 2 x 600 NVMe SSD instance storage. We instantiate S3-proxy on one other \texttt{m5.8xlarge} machine from \texttt{aws:us-west-1}. \newline 
% \textbf{Workloads Setups} \newline 
% \newline 
\textbf{Configuration.} We evaluate five traces in the 2-region base and cache setup and multi-cloud 3-region, 6-region, and 9-region. Our simulator evaluates all policies with the fixed base mode on a 2-region base and cache setting and with both fixed and free placement modes on the multi-cloud settings. \newline
\textbf{Metrics.} We measure the total monetary cost  (i.e., storage and network costs) for the entire duration of each trace when executed with different policies. In our simulator, we calculate the byte hit ratio (\%) as the proportion of bytes that can be read from the local region and the average read latency (ms) (see Appendix). \shu{Operation cost, it still matters? Or ignore it and say minimal now. Talk with Natacha.}

% \moshik{ The 7-regions Fix-base has one base, aws-east-1, where all the PUTs are located, and the GETs are uniformly randomized across 3 Azure regions and 3 GCP regions. It simulates a multi-cloud burst scenario, where all PUTs are located in one region and GETs are in other cloud providers.}
% \moshik {In the 9-region no-base, the requests are randomized acrossthe 9-regions according to 5 different types (the types are uniformly randomized)
% The types explanation can move to the Appendix, but I think it's important to have it
% \begin{itemize}
%     \item Type A - GETs and PUTs are uniformly randomized across all the 9-Regions
%     \item TypeB - For each object, one cloud Provider (3 Rigions) is the base (all the PUTs is there) and all the GETs in one Cloud Provider (3-Regions) (The GETs and the PUTs could be in the same cloud provider with probability of 1/3)
%     \item Type C - For each object, all the GETs are in one cloud provider (3 regions) and all the PUTs are uniformly randomized across all the 9-regions
%     \item Type D - For each object, all the PUTs are in one cloud provider (3 regions) and all the GETs are uniformly randomized across all the 9-regions
%     \item Type E - For all the objects, all the GETs are in aws-east-1 and the PUTs are uniformly randomized across 3 Azure regions and 3  GCP regions (this is the 7-regions scenario)
% \end{itemize}
% }
% ignoring the largest trace (018), which has more than x requests for time purposes. \newline 


% Because the traces contain billions of objects\shu{recheck} and large object sizes, we simulate the throughput and latency numbers from collected statistics (average RTT) and verify the prototype with two-region accesses.
% \subsection{Eviction Policy Evaluation}\label{sec:eval_policy}

% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=\textwidth]{figures/output_relative_to_skystore_percentage_new.pdf}
%     \vspace{-2em}
%     \caption{\textbf{\sys Cost Savings (\%) on 2-Region, Fixed Base (FB)}: \sys achieves on average 10.1\%-57.6\% cost savings over 31 traces and 7 baselines.}
%     \label{fig:2sites}
% \end{figure*}




\subsection{Two Region Base and Cache Setting}\label{sec:twosite}
We first explore how \sys policy behaves under a 2-region base and cache setting and show that our technique has merit as a standalone caching policy. In this setup, all PUTs are located in the base region, and all GETs occur in a separate cache region. We only evaluate storage and network costs from the cache regions and ignore the storage cost of the base region, as it is constant across all policies. The evaluation is run with an average $\teven$ of 1 month, calculated using the average network transfer cost of 22 AWS regions and storage cost as the average of standard AWS storage prices. 

Figure~\ref{fig:2sites} shows the cost efficiency of \sys policy compared to the other baselines evaluated across five traces described in Section~\ref{s:workload-gen}. The cost-saving percentages show how much \sys policy can save compared to each alternative, with negative values indicating cases where other methods are more cost-effective. Generally, \sys adapts well to varying workloads (e.g., on average, 15.4\%-54.8\% cost savings) \shu{This number is ok or not? but worst case performance we are best}, closely matching or surpassing the most cost-efficient baseline method for each trace.

While \sys performs robustly on all workloads, alternative policies may work well on specific traces but perform poorly on other request patterns. For example, the Always Evict policy works well on Trace 15 and Trace 19. Trace 15 has few repeated reads and very high one-hit-wonder ratios (i.e. 48\% of objects has only 1 access). Trace 29 is a trace where GETs are repeatedly read in month. In contrast, for traces with heavy repeated reads (e.g., Trace 65 and Trace 78), the Always Evict policy will repeatedly evict and re-fetch data across regions, resulting in 71$\times$ and 22$\times$ higher cost than \sys, respectively. 

% In Trace 29, Always Evict is around 0.1\% better than \sys because \sys reactively caches data on the read location and takes about a day to collect metadata and adapt to workloads with many one-hit-wonders, while almost all requests in Trace 014 appear before the second day. 

In contrast, for traces with heavy repeated reads (e.g., Trace 065), the Always Evict policy will repeatedly evict and re-fetch data across regions, resulting in 71$\times$ higher cost than \sys. On the other hand, the Always Store policy shows the opposite results compared to Always Evict; it performs best on heavy repeated read workloads (e.g., -3.3\% on Trace 65) and worst on one-hit-wonder workloads and the workloads that have high recency between read accesses (e.g., 2.8$\times$ and 2.5$\times$ more expensive on Trace 15 and Trace 29). 

A Fixed TTL method like TTL=$\teven$ without informed decisions about the workload access patterns some times do well on some workloads like Trace 65, but on average doing bad in the others. \sys achieves -13\% (Trace 055) to 78\% (Trace 072) saving (17.41\% on average) compared to TTL-CC. TTL-CC sometimes performs poorly because it models the GET times as a Poisson distribution and this does not occur in many real traces. Lastly, compared to EWMA, \sys achieves -10.16\% (Trace 011) to 78.3\% (Trace 065) savings, averaging 25.8\%. EWMA collects statistics on a per-object basis and predicts the next access time per object. This approach can sometimes work well, but oftentimes is misleading and does not reflect the overall workload pattern. Table\ref{table:avg_std} shows the average and standard deviation of the ratio between other policies and \sys approach. Overall, xxx

% OLD: TWO REGION BASE AND CACHE SETTING 
% We first explore how \sys policy behaves under a 2-region base and cache setting and show that our technique has merit as a standalone caching policy. In this setup, all PUTs are located in the base region, and all GETs occur in a separate cache region. We only evaluate storage and network costs from the cache regions and ignore the storage cost of the base region, as it is constant across all policies. The evaluation is run with an average $\teven$ of 24 hours for our 7-day trace, calculated using the average network transfer cost of 22 AWS regions and storage cost close to standard storage prices in the cloud. 


% Figure~\ref{fig:2sites} shows the cost efficiency of \sys policy compared to the other baselines evaluated across 31 traces. The cost-saving percentages show how much \sys policy can save compared to each alternative, with negative values indicating cases where other methods are more cost-effective. Generally, \sys adapts well to varying workloads (e.g., on average, 10.1\%-57.6\% cost savings), closely matching or surpassing the most cost-efficient baseline method for each trace. 

% While \sys performs robustly on all workloads, alternative policies may work well on specific traces but perform poorly on other request patterns. For example, the Always Evict policy works well on traces with few repeated reads or high one-hit-wonder ratios (e.g., 40-65\% one-hit objects for Trace 014 and 051, >90\% on Trace 069 and 070). In these cases, Always Evict is 1.3\%-8.9\% better than \sys because \sys reactively caches data on the read location and takes about a day to collect metadata and adapt to workloads with many one-hit-wonders. In contrast, for traces with heavy repeated reads (e.g., Trace 065), the Always Evict policy will evict and re-fetch data across regions repeatedly, resulting in 71$\times$ higher cost compared to \sys. On the other hand, the 
% Always Store policy shows the opposite results compared to Always Evict; it performs best on heavy repeated read workloads (e.g., -3.3\% on Trace 065) and worst on one-hit-wonder workloads (e.g., 4.3$\times$ more expensive on Trace 069). 

% A Fixed TTL method like TTL=1hr slightly outperforms \sys on some workloads where repeated reads are close together within the 1-hour timeframe. For example, it is 7-10\% more cost-efficient than \sys on Traces 009, 011, 018, 020, and 036. However, it incurs very high costs on traces with longer duration repeated reads, such as Trace 047 for which it is 3.6$\times$ more expensive than our solution. For the cases where TTL=1hr does perform better, we verify that \sys indeed learns a 1-hour TTL. However, it does so only after a warm-up phase; thus, the \% cost increase comes from the overhead of its warm-up period. Compared to the other fixed TTL methods like TTL=12hr, \sys ranges from 1\% more expensive on Trace 072 and up to 31.7\% cheaper on Trace 070. Compared to TTL=$\teven$, where $\teven$ is 24 hours in this setup, \sys achieves -3.38\% (Trace 065) to 47.4\% cost savings (Trace 070).  \sys achieves -13\% (Trace 055) to 78\% (Trace 072) saving (17.41\% on average) compared to TTL-CC. TTL-CC sometimes performs poorly because it models the GET times as a Poisson distribution and this does not occur in many real traces. Lastly, compared to EWMA, \sys achieves -10.16\% (Trace 011) to 78.3\% (Trace 065) savings, averaging 25.8\%. EWMA collects statistics on a per-object basis and predicts the next access time per object. This approach can sometimes work well, but oftentimes is misleading and does not reflect the overall workload pattern. Table\ref{table:avg_std} shows the average and standard deviation of the ratio between other policies and \sys approach. Overall, TTL=12hr performs the best and the Always Evict policy performs the worst.

% Figure~\ref{fig:opt} shows that \sys, on average, performs within 15\% of the CGP policy, which is the cost-optimal in this setup. However, in specific cases, such as Trace 043 and Trace 056, \sys underperforms the optimal by 30-32\%. This discrepancy arises because \sys aggregates access statistics for all objects in the bucket, whereas CGP has an oracle knowledge at a more granular per-object level. For instance, the times between GETs in Trace 043 and 056 vary significantly across objects — 42.8\%, 31.3\%, 19.7\%, and 5.5\% of objects have GET recency of more than three days, between one and three days, one hour to one day, and less than an hour, respectively. Conversely, in traces like 069 and 070, where nearly all objects have similar access recency (i.e., >99\% objects are accessed within an hour), \sys cost performance is only 1-2\% lower than the optimal. 
% OLD: TWO REGION BASE AND CACHE SETTING 



% \subsection{7-Region across Clouds (Fixed Base)} 
% Our evaluation extends to a multi-region and multi-cloud setting with a fixed base mode. We direct all PUT operations to one specific base region and GETs across 6 additional regions, evenly split between AWS, Azure, and GCP (Section~\ref{sec:eval-workload}). The derived $\teven$ values range from 4 hours to 2.2 days, calculated using the smallest value within each cloud and the largest value across clouds. Figure~\ref{fig:32trace-7region} and Table \ref{table:avg_std} demonstrate that \sys consistently performs well across traces, achieving an average of 11.2\% to 69.5\% cost savings over other baselines.

% Interestingly, policy effectiveness differs with the increased number of regions. Originally, the Always Evict policy is 2.67$\times$ worse than Always Store in 2 regions, but it outperforms the other by 1.8$\times$ in 7 regions. This is because read operations are now spread over more regions, so it is less likely repeated reads on the same object will occur in the same region.
% % due to the spread of read operations per objects into more regions. 
% Take Trace 013 as an example where 99\% of objects have 2-10 GETs; when these GETs are spread across the 7 regions, most regions see only a few GETs, which makes Always Evict more beneficial due to its minimal storage cost. On the other hand, the Always Store policy still performs reasonably well for traces like 036, which has heavy reads. Second, we see lower cost savings from Table~\ref{table:avg_std} on average when comparing 2-region results with 7-region ones, except TTL-CC, which performs particularly poorly in in the multi-cloud setting. This is expected because GETs are dispersed across regions, so the base network cost for fetching objects initially becomes higher. %, thus offsetting the differentiation between baselines.  

% % Second, \sys average cost saving numbers from Table~\ref{table:avg_std} are generally lower in 7-region compared to the 2-region setting in Section~\ref{sec:twosite}. This is also expected as the GETs get distributed across regions and repeated accesses at the cache regions becomes smaller, the base cost for fetching objects initially becomes higher, thus offset the differentiation between baselines. Also, the cost heterogeneity becomes larger in multi-cloud, which can exacerbate this issue. 

% % Trace 13 can be taken as an example, where 99\% of the objects have 2-10 GETs. 
% % For example, 99\% of objects in Trace 013 contain between 2-10 reads. When we create our 7 region traces, these reads are distributed across regions, making few GETs in each region. Thus, on average, the Always Evict policy performs better than Always Store, as it is not worth storing data with only a few accesses at the cache regions. 

% Lastly, the Trace 014 result shown in Figure~\ref{fig:32trace-7region} is an outlier case where \sys performs 25\% worse than a policy like Always Evict or TTL=1hr. This trace comes with many one-hit-wonder accesses, and 90\% of GETs appear in the first 36 hours. While we verify that \sys does identify the best TTL (which is close to the Always Evict policy, the best policy in this setting), \sys does so only after a large percentage of GETs had already occurred. Hence, it fails to keep costs low for this period of time. After a long enough warm-up phase, our results are better. The same reasoning applies to why \sys fails in 085 and 095 traces. We see similar behaviors when generalizing the fixed base mode to 9-region, shown in Appendix C. 

% Lastly, one outlier of \sys appears in Trace 014, where - in this trace, 90\% of the GETs occur in the first 36 hours. While \sys does identify the best TTL here, which is Always Evict, since there are hardly any repeated reads). However, it does so only after a large percent of the GETS had already occurred. Hence, it fails to keep up. After enough of a warm-up phase, our results become even better. Same reasonings apply for Trace 013 and Trace 095. Table~\ref{table:avg_std} lists the average saving of our method in this setting. The savings compared to TTL=12hr are over 11\%, then TTL=1hr, and then $\teven$. In this complex setting, TTL-CC did not fare well. We run the fixed base mode for 9-region traces as well and draw similar conclusions, as in Appendix\ref{}.


% Also, 
% This is because the cost for the initial get of an object is the same for all methods, and only subsequent gets make the difference. In the 7-region traces, there are many more initial gets and far fewer subsequent ones, leaving less potential for differentiation between methods. Also, higher network costs exacerbate this issue for multi-clouds. 

% The cost savings \sys achieves change from 57.6\% from the 2-region base and cache setup to 67.5\% because the network cost of the Always Evict policy is even more expensive, considering data now can be located in another cloud. \shu{Write about example of 047, reads are spreaded and always store always evict behavior; write about 013 (have few GETs, and when it becomes multi-region --> all the reads, 99\% between 2-10 reads), 036 (over 1) the majority of objects have between 10-100 reads, does not get affected}

\begin{figure*}[tbp]
    \centering
    \includegraphics[width=\textwidth]{figures/byte_hit_ratio_9_region_no_base.pdf}
    \vspace{-2em}
    \caption{\textbf{\sys Byte Hit Ratio (\%) on 9-Region, Free Placement (FP):} \sys policy on average within 10\% of the byte hit ratio of the  Always Store policy.}
    \label{fig:32trace-9region-byte-hit}
\end{figure*}



\begin{figure*}[tbp]
    \centering
    \includegraphics[width=\textwidth]{figures/savings_7_region_base_without_storage.pdf}
    \vspace{-2em}
    \caption{\textbf{\sys Cost Savings (\%) on 7-Region, Fixed Base (FB)}: \sys achieves on average 11.2\% - 69.5\% cost savings over 30 traces and 6 other baselines.}
    \label{fig:32trace-7region}
\end{figure*}



\begin{figure*}[tbp]
    \centering
    \includegraphics[width=\textwidth]{figures/savings_9_region_no_base.pdf}
    
    % \vspace{-2em}
    \caption{\textbf{\sys Cost Savings (\%) on 9-Region, Free Placement (FP)}: \sys achieves on average 2.0\%-59.4\% cost savings over over 30 traces and 6 other baselines.}
    \label{fig:32trace-9region}
\end{figure*}

\begin{table}[t]
\centering
\small
\begin{tabular}{lcccccc}
\toprule
\textbf{Policy} & \multicolumn{2}{c}{\textbf{2-Region (FB)}} & \multicolumn{2}{c}{\textbf{7-Region (FB)}} & \multicolumn{2}{c}{\textbf{9-Region (FP)}} \\
\cmidrule{2-7}
& \textbf{Avg} & \textbf{Std Dev} & \textbf{Avg} & \textbf{Std Dev} & \textbf{Avg} & \textbf{Std Dev} \\
\midrule
\textit{Always Evict} & 7.85 & 16.19 & 3.28 & 5.55 & 2.46 & 3.89 \\
\textit{Always Store} & 2.94 & 1.28 & 6.09 & 8.89 & 1.49 & 0.28 \\
\textit{TTL-CC} & 1.34 & 0.67 & 2.37 & 4.22 & 1.64 & 2.04 \\
\textit{TTL=12hr} & 1.22 & 0.15 & 1.13 & 0.15 & 1.02 & 0.05 \\
\textit{TTL=1hr} & 1.25 & 0.60 & 1.16 & 0.52 & 1.08 & 0.30 \\
\textit{Teven} & 1.46 & 0.30 & 1.42 & 0.33 & 1.08 & 0.12 \\
\textit{EWMA} & 1.49 & 0.66 & N/A & N/A & N/A & N/A \\
\textit{SPANStore} & N/A & N/A & N/A & N/A & 1.35 & 0.24 \\
\bottomrule \\
\end{tabular}%
\caption{Average and standard deviation of existing baselines, measured as the average ratio between baseline v.s. \sys total cost across traces. FB denotes the free base mode, and FP denotes the free placement mode.}
\vspace{-2em}
\label{table:avg_std}
\end{table}

% \subsection{9-Region across Clouds (Free Placement)}
% We additionally evaluate a 9-region multi-region and multi-cloud setup under the free placement mode, picking 3 regions from AWS, GCP, and Azure respectively. The $\teven$ values are similar to that of the 7-region setting. Figure~\ref{fig:32trace-9region} and Table~\ref{table:avg_std} show \sys on average achieves 2\% to 59\% cost savings in this setting. The behavior of the free placement mode is harder to predict than a fixed base setting. This is mainly because replicas are not evicted at their expected time if they are the only remaining replicas of these objects. Still, our method outperforms the other options across the traces. The average cost increase with the TTL=12hr policy is only 2\%, with the TTL=1hr policy at around 10\%. The smaller improvement of \sys is because we account for the storage cost of the base region in our setting. 

% We also implement SPANStore as one of the baselines in this experiment, as shown in Table\ref{table:avg_std}. SPANStore performs similarly to the Always Store policy as it does not consider removing objects in the accessed sets, even if these objects have not been accessed for a long time. In reality, SPANStore can sometimes perform worse than the Always Store policy when it erroneously pushes data to regions where reads are rare. We show that \sys can achieve 35\% cost savings compared to SPANStore even when the latter system is given oracular workload knowledge.  

% \subsection{Multiple Sites and Clouds - Free Placement}
%\subsection{System Comparisons}
%We evaluate all the algorithms on our end-to-end systems and compare them with commercial solutions, for example, AWS replications.  
%\subsubsection{Naive Solutions}
%Replicate everywhere, store in a single place 

%\subsubsection{Academic Baselines}
%\subsubsection{Commercial Solutions}



%\subsection{Eviction Policy Ablation}

\subsection{Type Generation Results}
\subsection{\sys Policy Ablation}
We also dive into \sys's policy in detail, investigating how \sys performs in terms of byte hit ratio, and whether the policy indeed chooses good TTLs in different workloads. 

\subsubsection{How does \sys's policy affect byte hit ratio?}
\label{sec:latency}

Aside from the cost, we study how \sys's policy affects the byte-hit ratio of each read operation, which reflects how it affects average read latency. We expect the Always Store policy to have the highest hit ratio among the baselines we evaluate, as it only incurs cold misses when an object is first accessed in a remote region. Figure~\ref{fig:32trace-9region-byte-hit} shows the byte hit ratio across 31 traces with the 9-region free placement setup: \sys achieves, on average, within 10\% of the hit ratio of the Always Store policy. This is because while \sys optimizes for cost, it also makes the best effort to retain objects in the cache as a caching policy, as the ratio between network and storage costs is often high. 
% \shu{explain sentence more}

\subsubsection{Is learning the past indicative of the future?}
\label{sec:future}
In our method, we implicitly assume that monitoring the workload and finding the best expected TTL over the past indicates the future. In other words, is the best TTL for the past also worthwhile in the future? 
We examine the learned TTL in the two-region experiments (with a $\teven$ value of 24 hours). We compare the best expected TTL found after only a part of the trace vs.\ the eventual best TTL over the full trace.  
The results are shown in Table~\ref{tab:ttlvs7} and indicate that once $\teven$ time has passed, the TTLs are largely similar.
Of the 31 traces, one stands out (trace number 013). It had hardly any traffic in the first five days, and most of the traffic occurred on the last day, making training early meaningless, even after three days. All the other traces either found the absolute best TTL after three days or gave very close TTL value, resulting in no more than a 5\% additional cost during the last four days of the trace (over the weekly best TTL). % An interesting question for future study would be how this changes over longer periods, requiring collecting information over a longer time frame. 
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|}
    \hline
     TTL training   &  \# traces with same TTL \\
     period & as full-week TTL \\
\hline
     1/2 day    &  16/31 \\
     1 day    &  24/31 \\
     3 days & 26/31 \\
     \hline
    \end{tabular} \\
    \caption{Comparing TTLs trained on a prefix of the trace vs.\ the best TTL for the full trace.}
    \label{tab:ttlvs7}
    % \vspace{-2em}
\end{table}

%\subsubsection{What is the overhead of \sys statistics collection?} %danny we don't have anything meaningful to say on this....

\subsection{System ablation}
%\subsubsection{Changes of Histograms}
%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{figures/costhist029.png}

%    \vspace{-1em} % Adjust this value as needed
%    \caption{The expected cost as a function of TTL for an example trace (no 29) with an hourly histogram. \shu{should move this to the system ablation studies in eval}}
%    \label{fig:costhist}
%\end{figure}

% \begin{figure*}[tbp]

%     \centering
%     \includegraphics[width=\textwidth]{figures/output_relative_to_skystore.pdf}
%     \label{fig:32trace-2region}
%     \vspace{-2em}
%     \caption{32 Trace, 2 Region Experiments (Relative To SkyStore) \shu{Put a line, but put what is higher cost above, and lower cost below (to make it easier to visualize)}}
% \end{figure*}

We use the JuiceFS benchmark to measure \sys's system overhead compared to naively using the provider's tool. We run the performance test on the object store and compare the latency for operations with and without \sys. The benchmark consists of put, get, list, head, and delete operations over 10K objects, each of size 128 KB, and measures the average latency per object. The result in Fig. \ref{fig:proxy-overhead} shows that the overhead of using \sys compared to using cloud provider's API is minimal: for put and get operations, the overhead is less than 10\%. Furthermore, \sys can even speed up the list and head operations by up to 3.4$\times$ because of the efficiency of the control plane. 

\begin{figure}
    % \centering
    \includegraphics[width=.85\linewidth]{figures/juicefs.pdf}
    \caption{Single object store performance: with and without \sys on region \textit{aws:us-east-2}, server on region \textit{aws:us-east-2}, reading from object store in \textit{aws:us-east-2}}.
    \label{fig:proxy-overhead}
    \vspace{-2em}
\end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=.85\linewidth]{figures/aws_throughput.pdf}
%     \caption{Scalability Experiments}
% \end{figure}

% \subsubsection{Single Object Store: scalability}
% Using https://github.com/dvassallo/s3-benchmark here to plot the relationship between thread count and performance. 

% s3 benchmark config: ./s3-benchmark --upload-csv result128 --bucket-name skystore-us-west-1 --threads-max 32 --payloads-min 10 --payloads-max 12
% Run Azure and GCP (different object models and system architecture), run it on different clouds (map S3 API to Azure and GCP API, multipart, juiceFS, scalability, cross-clouds performance, multipart (API that maps to existing cloud providers))

% \subsection{Limitation}
% \shu{Here: need to address 1) the instance cost of the metadata server 2) ignore operational cost, might double operational cost with additional write operation request along with read}

% \subsection{Synthetic Trace Ablations}
% \subsubsection{Details of Trace}
% To comprehensively examine Object Storage behavior, we analyzed 98 traces from the Storage Networking Industry Association’s (SNIA) I/O Traces, Tools, and Analysis (IOTTA) repository~\cite{SNIA_TRACE}.

% Each trace provides a log record of RESTful operations over a one-week period for a single bucket within IBM’s object storage system~\cite{LRUvsFIFO}. Each row in the trace represents a REST access with the following columns: 
% <TIMESTEMP> the time elapsed in milliseconds from the beginning of the week. 
% <OP> the operation type (GET, PUT, HEAD, DELETE, COPY).
% <OBJ\_KEY> an anonymized Object key.
% <SIZE> the Object Size.
% <RANGE> - Optional range columns.
% The original logs contained additional columns that were removed from the public dataset.

% \subsubsection{Tuning workload sizes}


% \subsubsection{Tuning read and write ratios}


% \subsection{Algorithms}
% \subsubsection{Naive Solutions: No Replication and Replicate Everywhere}


% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/combined_figure.pdf}
%     \caption{Simulation: read, write latency and cost comparisons} 
% \end{figure}
% We compare ourselves against SPANStore~\cite{}, a multi-cloud replication policy that optimizes objects in aggregate access sets periodically (per hour) to minimize access costs. SPANStore performs proactive replication on write, does not consider eviction and replication cost, and requires the anticipated workload as input.
% We run SPANStore in a best-case scenario where we input the actual workload rather than a prediction. SPANStore does not fix a storage region; thus, we evaluate SPANStore only in the free placement mode. Notably, SPANStore's exponentially growing optimizer overhead prevents us from applying it to traces that involve many cloud regions~\cite{SpanStore,ILP(cite spanstore)}.

% stores. SPANStore behaves the same as \textit{always store} policy in the 2-region base and cache setting, and incurs higher storage and network cost in the multi-cloud settings. 

% \textbf{Basic Solutions} We include two basic solutions, one is \textit{always evict}
% \begin{itemize}
% \item{\em Basic Solutions - }
% \begin{itemize}
%     \item {\em always evict} which amounts to storing all the objects only in their original written site with no caching at all.
%     \item {\em always store} which amounts to holding permanent replicas in every locations in which the object was ever read. 
% \end{itemize} 
% %\item{\em Academic placement methods - } Spanstore
% %Fixed cache policies (LRU, GDSF), academic baselines (SPANStore, Dynamic TTL, keep-not-keep (address it manually)) 
% \item{\em TTL based methods } - We test a number of options for setting the TTL:
% \begin{itemize}
%     \item $\tev =\teven$ this method discussed in Section~\ref{sec:teven} is equivalent to the method suggested and tested in \cite{tokeep2014} (see Section~\ref{sec:related}).
%     \item $\tev= 1$ hour - We see many traces fare well with this. 
%     \item $\tev=12$ hours - A medium length choice compared to our trace length.
%     \item TTL-CC from the paper \cite{TTLbasedCC2019}. Like our method, this updates the TTL of an edge based on the observed writes. Unlike our method it uses a stochastic approach that adjusts the TTL based on the subsequent behavior of every new item that enters the cache. 
% \end{itemize}
% \item {\em Other:} 
% \begin{itemize}
%     \item The Clairvoyant Greedy algorithm described in Section~\ref{sec:clairvoyant}. This is used as a baseline, particularly for the two-site tests as it is the optimal policy for that setting. 
%     \item EWMA - we implemented an attempt to predict the next access time of objects on a per object level using the Exponentially Weighted Moving Average (EWMA) method \cite{} and then to decide whether to evict the item or not accordingly. The results for this method were extremely poor and thus we omit them from the graphs.    
% \end{itemize}
% \end{itemize}

==> sections/6_evaluation_new.tex <==
% \FloatBarrier

\section{Implementation}
% \textbf{Cost Estimation.} 
% \textbf{Simulation.} We implement all policies described above with 1.9k lines of Python code. Because running all traces over multiple regions and clouds is too expensive and slow (i.e., some of the traces contain millions of requests and GBs of object sizes), we built a simulator to simulate the cost and latency of read and write operations for all traces. The simulation numbers are based on our data collection regarding storage cost for the Standard Storage tier and the bidirectional egress cost between 9 AWS, GCP, and Azure regions.  

% \noindent 
% \textbf{Prototype.} 
We prototype \sys as described in Section \ref{sec:Architecture}.
We implement all baselines (as outlined in Section~\ref{eval:baselines}) in 1.9k lines of Python code.
\sys's metadata server is implemented
 in Python in 3.5K lines of code and support running on a SQLite or Postgres database\cite{postgres-replication}. The S3-proxy is implemented in Rust in about 9k lines of code, connecting to AWS S3~\cite{aws-s3}, Google Cloud Storage~\cite{gcp-multi-region-bucket}, and Azure Blob Storage~\cite{ms-azure-blob}. We host the metadata server for prototype benchmarks on \texttt{m5d.8xlarge} instance in \texttt{aws:us-east-1}. It contains 32 vCPUs, 128 GiB of memory, and 2 x 600 NVMe SSD instance storage. We instantiate S3-proxy on client VMs, using \texttt{m5.8xlarge}, \texttt{Standard\_D32ps\_v5}, and \texttt{n2\-standard\-32} instance types on AWS, Azure, and GCP, respectively. Similarly, client machines contain 32 vCPUs, 128 GiB of memory, and 64 GB of storage. 

 % \newline 
% \textbf{Workloads Setups} \newline 
% \newline 



\section{Evaluation} \label{s:eval}
% In this section, we first introduce
%     the workloads (Section~\ref{eval:workloads-baselines-settings}) and deployment setups (Section~\ref{eval:metrics_baselines_deploy}) we use in our evaluation. Then, we compare \sys's cost-optimized replication policy against other policies
    % and answer the following questions: 
In this evaluation, we answer the following questions: 
    % \natacha{If you're looking for space, I'd just say "In this evaluation, we answer the following questions"}

\begin{enumerate}[noitemsep=*,leftmargin=*]
    \item What are the cost benefits of \sys's replication policy in a two-region, single-cloud setting? (Section~\ref{eval:two-region})
    % \natacha{not clear what you mean by "base and cache setting"}
    \item How does \sys adapt to a three-region, multi-cloud setting? (Section~\ref{eval:three-region})
    \item Does \sys scale to more regions in multi-cloud? (Section~\ref{eval:nine-region}) 
    \item What are the end-to-end latency and cost savings of \sys in the real world? (Section~\ref{eval:real})
    \item What are the overheads in \sys? (Section~\ref{eval:overheads})
\end{enumerate}


% Then, we showcase the cost improvements of 
%     \sys relative to other baselines within a cloud 
%     in a two-region base and cache setting (Section~\ref{eval:two-region}).
% Next, we analyze the performance of \sys in a multi-cloud setup
%     across three regions (Section~\ref{eval:three-region}),
%     and discuss its scalability to nine regions across
%     three clouds (Section~\ref{eval:nine-region}).
% Finally, we discuss the latency and cost of \sys
%     on a real deployment across three regions (Section~\ref{eval:real}).


\subsection{Multi-Region, Multi-Cloud Workloads}
\label{eval:workloads-baselines-settings}

We describe the object store traces we use in our evaluation and their characteristics (Section~\ref{eval:workload-gen}, Section~\ref{eval:trace}. 
We then carefully describe our methodology (Section~\ref{eval:multi-cloud-generation}) to generate multi-cloud traces from these traces. This was necessary as no publicly available multi-cloud traces exist to our knowledge. 

% \natacha{I would phrase it a bit differently. "use in our evaluation and their characteristics. We then carefully describe our methodology to generate multi-cloud traces from these workloads. This was necessary as there does not exist any publicly available mutli-cloud traces}

% We then generate multi-cloud workloads based on real-world use cases (Section~\ref{eval:multi-cloud-generation}). This is critical as there are no multi-region and multi-cloud traces that are publicly available to the best of our knowledge.

% We describe the multi-cloud workloads(Section~\ref{eval:workload-gen}),
%     baselines (Section~\ref{eval:baselines}),
%     and deployment settings
%     and metrics (Section~\ref{eval:deploy}) we consider in our evaluation.
% \souj{Add forward references to subsubsections}

\subsubsection{Workload generation from traces}
\label{eval:workload-gen}
Our workloads are drawn from the
    IBM Object Store traces~\cite{SNIA_TRACE} that record a week of RESTful operations (e.g., GET, PUT, HEAD, DELETE) 
    for a single region in the IBM cloud~\cite{LRUvsFIFO}. 
However, object storage systems are typically designed for long-term data retention where objects are stored for several months to years (e.g., the storage pricing per GB per month) ~\cite{long-term-storage}. 
Since these traces inadequately capture the life of objects in the cloud, we expand a day in each trace to a month in a single cloud setup and to around 3 months in a multi-cloud without changing the inherent characteristics of each trace. 
\shu{patterns: read/write ratio, frequency; storage cost, not okay to be short, so have to expand}
\shu{NEW: While these traces are great at capturing read and write access patterns because they are very short, they do not capture the true costs of long-term object storage, which is traditionally measured in months or years. Thus, we expand a day in each trace to a month in a single cloud setup and to around 3 months in a multi-cloud without changing the inherent characteristics of each trace.}
\natacha{Still needs work. If they "inadequately" capture the life of objects in the cloud, why use them? Could you say that while these traces are great at capture read/write access patterns, because they're so short, they don't capture the true costs of long-term object storage, which is traditionally measured in months of years? }
% Since these traces inadequately capture the life of objects in the cloud
%     that are typically stored for longer time periods (several months to years), 
%     we expand a day in each trace to a month 
%     without changing the inherent characteristics of each trace.
% this is too less of evidence 

% \shu{\textbf{Workload Expansion} However, this snapshot is too short to capture the full lifecycle of objects in a cloud object store environment. Object storage systems are typically designed for long-term data retention, with many objects being stored for months or even years (e.g., the storage pricing is structured per GB per month) ~\cite{}. Thus, we first expand traces to longer periods without changing their inherent characteristics. We treat the weekly traces to represent monthly patterns by considering the observed access patterns in a day to be effective on roughly a month's timescale. }

We pick five representative traces with salient characteristics
    in recency, frequency, size, burstiness, and PUT and GET distribution.
In the interest of space, 
    we outline the characteristics of these five traces and the key insights that inform the generation of multi-cloud and multi-region workloads. 
    % This is critical as there are no multi-region and multi-cloud workloads that are publicly available to the best of our knowledge.

% In the interest of space,
%     we use these five traces to demonstrate \sys's cost savings
%     in this paper and present complete results over 31 traces in our Appendix~\ref{}. 
% \souj{Make sure we have this} \shu{we don't have appendix allowed}

% We outline the characteristics of five representative traces
%     within a single region and the key insights that inform the
%     generation of multi-cloud and multi-region workloads;
%     this is critical as there are no multi-region and multi-cloud 
%     workloads that are publicly-available to the best of our knowledge.


\subsubsection{Trace characteristics}
\label{eval:trace}
Cloud applications have unique access patterns
    across dimensions like object sizes,
    PUT to GET ratios, access frequency, recency, and burstiness,
    as shown in Figure~\ref{fig:5_trace_new_analysis}. 


% \begin{itemize}[noitemsep=*,leftmargin=*]
% \item
% \textit{Object sizes}: We observe objects in different size ranges: tiny ($<$1KB), small (1KB to 1MB), medium (1MB to 1GB), and large (>1GB), as shown in Figure-\ref{fig:5_trace_new_analysis}a. 
% Two traces (T29 and T65) have nearly half tiny objects while others have little.
% All traces have a large proportion (34--97\%) of small objects. Medium-size objects are common (34--60\%) in two traces (T65 and T79) but rare (<20\%) in three others. 
% None of the traces except T65 and T79 have a few objects larger than 1GB. 
% % None of the traces except T65 and T79 have a few objects larger than 1GB. 
% % About 34\% and $>$60\% of objects in T65 and T79 are medium-sized. However, less than 20\% of the other traces have medium objects.
% % None of the traces except T65 and T79 have some large objects (i.e. <0.4\%). 
% \natacha{What's the high level point that you are trying to make? Some traces access primarily tiny or small objects, while some traces access medium objects only? Accesses to large objects are very rare (see trace X,Y?) Try to structure the paragraph rather than just give numbers.}
% % However, no objects in T29 and 
% % about 5--20\% of other traces (T78 and T15) have medium objects.
% % None of the trace except Trace 65 and 79 has about 0.03\% and 0.35\% large objects. 


% \item
% \textit{Access frequency and one-hit wonders}: 
%     In our traces, objects are one-hits (1 GET), cold (1-10 GETs),
%         warm (10-100 GETs), and hot (100-1000 GETs),
%         as shown in Figure~\ref{fig:5_trace_new_analysis}b.
%     % There is one one-hit-wonder heavy (50\% of the objects) trace, T15, while $<$20\% of objects in other traces are one-hits.
%     One-hits are generally rare, appearing mostly in T15 (50\% of the objects) and less than 20\% in other traces. 
%     All (98\%) objects in T29 a majority 61\% of objects in T79 are cold.
%     None of the objects in T29 are warm, and the remaining 21\% of objects in T79 are warm.
%     In two traces (T65 and T78, respectively), 67\% and 11\% of the objects are hot, while none of the other traces contain super hot object accesses. \natacha{Same comment as above. Try to craft a narrative around the numbers. "Most trace}
% \item
% \textit{Burstiness}: 
%      We measure burstiness as the fraction of GETs over time. In T78, most objects (60\%) appear during the last two months, while other traces have $<$50\% in the same period. T15 has an even distribution of accesses without any accesses in a couple of months. Three traces (T29, T65, and T79) nearly have an equal distribution of GETs, with a noticeable spike, where 30\% of objects are accessed in short intervals in two traces (T65 and T79),
%      as shown in Figure~\ref{fig:5_trace_new_analysis}c.
     

% \item
% \textit{Recency of accesses}:
%     Our traces also have varying recency, i.e., the time interval between consecutive GETs, as shown in Figure-\ref{fig:5_trace_new_analysis}d. Two traces (T15 and T78) have inter-arrival times within a day. In contrast, T65 and T79 show about 10\% of GET intervals falling between one day and one month. In T29, $>$80\% objects are read between one day and up to two months, and the remaining intervals even exceed two months.

    
% \item
% \textit{Ratio of GET and PUT operations}: 
%     Three traces (T65, T78, and T79) are read-dominated, as shown in the Figure~\ref{fig:5_trace_new_analysis}e. Others (T15 and T29) are write-heavy with 42\% and 30\% of PUTs. Note that T29 has $>$10M requests in total.

% \end{itemize}


\shu{newly written as above}
\begin{itemize}[noitemsep=*,leftmargin=*]
\item
\textit{Object sizes}: We observe objects in four size ranges: tiny ($<$1KB), small (1KB to 1MB), medium (1MB to 1GB), and large (>1GB), as shown in Figure-\ref{fig:5_trace_new_analysis}a. Two traces (T29 and T65) have 30--45\% of tiny objects while others have $<$0.5\% of tiny objects.
Three traces (T15, T29 and T78) have a majority (56--97\%) of small objects
while others have 34-40\% of small objects.
About 34\% and $>$60\% of objects in T65 and T79 are medium-sized. However, less than 20\% of the other traces have medium objects.
None of the traces except T65 and T79 have some large objects (i.e. <0.4\%). 
\natacha{What's the high level point that you are trying to make? Some traces access primarily tiny or small objects, while some traces access medium objects only? Accesses to large objects are very rare (see trace X,Y?) Try to structure the paragraph rather than just give numbers.}
% However, no objects in T29 and 
% about 5--20\% of other traces (T78 and T15) have medium objects.
% None of the trace except Trace 65 and 79 has about 0.03\% and 0.35\% large objects. 


\item
\textit{Access frequency and one-hit wonders}: 
    In our traces, objects are one-hits (1 GET), cold (1-10 GETs),
        warm (10-100 GETs), and hot (100-1000 GETs),
        as shown in Figure~\ref{fig:5_trace_new_analysis}b.
    About 50\% of the objects T15 are one-hits, while
       $<$20\% of objects in other traces are one-hits.
    All (98\%) objects in T29 a majority 61\% of objects in T79 are cold.
    None of the objects in T29 are warm, and the remaining 21\% of objects in T79 are warm.
    In two traces (T65 and T78, respectively), 67\% and 11\% of the objects are hot, while none of the other traces contain super hot object accesses. \natacha{Same comment as above. Try to craft a narrative around the numbers. "Traces differ in their degree of cacheability. While T15 has almost half of one-hit wonders, ... Right now it's hard to understand the high level picture for those paragraphs and it kinda just reads like a list of arbitrary numbers}
\item
\textit{Burstiness}: 
     We measure burstiness as the fraction of GETs over time. In T78, most objects (60\%) appear during the last two months, while other traces have $<$50\% in the same period. T15 has an even distribution of accesses without any accesses in a couple of months. Three traces (T29, T65, and T79) nearly have an equal distribution of GETs, with a noticeable spike, where 30\% of objects are accessed in short intervals in two traces (T65 and T79),
     as shown in Figure~\ref{fig:5_trace_new_analysis}c.
     

\item
\textit{Recency of accesses}:
    Our traces also have varying recency, i.e., the time interval between consecutive GETs, as shown in Figure-\ref{fig:5_trace_new_analysis}d. Two traces (T15 and T78) have inter-arrival times within a day. In contrast, T65 and T79 show about 10\% of GET intervals falling between one day and one month. In T29, $>$80\% objects are read between one day and up to two months, and the remaining intervals even exceed two months.

    
\item
\textit{Ratio of GET and PUT operations}: 
    Three traces (T65, T78, and T79) are read-dominated, as shown in the Figure~\ref{fig:5_trace_new_analysis}e. Others (T15 and T29) are write-heavy with 42\% and 30\% of PUTs. Note that T29 has $>$10M requests in total.
    \natacha{Might be easier to rename traces A,B,C,D,E rather than give them numbers. Makes it sound more arbirary (to me at least)}

\end{itemize}


% \subsubsection{Trace characteristics}
% \label{eval:trace}
% Cloud applications have unique access patterns
%     across dimensions like object sizes,
%     PUT to GET ratios, access frequency, recency, and burstiness,
%     as shown in Figure~\ref{fig:5_trace_new_analysis}. 


% \begin{itemize}[noitemsep=*,leftmargin=*]
% \item
% \textit{Object sizes}: We observe objects in four size ranges: tiny ($<$1KB), small (1KB to 1MB), medium (1MB to 1GB), and large (>1GB), as shown in Figure-\ref{fig:5_trace_new_analysis}a. Two traces (T29 and T65) have 30--45\% of tiny objects while others have $<$0.5\% of tiny objects.
% Three traces (T15, T29 and T78) have a majority (56--97\%) of small objects
% while others (T90 and T65) have have 34-40\% of small objects.
% About 34\% and $>$60\% of objects in two traces (T65 and T79) are medium-sized. However, less than 20\% of the other traces have medium objects.
% None of the traces except T65 and T79 have large objects, and the percentage is low (i.e. <0.4\%). 
% % However, no objects in T29 and 
% % about 5--20\% of other traces (T78 and T15) have medium objects.
% % None of the trace except Trace 65 and 79 has about 0.03\% and 0.35\% large objects. 


% \item
% \textit{Access frequency and one-hit wonders}: 
%     In our traces, objects are one-hits (1 GET), warm (1-10 GETs),
%         hot (10-100 GETs), and super hot (100-1000 GETs),
%         as shown in Figure-\ref{fig:5_trace_new_analysis}b.
%     About 50\% of the objects in a trace (T15) are one-hits, while
%        $<$20\% of objects in other traces are one-hits.
%     While almost all (98\%) objects in a trace (T29) are warm,
%         a majority 61\% of objects in another (T79) are warm.
%     None of the objects in T29 are hot, and the remaining 21\% of objects in T79 are hot.
%     In two traces (T65 and T78 respectively), 67\% and 11\%
%         of the objects are super hot while none of the objects
%         in other traces are super hot.
%     \souj{I think these numbers do not add up? Fix them?}

% \item
% \textit{Recency of accesses}:
%     Our traces also have varying recency, i.e., time interval between consecutive GETs, as shown in Figure-\ref{fig:5_trace_new_analysis}c. Two traces (T15 and T78), have inter-arrival times that are within a day. In contrast, T65 and T79 show about 10\% of GET intervals falling between one day and one month. In T29 $>$80\% objects are read within one hour to two months, and the remaining intervals exceeding two months.
    
% \item
% \textit{Burstiness}: 
%      We measure burstiness as the fraction of GETs over time. In T78, a majority of objects (60\%) appear during the last two months, while other traces have  $<$50\% in the same period. T15 has an even distribution of accesses without any accesses in a couple of months. Three traces (T29, T65, and T79) nearly have an equal distribution of GETs, with a noticeable spike, where 30\% of objects are accessed in short intervals in two traces (T65 and T79),
%      as shown in Figure-\ref{fig:5_trace_new_analysis}d.
%     \souj{Check description and numbers}

% \item
% \textit{Ratio of GET and PUT operations}: 
%     Three traces (T65, T78, and T79) are read-dominated, as shown in the Figure~\ref{fig:5_trace_new_analysis}e. Others (T15 and T29) are write-heavy with 42\% and 30\% of PUTs. Note that T29 has $>$10M requests in total.

% \end{itemize}

\noindent
\subsubsection{Multi-region, Multi-cloud workload generation}
\label{eval:multi-cloud-generation}
To address the lack of multi-cloud workloads, we use our five traces to synthetically generate such workloads in three steps.

\noindent
\textbf{Step 1: single to 2-region, base and cache}. We first explore the single-cloud, two-region base and cache setup described in Section~\ref{s:problem-twosite}. This setup represents a popular approach~\cite{separate-compute} where data is already located in one region, but the computation is run elsewhere for resource availability (e.g., geo-distributed model serving service). Recall that our traces are from a single (base) region within the IBM cloud. To support this setup, we direct all GET operations to the cache region and PUT operations to the base region. 
\natacha{I'd rephrase to: We generate a workload in which all PUT operations go to the base region and all GET operations to the cache region.}
% To support two regions where objects are accessed from another (cache) region
%     within the same cloud, which is a popular deployment setting (\ref{eval:deploy}),
%     we direct all GET operations to the cache region.
% \souj{Fix the forward reference}

\noindent
\textbf{Step 2: 2-region to multi-region and multi-cloud}. Our synthesis of multi-cloud workloads is informed by our conversations with industry experts and their observations, which highlight the following patterns:
% \souj{Fix missing citations and references below}
\begin{enumerate}[noitemsep=*,leftmargin=*]
    \item \textit{Type A (Uniform Workloads)}:
    Applications like
        networks of IoT sensors~\cite{razzaque2024analysisstatusupdatewireless} and 
        e-commerce websites~\cite{Hristoski_2016}
        have uniformly random access patterns.
    For this workload, we distribute PUTs and GETs 
        randomly across regions and clouds.

    \item \textit{Type B (Region-Aware Workloads)}:
    Applications like 
        satellite image analysis~\cite{googleLandsatData},
        disaster recovery~\cite{disaster-recover}, and 
        cloudburst~\cite{cloud-burst},
        Data is ingested in one but consumed from another region. 
    For this workload, we assign a PUT region and a GET region per object and distribute requests accordingly. 

    \item \textit{Type C (Aggregation Workloads)}:
    Applications that aggregate regional sales data,
        logs, etc., collect data from different regions~\cite{lakehouse}
        and access or analyze it from one central region.   
    For this workload, we distribute PUTs to multiple regions for data to be ingested across regions and dedicate all GETs to only one region.
        
    \item \textit{Type D (Replication Workloads)}: 
    CDN~\cite{peroni2024endtoendpipelineperspectivevideo}, container registry~\cite{278314}, and
        geo-distributed model serving~\cite{alkassab2023deeprefdeepreinforcementlearning} typically 
        write to a single region and read from
        multiple other regions.
    For this workload, we dedicate 
        PUTs on an object to one region at random
        and distribute GETs across other regions.
    
    
\end{enumerate}

\noindent
\textbf{Step 3: Combined multi-cloud workload}. 
% \shu{why synthetic? everything up to this point is synthetic, we just pick one to run our real prototype}
Each workload above stores and accesses 6.7 TB of data on average.
It costs about 0.2M dollars to evaluate all workloads and setups of
    \sys in real cloud deployments. 
Therefore, we combine our multi-cloud workloads into
    a single workload type and run a single trace (T65) and two baselines to demonstrate our end-to-end system and latency performance in Section~\ref{eval:end-to-end}.

% Finally, we evaluate \sys prototype in the real world.
% The total size of object store operations averaging across the five traces we select is 6.7 TB per trace. 
% With 5 traces, 4 types of trace adaptation methods (i.e., Type A-D), 8 different policies to run over 3 setups (i.e., 3, 6, and 9 regions), this generates in total 480 configurations. Considering the storage and network costs, this will cost close to 0.2M dollars to run in real cloud setups. 
% Since it is expensive to evaluate all settings, we combine Type A, B, C, and D workloads to Type E for each of the five traces we select and only run in the 9-region setups to show performance from \sys in the real world. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TWO REGION GRAPHS %%%%%%%%%%%%%%%%%
\begin{figure*}[tbp]
    \centering
    \includegraphics[width=.95\textwidth]{figures/nsdi/TypeE_2_REGIONS_output_relative_to_skystore_times_15_29_65_78_79.pdf}
    \vspace{-1em}

    \caption{\textbf{2-Region, Fixed Base (FB)}: Ratio between baseline cost vs. \sys. On average across traces, \sys is \textbf{1.4-20.0$\times$} cheaper than other baselines.} % (Always Evict: 20.0$\times$, Always Store: 2.2$\times$, $\teven$: 1.4$\times$, TTL-CC: 1.6$\times$, EWMA: 3.5$\times$, AWS Multi-Region Bucket: 3.1$\times$)
    \label{fig:2sites-update}
\end{figure*}


% Please add the following required packages to your document preamble:
\begin{table*}
\setlength\extrarowheight{5pt} % make the tables look less cramped
\centering
\resizebox{\textwidth}{!}{%
\Huge
\begin{tabular}{c|cccc|c|cccccc|cc|c|c|ccc}
\hline
 & \multicolumn{5}{c|}{\textbf{Size (\%)}} & \multicolumn{6}{c|}{\textbf{Read Frequency (\%)}} & \multicolumn{3}{c|}{\textbf{Request Arrival}} & \textbf{Recency} & \multicolumn{3}{c}{\textbf{Number of Requests}} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}IBM Trace\\Number\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# Tiny\\ (\textless{}1kB)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# Small\\ (1KB-1MB)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# Medium\\ (1MB-1GB)\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c|]{@{}c@{}}\# Large\\ (\textgreater{}1GB)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ (KB)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}One-Hit\\ Wonders\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Cold\\ (1--10)\end{tabular}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Warm\\ (10--100)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Hot\\ (100-1K)\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Super Hot \\ (\textgreater{}1K)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ \#GETs\end{tabular}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}\%in first 3\\ months\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\%in last 4\\ months\end{tabular}}} & \textbf{\begin{tabular}[|c]{@{}c@{}}Avg. GET Tail\\ months\end{tabular}} & \textbf{\begin{tabular}[c|]{@{}c@{}}Avg.\\ days\end{tabular}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}GET\\ (\%)\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}PUT\\ (\%)\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Total\\ (M)\end{tabular}}} \\ \hline
\rowcolor[HTML]{E3EEF9} 
T15 & {0} & {80} & 20 & {0} & 628 & \cellcolor[HTML]{DCEAF7}{\ul \textbf{48}} & 52 & {0} & {0} & \multicolumn{1}{c|}{\cellcolor[HTML]{E3EEF9}{0}} & 3 & 42 & 58 & 2.3 & 0.6 & {57} & {\ul \textbf{43}} & 1.6 \\
\rowcolor[HTML]{B7D4EA} 
T29 & {\ul \textbf{44}} & {56} & {0} & {0} & 3 & 2 & {\ul \textbf{98}} & {0} & {0} & \multicolumn{1}{c|}{\cellcolor[HTML]{B7D4EA}{0}} & 3 & 57 & 43 & 3.5 & {\ul \textbf{41.6}} & 70 & 30 & {\ul \textbf{13}} \\
\rowcolor[HTML]{6AAED6} 
T65 & {31} & {34} & {34} & {0.03} & 1,536 & 2 & 9 & 22 & {\ul \textbf{67}} & \multicolumn{1}{c|}{\cellcolor[HTML]{6AAED6} {\ul \textbf{0.1}}} & {\ul \textbf{93}} & 52 & 48 & 3 & 1.3 & {\ul \textbf{99}} & 1 & 0.3 \\
\rowcolor[HTML]{2E7EBC} 
{\color[HTML]{FFFFFF} T78} & {\color[HTML]{FFFFFF} 0} & {\color[HTML]{FFFFFF} {\ul \textbf{98}}} & {\color[HTML]{FFFFFF} 2} & {\color[HTML]{FFFFFF} 0} & {\color[HTML]{FFFFFF} 578} & {\color[HTML]{FFFFFF} 6} & {\color[HTML]{FFFFFF} 31} & {\color[HTML]{FFFFFF} {\ul \textbf{51}}} & {\color[HTML]{FFFFFF} 11} & \multicolumn{1}{c|}{\cellcolor[HTML]{2E7EBC}{\color[HTML]{FFFFFF} \ul \textbf{0.1}}} & {\color[HTML]{FFFFFF} 26} & {\color[HTML]{FFFFFF} 22} & {\color[HTML]{FFFFFF} \ul \textbf{78}} & {\color[HTML]{FFFFFF} 0.8} & {\color[HTML]{FFFFFF} 2.6} & {\color[HTML]{FFFFFF} 95} & {\color[HTML]{FFFFFF} 5} & {\color[HTML]{FFFFFF} 2.4} \\
\rowcolor[HTML]{084A91} 
{\color[HTML]{FFFFFF} T79} & {\color[HTML]{FFFFFF} 0} & {\color[HTML]{FFFFFF} 40} & {\color[HTML]{FFFFFF} {\ul \textbf{60}}} & {\color[HTML]{FFFFFF} {\ul \textbf{0.35}}} & {\color[HTML]{FFFFFF} \ul \textbf{48,386}} & {\color[HTML]{FFFFFF} 17} & {\color[HTML]{FFFFFF} {61}} & {\color[HTML]{FFFFFF} 22} & {\color[HTML]{FFFFFF} 0} & \multicolumn{1}{c|}{\cellcolor[HTML]{084A91} \color[HTML]{FFFFFF}{0}} & {\color[HTML]{FFFFFF} 9} & {\color[HTML]{FFFFFF} {\ul \textbf{60}}} & {\color[HTML]{FFFFFF} 40} & {\color[HTML]{FFFFFF} {\ul \textbf{4.1}}} & {\color[HTML]{FFFFFF} 8.3} & {\color[HTML]{FFFFFF} 89} & {\color[HTML]{FFFFFF} 11} & {\color[HTML]{FFFFFF} 0.1}
\end{tabular}%
}
\vspace{2pt}
\caption{IBM Trace Characteristics: each trace with characteristics highlighted with bold and underscore.}
\label{tab:trace_characteristics}
\end{table*}



\subsection{Deployment Settings \& Baselines}\label{eval:metrics_baselines_deploy}
% \shu{I like simple title: Baselines and Deployment Setup}
\subsubsection{Deployment settings and metrics}
\label{eval:deploy} 
In multi-cloud settings, we evaluate policies in two modes: fixed base (FB) and free placement (FP). By default, we assume FB mode where each object has a non-evictable base region. In FP mode, any replicas can be evicted, but at least one must remain. We compare \sys with SPANStore (Section~\ref{eval:baselines}) that operates only in FP mode. 
 \newline 
\textbf{Region Setup.} Our multi-cloud setup involves AWS S3, Azure Blob Storage, and GCS. We run 3-region\footnote{\path{aws:us-east-1}, \path{azure:eastus}, \path{gcp:us-east1-b}}, 6-region\footnote{\path{aws:us-east-1}, \path{aws:us-west-2}, \path{azure:eastus}, \path{azure:westus}, \path{gcp:us-east1-b}, \path{gcp:us-west1-a}}, and 9-region\footnote{\path{aws:us-east-1}, \path{aws:us-west-2}, \path{aws:eu-west-1}, \path{azure:eastus}, \path{azure:westus}, \path{azure:wasteurope}, \path{gcp:us-east1-b}, \path{gcp:us-west1-a}, \path{gcp:europe-west1-b}} experiments where we select 1, 2, and 3 regions from each cloud provider, respectively. \newline 
\textbf{Metrics} We calculate the monetary cost of storage and network for running a trace end-to-end, based standard storage pricings and bidirectional network cost between each cloud region. We ignore the base storage region cost in FB mode that is constant across all baselines. \shu{wordings ok?} We also measure average, p90, and p99 GET and PUT latency in our prototype evaluations.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TWO REGION GRAPHS %%%%%%%%%%%%%%%%%
\subsubsection{Baselines}

\label{eval:baselines}
% We measure the total cost in dollars incurred by \sys
%     and compare it against the following baselines.
% We also measure byte hit ratios in \sys and with
%     policies to estimate average read latency (see Appendix).

% \souj{Fix appendix reference here}

% We measure the total cost in dollars (i.e., storage and network costs) for the entire duration of each trace when executed with different policies. In our simulator, we calculate the byte hit ratio (\%) as the proportion of bytes that can be read from the local region and the average read latency (ms) (see Appendix). 

% We evaluate five traces in the 2-region base and cache setup and multi-cloud 3-region, 6-region, and 9-region. Our simulator evaluates all policies with the fixed base mode on a 2-region base and cache setting and with both fixed and free placement modes on the multi-cloud settings. 

We compare against the following baselines:
\begin{itemize}[noitemsep=*,leftmargin=*]
    \item 
    \textbf{Always Evict / Always Store} policy either stores each object in one storage location and never replicates, or always replicates objects to regions where GET is initiated and never evicts.

    % \item 
    % \textbf{Always Store} policy replicates objects to any
    % regions where a GET request is initiated. 
    
    \item
    \textbf{TTL-based Eviction} policies include 
    (a) $\tev=\teven$ (Section~\ref{eqn:teven}),
    (b) TTL-CC~\cite{TTLbasedCC2019}, a dynamic policy that stochastically sets TTL based on cached object behavior. 

    \item
    \textbf{Clairvoyant Greedy Policy (CGP)} (Section~\ref{sec:clairvoyant}) is an oracle that decides to store or evict given future access times of each object. CGP is cost-optimal under the 2-region. 
    % CGP is the most optimal policy.

    \item
    \textbf{EWMA}
    uses an Exponentially Weighted Moving Average \cite{ewma} to predict the next access time per object and chooses whether to evict it accordingly. We set the decay factor $\alpha$ to be 0.5. 
    % In addition, we design a simple baseline policy that uses the  
    % \cite{EWMA} 
    
    % SPANStore performs proactive replication on write, does not consider eviction and costs of replication, and requires the anticipated workload as input.
    % In our evaluation, SPANStore solver is fed with actual workloads which is its best-case scenario; note that, SPANStore only supports fixed base mode. \shu{this is not correct, it only support free placement mode}
    
    % We run SPANStore in a best-case scenario where the actual workloads, instead of predicted ones, are fed into its solver. We evaluate it only in the free placement mode because SPANStore does not fix a storage region. 

    \item
    \textbf{SPANStore} is a multi-cloud replication policy~\cite{spanstore} that replicates objects per hour to minimize access costs. We evaluate it only in the free placement (FP) mode because SPANStore does not fix a storage region. %We run SPANStore in a best-case scenario where the actual workloads are fed into its solver. 

    \item
    \textbf{Industrial Baselines} include AWS Multi-Region Buckets~\cite{aws-access-point} (and similarly, GCP Multi-Region Bucket~\cite{gcp-multi-region-bucket}) and JuiceFS~\cite{juicefs}. Upon PUT, an object is asynchronously replicated to the pre-configured secondary region(s). We evaluate AWS in a 2-region setup and JuiceFS in a multi-cloud setup, assuming object is replicated to all other regions. Our analysis excludes provider charges for these services. 
\end{itemize}

% Two-region base and cache setting: This setup represents a popular approach~\cite{separate-compute} where data is already located in one region like for low storage cost, but the computation is run elsewhere like for resource availability and low compute cost like geo-distributed model serving service. 





\subsection{Single-Cloud 2 Regions: Base and Cache}
\label{eval:two-region}



% In this setup, all PUTs are located in the base region, and all GETs occur in a separate cache region. We only evaluate storage and network costs from the cache regions and ignore the storage cost of the base region, as it is constant across all policies. 
We first evaluate \sys policy in a 2-region base and cache setup and show that our technique has merit as a standalone caching policy.  
    Figure~\ref{fig:2sites-update} compares the cost of \sys to six baseline policies across five traces (detailed in Section~\ref{eval:workloads-baselines-settings} and Table~\ref{tab:trace_characteristics}).
    \sys is, on average, 1.4-20$\times$ cheaper than the alternatives. 
    % The comparison shows how much more expensive each baseline is relative to \sys, with \sys being, on average, $1.4$-$20$$\times$ cheaper across traces than alternatives.
    % \natacha{You can shorten to ""GlboalStore is, on average, 1.4-20x cheaper than the alternatives}


While \sys performs consistently across workloads, alternative policies excel in specific cases but underperform elsewhere. 
For instance, Always Evict does well on one-hit-wonder heavy traces like T15 (48\% of one-hit-wonders) by avoiding unnecessary storage costs. 
    It is only 1.3$\times$ more expensive than \sys due to network cost paid for remaining objects with cold accesses. 
In traces (T29) with long recency between GETs (e.g., 1.5 months, beyond $\teven$) where storing data is more expensive than re-fetching it later, Always Evict is even 1\% cheaper \sys as it completely avoids caching. \sys reactively caches first and takes time to adjust its TTL in this case. 
    % In such cases, storing data for long is more expensive than evicting and re-fetching it later. Here, Always Evict performs marginally better (1\%) than \sys because \sys takes time to adjust its TTL. 
In contrast, 
    for T65 and T78 with primarily warm and hot objects and short recency (1.3-2.6 days), Always Evict incurs 73$\times$ and 23$\times$ higher costs due to frequent re-fetching data across regions. 
Surprisingly, 
    in T79, where 88\% of objects are one-hit-wonders or cold, Always Evict is still 2$\times$ worse than \sys.
    This is because T79's average object size is large (48MB), which makes network costs expensive due to the volume of data transferred.
On average, 
    \sys is 20$\times$ more cost-effective than the Always Evict. 



% \begin{table}[ht]
% \centering
% \small
% \setlength{\tabcolsep}{4pt} % Reduce horizontal padding
% \renewcommand{\arraystretch}{0.85} % Reduce vertical padding
% \begin{tabular}{lcccccc}
% \hline
% \textbf{Policy}       & \multicolumn{6}{c}{\textbf{Cost vs. Optimal}} \\
%                       & \textbf{T15} & \textbf{T29} & \textbf{T65} & \textbf{T78} & \textbf{T79} & \textbf{Avg} \\
% \hline
% Always Evict          & 1.38 & 1.03 & 77.45 & 27.75 & 3.14 & 22.15 \\
% Always Store          & 3.85  & 2.27  & 1.03  & 1.87  & 3.43  & 2.49  \\
% Teven                 & 1.89  & 2.15  & 1.03  & 1.44  & 1.45 & 1.59  \\
% TTL-CC                & 1.16  & 1.74  & 1.11  & 2.70  & 2.65 & 1.87  \\
% EWMA                  & 1.38  & 1.03  & 11.04  & 3.80  & 2.25  & 3.90  \\
% AWS Multi-Region Bucket & 6.30  & 3.50  & 1.04  & 2.84  & 3.79  & 3.49  \\
% \cellcolor{Gray}GlobalStore   & \cellcolor{Gray}1.09  & \cellcolor{Gray}1.04  & \cellcolor{Gray}1.07  & \cellcolor{Gray}1.23  & \cellcolor{Gray}1.32  & \cellcolor{Gray}1.15  \\ % Highlight the row with gray
% \hline
% \end{tabular}
% \vspace{0.5em}
% (\caption{Two-Region Base and Cache: Cost vs. Optimal across individual traces and their average.}
% \label{tab:cost_vs_optimal}
% \end{table}




Always Store replicates data on read and shows results opposite to Always Evict. 
It outperforms \sys by 3\% on hot-access traces like T65, where \sys incurs a few misses due to initial histogram adaptation delay that leads to higher network costs.
However, it struggles with T15 and T29 with infrequently or sporadically accessed objects, incurring 4$\times$ and 2$\times$ higher costs than \sys, respectively. 
Surprisingly, on T79, despite 80\% of objects being accessed more than once, Always Store is still 3$\times$ more expensive than \sys. 
This is due to the request pattern: 60\% of objects arrive in the first three months, with a 4.1-month average GET tail, causing Always Store to retain objects too long after their last access. Even on T78, which has 51\% of warm objects, \sys is 1.5$\times$ cheaper by evicting not-accessed objects earlier.
On average, \sys is 2.2$\times$ cheaper than Always Store. 

% \begin{figure*}[tbp]
%     \centering
%     \makebox[\textwidth][c]{%
%         \includegraphics[width=1.1\textwidth]{figures/nsdi/3_region_typeABCD_new.pdf}
%     }
%     \vspace{-2em}
%     \caption{\textbf{\sys v.s. Baselines in 3-Region, Fixed Base (FB), Four Workloads}: baseline over \sys is 0.94 to 120$\times$ across workloads and traces. \shu{Can this graph be longer than textwidth? too hard to see the numbers}}
%     %  Average across traces for each type, then take min and max across types: Always Evict: 9.3 -- 29.8$\times$, Always Store: 1.7 -- 1.8$\times$, $\teven$: 1.2 -- 1.3 $\times$, TTL-CC: 1.2 -- 1.8$\times$, EWMA: 2.9 -- 4.9$\times$, JuiceFS: 4.8 -- 6.7$\times$. 
%     \label{fig:3region-ABCD}
% \end{figure*}



The $\teven$ policy (Section~\ref{}) balances storage and network costs by keeping objects until re-fetching becomes as costly as storing. 
    In this setup, the average $\teven$ is 1 month, based on the ratio between average network cost and standard S3 prices across 22 AWS regions.
    $\teven$ performs best on T65, where all GETs occur within a month, allowing it to discard objects early and slightly outperform Always Store by 0.1\%. 
    However, it fails to account for workload patterns, leading to 1.7-2$\times$ higher costs than \sys on T15 and T29 as it retains infrequently accessed objects for too long. 
    On T78 and T79, which feature a moderate access frequency (a mix of one-hit, cold, and warm) and short recency (2-8 days), $\teven$ strikes a reasonable balance. However, because it relies solely on pricing and lacks workload awareness, \sys can still achieve 1.4$\times$ lower cost.
    On average, \sys is 1.4$\times$ more cost-effective than $\teven$. 
    
    % $\teven$ performs moderately well on T78 and T79, where most objects have a median of 1-100 accesses and short average recency (2-8 days). 
    % In these traces, $\teven$ strikes a reasonable balance by not evicting objects too early or storing them unnecessarily long. 
    % While $\teven$ is the best-performing baseline overall, it is still 1.4$\times$ more expensive than \sys, which can dynamically adjust to workload variations. 
    
    % However, this performance is more circumstantial than adaptive, as $\teven$ is less capable of adjusting to workload-specific variations compared to \sys.

TTL-CC\cite{TTLbasedCC2019} dynamically adjusts TTLs using a stochastic method based on cache hits and assumes a Poisson distribution, applying a single TTL across all objects. 
    It performs well (within 10\% of \sys) on T15 and T65, where patterns are dominated by many one-hit-wonders or hot object accesses.
    However, it struggles with more diverse access patterns, as in T78 and T79, where mixed object types (one-hit-wonders: 6-17\%, cold: 31-61\%, and warm: 22-51\%) exist. 
    Here, applying a single TTL across all objects results in 2$\times$ higher cost than \sys.
    In T29, TTL-CC over-retains sporadically accessed objects and pays higher storage costs, leading to a 1.7$\times$ higher cost.
    % In T29, despite the prevalence of cold objects and long recency, TTL-CC is 1.7$\times$ more expensive than \sys due to over-retaining objects based on sporadic hits.      
    Overall, real-world patterns are more complex than TTL-CC Poisson model, causing it to be 1.6$\times$ more expensive than \sys on average.



% EWMA is a policy that predicts the next access per object using an exponential weighted moving average and compares it with $\teven$ to decide whether to store it.
EWMA stores object with shorter predicted access times and evicts those with longer ones based on exponentially weighted moving averages. 
    It performs well in T15 (1.3$\times$) and T29 (0.99$\times$), quickly evicting one-hit and cold objects and minimizing storage costs. 
    However, in T65, T78, and T79, EWMA evicts objects too aggressively and pays higher network costs for misses. 
    While adaptive, EWMA’s decay factor needs fine-tuning for better cost efficiency. On average, it is 3.5$\times$ more expensive than \sys.

Commercial services like AWS Multi-Region Bucket~\cite{aws-access-point} behave like Always Store but proactively replicate data on write rather than read, leading to higher storage costs when GET appears later. In traces T15, T29, and T78 with PUT-GET gaps of 1-1.5 months, costs are 1.3-1.5$\times$ higher than Always Store and 2-6$\times$ higher than \sys. In shorter PUT-GET gap (less than 20 days) traces like T65 and T79, costs are comparable to Always Store and are 0.98-3$\times$ compared to \sys. 
Overall, AWS Multi-Region Bucket is 3.1$\times$ more expensive than \sys on average.

% We also evaluate CGP, the Oracle policy that achieves optimal cost in this setup (Table~\ref{tab:cost_vs_optimal}). On average, \sys operates within 15\% of the optimal cost, while others range from 1.6-22.2$\times$ higher. The 15\% difference is due to \sys aggregating access statistics at the bucket level, whereas CGP has an oracle knowledge of per-object granularity. \sys performs worse in T78 and T79 (1.2-1.3$\times$ than optimal) due to the mixed cold and warm objects with varying recencies, taking some time to adapt. In other traces, \sys remains within 10\% of optimal. We also show empirically that $\teven$ costs are within 2$\times$ of the optimal, as proven in Section~\ref{}. 



We also evaluate CGP, the Oracle policy with optimal cost (Table~\ref{tab:cost_vs_optimal}). On average, \sys operates within 15\% of optimal, while others range from 1.6-22.2$\times$ higher. The 15\% gap is due to \sys aggregating statistics at the bucket level, unlike CGP has oracle knowledge at per-object granularity. \sys performs slightly worse (1.2-1.3$\times$) on T78 and T79 than optimal due to a mix of object frequencies and recency, but remains within 10\% of optimal on other traces. We also show that $\teven$ costs are empirically within 2$\times$ of optimal, as proven in Section~\ref{}.

% \natacha{This section read well and was pretty clear! I realise that it's long, but it didn't feel overly detailed}

\begin{table}[ht]
\centering
\small
\setlength{\tabcolsep}{5pt} % Reduce horizontal padding
\renewcommand{\arraystretch}{0.85} % Reduce vertical padding
\begin{tabular}{lcccccc}
\hline
\textbf{Policy}       & \multicolumn{6}{c}{\textbf{Cost vs. Optimal}} \\
                      & \textbf{T15} & \textbf{T29} & \textbf{T65} & \textbf{T78} & \textbf{T79} & \textbf{Avg} \\
\hline
Always Evict          & 1.4 & 1.0 & 77.5 & 27.8 & 3.1 & 22.15 \\
Always Store          & 3.9  & 2.3  & 1.0  & 1.9  & 3.4  & 2.49  \\
Teven                 & 1.9  & 2.2  & 1.0  & 1.4  & 1.5 & 1.59  \\
TTL-CC                & 1.2  & 1.7  & 1.1  & 2.7  & 2.7 & 1.87  \\
EWMA                  & 1.4  & 1.0  & 11.0  & 3.8  & 2.3  & 3.90  \\
AWS Multi-Region Bucket & 6.3  & 3.5  & 1.0  & 2.8  & 3.8  & 3.49  \\
\cellcolor{Gray}GlobalStore   & \cellcolor{Gray}1.1  & \cellcolor{Gray}1.0  & \cellcolor{Gray}1.1  & \cellcolor{Gray}1.2  & \cellcolor{Gray}1.3  & \cellcolor{Gray}1.14  \\ % Highlight the row with gray
\hline
\end{tabular}
\vspace{0.3em}
\caption{Two-Region Base and Cache: Cost vs. Optimal across individual traces and their average.}
\label{tab:cost_vs_optimal}
\end{table}

\begin{table}%[ht]
\centering
\small
\setlength{\tabcolsep}{1.8pt} % Adjust horizontal padding
\renewcommand{\arraystretch}{0.9} % Moderate vertical padding
\begin{tabular}{lccccc} 
\toprule
\textbf{Policy} & \makecell{\textbf{Type A} \\ (Uniform)} & \makecell{\textbf{Type B} \\ (Region)} & \makecell{\textbf{Type C} \\ (Aggregation)} & \makecell{\textbf{Type D} \\ (Replication)} & \textbf{Average} \\
\midrule
Always Evict & 9.3 & 29.8 & 24.0 & 10.4 & 18.4$\times$ \\
Always Store & 1.8 & 1.7 & 1.7 & 1.9 & 1.8$\times$ \\
$\teven$ & 1.3 & 1.3 & 1.3 & 1.3 & 1.3$\times$ \\
TTL-CC & 1.7 & 1.2 & 1.3 & 1.8 & 1.5$\times$ \\
EWMA & 2.9 & 4.9 & 4.4 & 3.0 & 3.8$\times$ \\
JuiceFS & 4.8 & 1.9 & 1.9 & 4.8 & 5.7$\times$ \\
\bottomrule
\end{tabular}
\vspace{0.8em}
\caption{3-Region Fixed Base: baseline cost over \sys ($\times$), averaged across traces and across workload types.}
\label{tab:cost_comparison_3_region_avg}
\end{table}



% Report everything
% \begin{table}[ht]
% \centering
% \small
% \setlength{\tabcolsep}{4pt} % Reduce horizontal padding
% \renewcommand{\arraystretch}{0.9} % Reduce vertical padding
% \begin{tabular}{lcccccc}
% \hline
% \textbf{Policy}       & \multicolumn{6}{c}{\textbf{Cost vs. Optimal}} \\
%                       & \textbf{T15} & \textbf{T29} & \textbf{T65} & \textbf{T78} & \textbf{T79} & \textbf{Avg} \\
% \hline
% Always Evict          & 1.38 & 1.03 & 77.45 & 27.75 & 3.14 & 22.15 \\
% Always Store          & 3.85  & 2.27  & 1.03  & 1.87  & 3.43  & 2.49  \\
% Teven                 & 1.89  & 2.15  & 1.03  & 1.44  & 1.45 & 1.59  \\
% TTL-CC                & 1.16  & 1.74  & 1.11  & 2.70  & 2.65 & 1.87  \\
% EWMA                  & 1.38  & 1.03  & 11.04  & 3.80  & 2.25  & 3.90  \\
% AWS Multi-Region Bucket & 6.30  & 3.50  & 1.04  & 2.84  & 3.79  & 3.49  \\
% \cellcolor{Gray}GlobalStore   & \cellcolor{Gray}1.09  & \cellcolor{Gray}1.04  & \cellcolor{Gray}1.07  & \cellcolor{Gray}1.23  & \cellcolor{Gray}1.32  & \cellcolor{Gray}1.15  \\ % Highlight the row with gray
% \hline
% \end{tabular}
% \vspace{0.5em}
% \caption{Two-Region Base and Cache: Cost vs. Optimal across individual traces and their average.}
% \label{tab:cost_vs_optimal}
% \end{table}







% Just report average 
% \begin{table}[ht]
% \centering
% \small
% \setlength{\tabcolsep}{4pt} % Reduce horizontal padding
% \renewcommand{\arraystretch}{0.9} % Reduce vertical padding
% \begin{tabular}{lc}
% \hline
% \textbf{Policy}       & \textbf{Cost vs. Optimal} \\
% \hline
% Always Evict  & 22.15 \\
% Always Store  & 2.49  \\
% Teven         & 1.59  \\
% TTL-CC        & 1.87  \\
% EWMA          & 3.90  \\
% AWS Multi-Region Bucket & 3.49  \\
% \cellcolor{Gray}GlobalStore   & \cellcolor{Gray} 1.15  \\ % Highlight the last row with gray
% \hline
% \end{tabular}
% \vspace{0.5em}
% \caption{Two-Region: Average cost vs. Optimal across traces.}
% \label{tab:cost_vs_optimal}
% \end{table}
 
% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=1\textwidth]{figures/nsdi/3_region_typeABCD_new.pdf}
%     \vspace{-2em}
%     \caption{\textbf{\sys v.s. Baselines in 3-Region, Fixed Base (FB), Type A-D}:  across traces, on average, \sys is 1.2 -- 9.3$\times$ cheaper compared to the six other baselines on Type A, 1.2 -- 29.8$\times$ cheaper on Type B, 1.3 -- 24.0$\times$ cheaper on Type C, and 1.3 -- 10.4$\times$ cheaper on Type E. Average across traces for each type, then take min and max across types: Always Evict: 9.3 -- 29.8$\times$, Always Store: 1.7 -- 1.8$\times$, $\teven$: 1.2 -- 1.3 $\times$, TTL-CC: 1.2 -- 1.8$\times$, EWMA: 2.9 -- 4.9$\times$, JuiceFS: 4.8 -- 6.7$\times$}
%     \label{fig:3region-ABCD}
% \end{figure*}

% \vspace{-20pt}
\vspace{-2em}
\subsection{Multi-Cloud: 3 Regions}
\label{eval:three-region}



Our evaluation extends to a 3-region, 3-cloud setup (Section~\ref{eval:deploy}) in fixed base (FB) mode using five traces across four workloads described in Section~\ref{eval:multi-cloud-generation}: uniform, region-aware, aggregation, and replication. 
Region-aware and aggregation workloads concentrate GETs of single or multiple objects in one region. Uniform and replication workloads distribute GETs across regions, leading to sparser and longer recency access. 
We evaluate JuiceFS instead of AWS Multi-Region Bucket as the latter does not operate across clouds. Table~\ref{tab:cost_comparison_3_region_avg} summarizes the baseline cost over \sys cost, averaging across traces per type and workload types. 
% Figure~\ref{fig:3region-ABCD} and 
% \natacha{say why you switch to JuiceFS over AWS Multi-Region (even if it's obvious}
% We observe that policy performance across traces in 3-region setups largely mirrors 2-region, but cost ratios differ across workloads. In summary, \sys outperforms baselines by 1.2 -- 29.8$\times$ averaging across traces and workloads (Table~\ref{tab:cost_comparison_3_region_avg}). 

% \natacha{What do you mean by cost ratio here? If it's true that it largely mirrors the 2-region setup, I would significantly condense the summary, and only highlight the most important/interesting differences? Edit: post slack conversation, I'd say: only the relative performance number changes}

In summary, 3-region multi-cloud results largely mirror the 2-region setup. The trends across traces remain the same, but the absolute numbers differ from the 2-region setup and differ across workloads. The primary reason why they change from 2-region is because of higher (1.8$\times$) network fees in multi-cloud compared to single-cloud. Across workloads, we show how different policies behave differently, as shown below. Overall, \sys continues to outperform baselines by a factor of 1.2 to 29.8 on average. 
% while its worst-case performance is within 6\% of the best-performing baseline. 


% policy performance trends across traces in a 3-region multi-cloud setup largely mirrors the 2-region setup, but the relative performance number changes across workloads. Type B (region-aware) and Type C (aggregation) workloads concentrate GETs in one region, showing similar cost results. In contrast, Type A (uniform) and Type D (replication) workloads distribute GETs across regions, leading to sparser and longer recency access. Different policies react differently to this change. As we go from single-cloud to multi-cloud, \sys outperforms baselines by 1.2 -- 29.8$\times$ (Table~\ref{tab:cost_comparison_3_region_avg}).  \nc{I'd move the results to right after you talk about cost ratios.}

% \natacha{Are egress fees always the reason for why the relative cost changes? If yes, I'd maybe just say that and structure the paragraph:
% 1) 3-region multicloud results largely mirror the 2 region setup; trends remain the same but absolute numbers differ. GlobalStore continus to outperform baselines by a factor of X to Y. Type B ... Different policies react ... The primary reason for why absolute numbers change is because of egress fees (or something alone those lines)}

Always Evict is 9.3-29.8$\times$ more expensive than \sys on average. 
    It performs slightly better (9.3$\times$ and 10.4$\times$ vs. \sys) in uniform and replication workloads. 
    As GETs per object are distributed, all policies have uniformly high network costs of cold misses in each region. Thus, their performance gap is narrower. 
    In contrast, Always Evict performs worse (29.8$\times$ and 24.0$\times$) in region-aware and aggregation workloads; in read-heavy traces like T65, it can be 120$\times$ worse due to high cross-cloud network fees. 
    % Multi-cloud egress fees are 1.8$\times$ more expensive than a 2-region setup; thus, Always Evict pays a much higher network cost for a cache miss. 
    % Always Evict performs well in T15 and T29 with low frequency and long recency patterns, where workload types have less impact on these characteristics.
    Similarly, EWMA performs close to Always Evict except that it retains objects for slightly longer in read-heavy traces, costing 2.9 -- 4.9$\times$ more than \sys on average. 

\begin{figure*}[tbp]
    \centering
    \includegraphics[width=\textwidth]{figures/nsdi/scalability_3_6_9.pdf}
    \vspace{-2em}
    % \caption{\textbf{\sys Cost Savings (\%) on 2-Region, Fixed Base (FB)}: \sys achieves on average 1.4-20.0$\times$ cost savings over 5 traces and 5 baselines.}
    \caption{\textbf{\sys Total Cost on 3, 6, and 9 Regions across Workloads A-D: Cost is normalized over 3-region cost.}}
    \label{fig:3-6-9-scalability}
\end{figure*}

Always Store and JuiceFS are on average 1.7–1.9$\times$ and 1.9–4.8$\times$ more costly than \sys, respectively.  
Decreasing access frequency and increasing recency reduce the benefit of storing data. 
Thus, Always Store excels (1.7$\times$ vs. \sys) in region-aware and aggregation workloads but underperforms (1.8 -- 1.9$\times$) in uniform and replication workloads.
In T65, Always Store outperforms \sys by 4-6\% due to heavy reads and high network costs, while \sys incurs slightly higher costs during initial adaptation.
On the other hand, JuiceFS performs 2.7$\times$ worse than Always Store in uniform and replication workloads, incurring high network and storage costs by replicating to all regions upon each PUT, even without future GETs. In region-aware and aggregation workloads, JuiceFS costs are similar to Always Store given a pre-defined replication region, with a slight increase due to storage costs.



% Thus, it performs on average better (1.2-1.3$\times$) in region-aware and aggregation workloads where trace patterns are more concentrated in one region and worse (1.7-1.8$\times$) in uniform or replication workloads. 

% where trace patterns are more concentrated in one region
% than the other two workloads because it decides to store for shorter when GETs are spread, and it observes lower hits in each region
% TTL-CC behaves more like Always Evict due to sparse GETs, and frequent eviction in such workloads for T79 is a more cost-effective strategy. But when trace patterns are concentrated in one region, there is a mix of cold, warm, ont-hit accesses, and as TTL-CC only set one TTL per object, it performs worse. 

% For example, in Trace 29, TTL-CC behaves similarly to Always Evict in Type A due to sparse GETs but resembles Always Store in Type C because of the dense accesses. 
% In Trace 65, TTL-CC performs closer to Always Store across both types, but the higher network cost of Type A leads to worse performance compared to \sys.

% An interesting observation with TTL-CC is in Type A and Type C of Trace 79, where it shows similar performance. The key difference lies in the network and storage costs—Type A’s higher network cost penalizes mistakes more severely, leading to higher overall costs compared to Type C, where GETs are more likely to occur in the same region. This behavior highlights the limitations of applying a single global TTL in more complex multi-region scenarios.


TTL-CC costs 1.2 -- 1.8$\times$ more than \sys on average, adjusting its TTL longer with more cache hits. It performs on average better (1.2-1.3$\times$ vs. \sys) in region-aware and aggregation workloads, but worse (1.7-1.8$\times$) in uniform or replication workloads. 
For example, in T65, TTL-CC incurs 3.6-4.5$\times$ higher cost in uniform and replication workloads due to fewer hits in each region, and thus shorter storage times and increased re-fetch costs. 
An exception is T79, where TTL-CC performs 1.6$\times$ better in uniform and replication workloads by adapting to colder access patterns but struggles with mixed cold and warm accesses in region-aware and replication workloads. 
% than region-aware and replication workloads. In the latter two workloads for T79, mixed of cold and warm accesses are concentrated in one region, making TTL-CC less adaptable as it sets a single TTL for all objects. However, in uniform and replication workloads, TTL-CC effectively learns the colder access patterns, leading to more cost-effective evictions.




% The $\teven$ policy shows the strongest performance over other baselines, costing 1.3$\times$ more than \sys on average. This policy performs roughly the same no matter how requests are distributed, striking a good balance between storage and network costs in multi-cloud. 
The $\teven$ policy continues to perform strongly, averaging 1.3$\times$ higher cost than \sys. It maintains similar performance across different request distributions, balancing storage and network costs well in multi-cloud.
In T15, T29, and T78, for uniform and replication workloads with sparse GETs, $\teven$ costs 1.1-1.7$\times$ more than \sys due to unnecessary storage for objects even though there are no next GETs. 
% In T79, it performs slightly better (1.2$\times$) in uniform or replication workloads than in region-aware and aggregation workloads. This is because, in uniform and replication workloads, sparse reads make \sys evict more and thus pay for higher network costs. 
% \natacha{As a rule of thumb, I'd say: if you've already said this in the previou section, don't include it here}
% analysis is not true here!! teven will not pay for more storage cost if increase region 


% As the number of regions increases and grows from single-cloud to multi-cloud, the differentiation between placement strategies decreases. However, \sys still demonstrates a strong ability to optimize costs. 
% The findings emphasize how multi-cloud setups increase the importance of dynamic adaptation, with \sys providing significant cost savings compared to static policies like Always Evict, Always Store, and TTL-CC.

\subsection{Multi-Cloud: Scale to 6 and 9 Regions}
\label{eval:nine-region}



%%%%%%%%%%%% COMBINE TABLE %%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\small
\begin{tabular}{lcccccc}
\toprule
\textbf{Policy} & \multicolumn{2}{c}{\textbf{3-Region (FB)}} & \multicolumn{2}{c}{\textbf{6-Region (FB)}} & \multicolumn{2}{c}{\textbf{9-Region (FB)}} \\
\cmidrule{2-7}
& \textbf{Avg} & \textbf{Std Dev} & \textbf{Avg} & \textbf{Std Dev} & \textbf{Avg} & \textbf{Std Dev} \\
\midrule
\textit{Always Evict} & 18.4 & 31.6 & 15.0 & 27.0 & 12.9 & 23.9 \\
\textit{Always Store} & 1.8 & 0.7 & 2.0 & 0.8 & 2.1 & 0.8 \\
\textit{Teven} & 1.3 & 0.3 & 1.4 & 0.3 & 1.4 & 0.3 \\
\textit{TTL-CC} & 1.5 & 1.0 & 1.3 & 0.5 & 1.4 & 0.7 \\
\textit{EWMA} & 3.8 & 4.7 & 3.2 & 3.4 & 3.1 & 3.4 \\
\textit{JuiceFS} & 3.4 & 2.9 & 7.3 & 7.2 & 8.6 & 10.9 \\
\midrule
\textbf{Policy} & \multicolumn{2}{c}{\textbf{3-Region (FP)}} & \multicolumn{2}{c}{\textbf{6-Region (FP)}} & \multicolumn{2}{c}{\textbf{9-Region (FP)}} \\
\cmidrule{2-7}
& \textbf{Avg} & \textbf{Std Dev} & \textbf{Avg} & \textbf{Std Dev} & \textbf{Avg} & \textbf{Std Dev} \\
\midrule
\textit{Always Evict} & 11.9 & 21.1 & 11.4 & 22.4 & 11.4 & 23.4 \\
\textit{Always Store} & 1.3 & 0.2 & 1.4 & 0.2 & 1.5 & 0.2 \\
\textit{JuiceFS} & 1.7 & 0.6 & 3.0 & 1.8 & 3.5 & 2.8 \\
\textit{SPANStore} & 1.4 & 0.2 & 1.5 & 0.2 & 1.6 & 0.3 \\
\bottomrule \\
\end{tabular}%
\caption{3, 6, 9-Region, 5 traces, Type A-D, Fixed Base (FB) and Free Placement (FP): Average and standard deviation of cost of baselines over \sys.}
\vspace{-2em}
\label{table:avg_std_combined}
\end{table}
%%%%%%%%%%%% COMBINE TABLE %%%%%%%%%%%%%%%%%%%%%%


We now explore how different policy scales from 3 to 6 and 9 regions in both fixed base (FB) and free placement (FP) modes. 
In FP mode, \sys is compared to Always Evict, Always Store, and commercial/academic baselines like JuiceFS and SPANStore.
We evaluate SPANStore only in FP mode as it does not support a fixed storage region. 

Figure~\ref{fig:3-6-9-scalability} shows how \sys cost scales from 3 to 9 regions per workload type across traces in FB mode. 
Region-aware and aggregation-workloads (Figure~\ref{fig:3-6-9-scalability}b, ~\ref{fig:3-6-9-scalability}c) show minimal cost variation when scaling to more regions. This is because no matter how the region scales, GETs of a single object are still concentrated in a single region. 
One exception is that the T65 aggregation workload experiences a slightly higher cost scaling to the 6 and 9 regions. This increase is due to the selection of the GET region (\texttt{aws:us-east-1}), which has a slightly higher network ingress cost when scaling to 6 and 9 region. 
For uniform and replication workloads (Figure~\ref{fig:3-6-9-scalability}a, ~\ref{fig:3-6-9-scalability}d), the cost also remains relatively stable even as regions increase. This is particularly evident in traces originally with cold accesses (T15, T29, and T79), where scaling to 9 regions yields similar costs. However, for traces with lots of warm and hot objects, such as T65 and T78,  cost increases proportionally (i.e., around 1.5$\times$ and 1,2$\times$) as GET requests are distributed across more regions, causing higher cold miss network costs per object for more regions. 

% In region-aware and aggregation workloads (Figure~\ref{fig:3-6-9-scalability}b, ~\ref{fig:3-6-9-scalability}c), 3, 6, and 9 region workloads are more or less similar, with slight variations due to slightly higher network cost variances when scaling to more regions. Scaling to 9 regions in aggregation workloads leads to slightly more cost increase for T65 than region-aware workload because we random sample to pick \texttt{aws:us-east-1} as the GET region for all objects, and as region scales, the ingress cost to this region becomes slightly more expensive than the average network cost used in region-aware workload.

Table~\ref{table:avg_std_combined} illustrates how scaling affects baseline costs relative to \sys.
In fixed base (FB) mode, Always Evict and EWMA improve relative performance as the number of regions increases (18.4 to 12.9$\times$, 3.8 to 3.1$\times$, respectively).
Sparse access frequencies and long recency make eviction a better choice and make cold miss network cost higher for \sys, narrowing the relative performance gap. 
% as access frequencies are sparse in each region, thus \sys also needs to pay for cold miss network cost, making the performance gap smaller. 
On the other hand, Always Store and JuiceFS become worse (1.8 to 2.1$\times$, 3.4 to 8.6$\times$, respectively) compared to \sys as regions increase. More regions lead to more replicas that contribute to higher storage costs, and these policies never evict. JuiceFS experiences significant scaling inefficiencies due to its proactive replication strategy, replicating to all the other regions upon PUT and paying for higher storage and network costs as regions scale.  
Both $\teven$ and TTL-CC remain fairly consistent (1.3-1.4$\times$ and 1.3-1.5$\times$), showing only slight fluctuations in relative cost compared to \sys from 3 to 9 regions.
% $\teven$ and TTL-CC remain roughly similar, around 1.3-1.4 $\times$ and 1.3-1.5 $\times$ more expensive than \sys, respectively. TTL-CC performs slightly better with more regions due to more distinct sparse access patterns in each region. 

In FP mode, the relative cost numbers compared to \sys are slightly lower than in FB mode due to additional no-base region storage costs for all baselines. SPANStore, a state-of-the-art multi-region replication policy, performs similarly to Always Store since it does not remove long-unused objects. In some traces like T29 and T79, it performs worse by pushing data to regions that are rarely accessed. We evaluate SPANStore with a best-case scenario, given its solver the oracular workload knowledge. \sys is 1.4 to 1.6$\times$ cheaper than SPANStore across traces and workloads, scaling from 3 to 9 regions.

% In FP mode, we draw similar conclusions, with the relative cost number compared to \sys slightly lower than in FB mode because of the additional no-base region storage cost. We evaluate state-of-the-art multi-region replication policy SPANStore. It performs similarly to the Always Store policy as it does not consider removing objects in the accessed sets, even if these objects have not been accessed for a long time. In reality, SPANStore can sometimes perform worse than the Always Store policy when it erroneously pushes data to regions where reads are rare. We show that \sys is 1.4 to 1.6$\times$ cheaper compared to SPANStore scaling to 9 region across traces and workloads, even when the latter system is given oracular workload knowledge.

% \begin{enumerate}
%     \item We show the \sys normalized total cost over 3-region cost results and demonstrate that across workload types, we scale our cost. The boost in T65 in Type A and D is due to heavy repeated reads across regions, and if those GETs get distributed across regions any poilcy have to pay for high network cost for cold miss. 
%     \item Fixed base: more regions we have, always evict perform better, always store perform worse. $\teven$ also perform slightly worse scaling to more regions, as there are diversity in network costs going from 3 to 6 to 9, making it hard if just taking average ratio. In more regions, GETs are sparse, TTL-CC and EWMA behaves like Always Evict and adapt to sparse access pattern, thus becoming better. Replicate on write method does not scale with more regions, as it naively replicates to all other regions.
%     \item Free placement: we also evaluate our baseline SPANStore in free placement mode, and show that it does not scale with more regions. Free placement modes generally produces lower differnce of policy v.s. ours because the base storage cost is higher. 
% \end{enumerate}

%%%%%%%%%%%% SEPARATE TABLE %%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Policy} & \multicolumn{2}{c}{\textbf{3-Region (FB)}} & \multicolumn{2}{c}{\textbf{6-Region (FB)}} & \multicolumn{2}{c}{\textbf{9-Region (FB)}} \\
% \cmidrule{2-7}
% & \textbf{Avg} & \textbf{Std Dev} & \textbf{Avg} & \textbf{Std Dev} & \textbf{Avg} & \textbf{Std Dev} \\
% \midrule
% \textit{Always Evict} & 18.4 & 31.6 & 15.0 & 27.0 & 12.9 & 23.9 \\
% \textit{Always Store} & 1.8 & 0.7 & 2.0 & 0.8 & 2.1 & 0.8 \\
% \textit{Teven} & 1.3 & 0.3 & 1.4 & 0.3 & 1.4 & 0.3 \\
% \textit{TTL-CC} & 1.5 & 1.0 & 1.3 & 0.5 & 1.4 & 0.7 \\
% \textit{EWMA} & 3.8 & 4.7 & 3.2 & 3.4 & 3.1 & 3.4 \\
% \textit{JuiceFS} & 3.4 & 2.9 & 7.3 & 7.2 & 8.6 & 10.9 \\
% \bottomrule \\
% % \cmidrule{2-7}
% % & \textbf{Avg} & \textbf{Std Dev} & \textbf{Avg} & \textbf{Std Dev} & \textbf{Avg} & \textbf{Std Dev} \\
% % \midrule
% % \textit{Always Evict} & 18.38 & 31.58 & 14.93 & 27.06 & 12.89 & 23.85 \\
% % \textit{Always Store} & 1.76 & 0.65 & 2.05 & 0.77 & 2.13 & 0.82 \\
% % \textit{Teven} & 1.27 & 0.31 & 1.39 & 0.28 & 1.37 & 0.28 \\
% % \textit{TTL-CC} & 1.49 & 1.01 & 1.34 & 0.51 & 1.38 & 0.65 \\
% % \textit{EWMA} & 3.80 & 4.65 & 3.18 & 3.44 & 3.05 & 3.42 \\
% % \textit{JuiceFS} & 3.36 & 2.87 & 7.33 & 7.20 & 8.60 & 10.85 \\
% % \bottomrule \\
% \end{tabular}%
% \caption{3, 6, 9-Region, Fixed Base, Type A-D: Average and standard deviation of cost of baselines over \sys.}
% \vspace{-2em}
% \label{table:avg_std}
% \end{table}
% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Policy} & \multicolumn{2}{c}{\textbf{3-Region (FP)}} & \multicolumn{2}{c}{\textbf{6-Region (FP)}} & \multicolumn{2}{c}{\textbf{9-Region (FP)}} \\
% \cmidrule{2-7}
% & \textbf{Avg} & \textbf{Std Dev} & \textbf{Avg} & \textbf{Std Dev} & \textbf{Avg} & \textbf{Std Dev} \\
% % \midrule
% % \textit{Always Evict} & 11.91 & 21.05 & 11.41 & 22.41 & 11.35 & 23.38 \\
% % \textit{Always Store} & 1.28 & 0.15 & 1.41 & 0.17 & 1.50 & 0.19 \\
% % \textit{Teven} & 1.00 & 0.06 & 1.09 & 0.24 & 1.11 & 0.15 \\
% % \textit{TTL-CC} & 1.00 & 0.07 & 1.14 & 0.49 & 1.64 & 2.04 \\
% % \textit{EWMA} & 1.79 & 1.88 & 1.65 & 1.39 & 2.21 & 1.73 \\
% % \textit{SPANStore} & 1.41 & 0.19 & 1.46 & 0.24 & 1.55 & 0.29 \\
% % \textit{JuiceFS} & 1.73 & 0.62 & 3.04 & 1.82 & 3.54 & 2.76 \\
% % \bottomrule \\
% \midrule
% \textit{Always Evict} & 11.9 & 21.1 & 11.4 & 22.4 & 11.4 & 23.4 \\
% \textit{Always Store} & 1.3 & 0.2 & 1.4 & 0.2 & 1.5 & 0.2 \\
% % \textit{Teven} & 1.0 & 0.1 & 1.1 & 0.2 & 1.1 & 0.2 \\
% % \textit{TTL-CC} & 1.0 & 0.1 & 1.1 & 0.5 & 1.6 & 2.0 \\
% % \textit{EWMA} & 1.8 & 1.9 & 1.7 & 1.4 & 2.2 & 1.7 \\
% \textit{JuiceFS} & 1.7 & 0.6 & 3.0 & 1.8 & 3.5 & 2.8 \\
% \textit{SPANStore} & 1.4 & 0.2 & 1.5 & 0.2 & 1.6 & 0.3 \\
% \bottomrule \\
% \end{tabular}%
% \caption{3, 6, 9-Region, Free Placement, Type A-D: Average and standard deviation of cost of baselines over \sys.}
% \vspace{-2em}
% \label{table:avg_std}
% \end{table}
%%%%%%%%%%%% SEPARATE TABLE %%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Multi-Cloud: End-to-End Benchmark}
\label{eval:end-to-end}
% \shu{ack everything is done in simulation because of cost, see what we expect; --> not going back to simulation; revision, keep it clean; until before: it is cost, representative example, get some latency results (why not simulate the other ones)}
% \begin{table}[ht]
% \centering
% \small
% \setlength{\tabcolsep}{4pt} % Adjust horizontal padding
% \renewcommand{\arraystretch}{1.2} % Moderate vertical padding
% \begin{tabularx}{\linewidth}{l*{3}{X}*{3}{X}p{1cm}p{1cm}} % Increased width of the last two columns
% \toprule
% \textbf{Policy} & \multicolumn{3}{c}{\makecell{\textbf{GET} \\ \textbf{Latency (ms)}}} & \multicolumn{3}{c}{\makecell{\textbf{PUT} \\ \textbf{Latency (ms)}}} &  \makecell{\textbf{GET Lat.} \\ \textbf{vs. AS} \\ \textbf{}} & \makecell{\textbf{Cost (\$)} \\ \textbf{vs. AS}} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} % Lines under GET and PUT sections only
%  & \textbf{Avg} & \textbf{P90} & \textbf{P99} & \textbf{Avg} & \textbf{P90} & \textbf{P99} & \textbf{} & \\
% \midrule
% Always Store & 172 & 235 & 340 & 840 & 562 & 784 & 1$\times$ & 1.0$\times$ \\
% Always Evict & 278 & 440 & 762 & 800 & 507 & 715 & 1.6$\times$ & 76.78$\times$ \\
% GlobalStore  & 178 & 232 & 762 &  &  &  & 1.0$\times$ & 1.05$\times$ \\
% \bottomrule
% \end{tabularx}
% \vspace{0.8em}
% \caption{End-to-End System Evaluation: T65 (hot objects, mix of size).}
% \label{tab:end_to_end_result}
% \end{table}

\begin{table}[ht]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt} % Adjust horizontal padding
\renewcommand{\arraystretch}{1.2} % Moderate vertical padding
\begin{tabularx}{\linewidth}{l*{3}{>{\centering\arraybackslash}X}*{3}{>{\centering\arraybackslash}X}p{1.2cm}p{1.1cm}} % Reduced width of the last two columns for better fit
\toprule
\textbf{Policy} & \multicolumn{3}{c}{\makecell{\textbf{GET} \\ \textbf{Latency (ms)}}} & \multicolumn{3}{c}{\makecell{\textbf{PUT} \\ \textbf{Latency (ms)}}} & {\makecell{\textbf{GET Lat.} \\ \textbf{vs. AS}}} & {\makecell{\textbf{Cost (\$)} \\ \textbf{vs. AS}}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} % Lines under GET and PUT sections only
 & \textbf{Avg} & \textbf{P90} & \textbf{P99} & \textbf{Avg} & \textbf{P90} & \textbf{P99} &  & \\
\midrule
Always Store & 172 & 235 & 340 & 840 & 562 & 784 & 1.00$\times$ & 1.00$\times$ \\
Always Evict & 278 & 440 & 762 & 800 & 507 & 715 & 1.61$\times$ & 76.78$\times$ \\
GlobalStore  & 184 & 230 & 408 & 822 &  520 & 782 & 1.06$\times$ & 1.05$\times$ \\
\bottomrule
\end{tabularx}
\vspace{0.5em}
\caption{End-to-End System Evaluation on T65.}
\label{tab:end_to_end_result}
\end{table}
\vspace{-2em}
So far, results in the previous evaluations are based on cost simulations. Now, we present an end-to-end system evaluation using the T65 trace (0.3M requests), comparing the performance of Always Store, Always Evict, and \sys across GET/PUT latencies and costs relative to Always Store. The results are shown in Table~\ref{tab:end_to_end_result}.
% We want to demonstrate when running a 0.3 million trace end-to-end, \sys metadata, histogram collections, and background eviction does not add much to the overheads. 
Always Store achieves the best GET latency, with an average of 172 ms and a P99 of 340 ms, due to its full caching strategy. Always Evict, which avoids local caching, has significantly higher latencies (1.6$\times$ slower than Always Store) with a P99 of 762 ms. \sys delivers comparable performance to Always Store, with only a slight 3\% increase in GET latency due to histogram collection for workload adaptation. PUT latencies are consistent across policies, as writes are directed locally. In terms of cost, Always Store offers the lowest baseline, aligning with previous 2- and 3-region results in Section~\ref{eval:two-region} and Section~\ref{eval:three-region}. Always Evict incurs up to 76.78$\times$ higher costs, while \sys achieves nearly the same cost as Always Store (within 5\%), with only a slight latency increase (1.06$\times$) due to its background eviction process.

% \sys prioritizes cost objectives and an effort to retain objects locally if the cost is not too high. In a read-heavy workload, it performs closest to the best-performing replication on the read baseline (see Section~\ref{eval:end-to-end}). Due to budget constraints, we profile inter-region access latency and throughput for 3-regions and simulate the latency across baselines in a long-recency workload, shown in Table~\ref{tab:end_to_end_simulate_29}. We show that \sys achieves 2.3$\times$ cheaper than Always Store, at only a 24\% increase in latency. 
% In terms of cost, Always Store, with its aggressive caching strategy, provides the best baseline cost. By contrast, Always Evict incurs the highest cost, up to 76.78$\times$ more expensive. \sys performs nearly as well the cost and latency to the best-performing Always Store in this trace, achieving cost savings within 5\% of Always Store (additional 5\% for initial histogram adaptation) and a slight latency increase of 1.06$\times$ due to background eviction process. 


\subsection{Overheads and Trade-offs}
\label{eval:overheads}
\shu{Not done yet}

% \subsubsection{Operational Overheads}
% \subsubsection{Histogram Overhead}
\subsubsection{What is \sys cost overhead?}

\subsubsection{What is \sys system overhead?}
\begin{figure}
    % \centering
    \includegraphics[width=.75\linewidth]{figures/juicefs.pdf}
    \caption{\sys System Performance v.s. AWS APIs: client, server, and object store on region \textit{aws:us-east-2}.}
    \label{fig:proxy-overhead}
    \vspace{-2em}
\end{figure}


Using the JuiceFS benchmark, we evaluate \sys's overhead compared to direct usage of the cloud provider’s API. The benchmark includes put, get, list, head, and delete operations on 10K objects (128 KB each), measuring average latency per operation. As shown in Fig. \ref{fig:proxy-overhead}, \sys adds less than 10\% overhead for put and get operations due to the round-trip time to the metadata server. Additionally, \sys improves list and head operations by up to 3.4$\times$ due to the efficiency of its control plane.
% We use the JuiceFS benchmark to measure \sys's system overhead compared to naively using the provider's tool. We run the performance test on the object store and compare the latency for operations with and without \sys. The benchmark consists of put, get, list, head, and delete operations over 10K objects, each of size 128 KB, and measures the average latency per object. The result in Fig. \ref{fig:proxy-overhead} shows that the overhead of using \sys compared to using the cloud provider's API is minimal: for put and get operations, the overhead is less than 10\%. Furthermore, \sys can even speed up the list and head operations by up to 3.4$\times$ because of the efficiency of the control plane. 


% \subsubsection{Is learning the past indicative of the future?}
% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|c|}
%     \hline
%      TTL training   &  \# traces with same TTL \\
%      period & as full-week TTL \\
% \hline
%      1/2 day    &  16/31 \\
%      1 day    &  24/31 \\
%      3 days & 26/31 \\
%      \hline
%     \end{tabular} \\
%     \vspace{1em}
%     \caption{Comparing TTLs trained on a prefix of the trace vs.\ the best TTL for the full trace.}
%     \label{tab:ttlvs7}
%     % \vspace{-2em}
% \end{table}

% In our method, we implicitly assume that monitoring the workload and finding the best expected TTL over the past indicates the future. In other words, is the best TTL for the past also worthwhile in the future? 
% We examine the learned TTL in the two-region experiments (with a $\teven$ value of 24 hours). We compare the best expected TTL found after only a part of the trace vs.\ the eventual best TTL over the full trace.  
% The results are shown in Table~\ref{tab:ttlvs7} and indicate that once $\teven$ time has passed, the TTLs are largely similar.
% Of the 31 traces, one stands out (trace number 013). It had hardly any traffic in the first five days, and most of the traffic occurred on the last day, making training early meaningless, even after three days. All the other traces either found the absolute best TTL after three days or gave very close TTL value, resulting in no more than a 5\% additional cost during the last four days of the trace (over the weekly best TTL). 

\subsubsection{Latency Trade-Offs}




\shu{maybe need to run some ablation on latency SLOs}


\subsubsection{How does changing cost pricing affect the cost models? (R2) / operational cost overhead / how well does our policy learn the TTL}


\noindent




% \subsection{\sys Policy Ablation}
% We also dive into \sys's policy in detail, investigating how \sys performs in terms of byte hit ratio, and whether the policy indeed chooses good TTLs in different workloads. 

% \subsubsection{How does \sys's policy affect byte hit ratio?}
% \label{sec:latency}

% Aside from the cost, we study how \sys's policy affects the byte-hit ratio of each read operation, which reflects how it affects average read latency. We expect the Always Store policy to have the highest hit ratio among the baselines we evaluate, as it only incurs cold misses when an object is first accessed in a remote region. Figure~\ref{fig:32trace-9region-byte-hit} shows the byte hit ratio across 31 traces with the 9-region free placement setup: \sys achieves, on average, within 10\% of the hit ratio of the Always Store policy. This is because while \sys optimizes for cost, it also makes the best effort to retain objects in the cache as a caching policy, as the ratio between network and storage costs is often high. 
% \shu{explain sentence more}

% \subsubsection{Is learning the past indicative of the future?}
% \label{sec:future}
% In our method, we implicitly assume that monitoring the workload and finding the best expected TTL over the past indicates the future. In other words, is the best TTL for the past also worthwhile in the future? 
% We examine the learned TTL in the two-region experiments (with a $\teven$ value of 24 hours). We compare the best expected TTL found after only a part of the trace vs.\ the eventual best TTL over the full trace.  
% The results are shown in Table~\ref{tab:ttlvs7} and indicate that once $\teven$ time has passed, the TTLs are largely similar.
% Of the 31 traces, one stands out (trace number 013). It had hardly any traffic in the first five days, and most of the traffic occurred on the last day, making training early meaningless, even after three days. All the other traces either found the absolute best TTL after three days or gave very close TTL value, resulting in no more than a 5\% additional cost during the last four days of the trace (over the weekly best TTL). 


% An interesting question for future study would be how this changes over longer periods, requiring collecting information over a longer time frame.




% \subsection{System ablation}
%\subsubsection{Changes of Histograms}
%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{figures/costhist029.png}

%    \vspace{-1em} % Adjust this value as needed
%    \caption{The expected cost as a function of TTL for an example trace (no 29) with an hourly histogram. \shu{should move this to the system ablation studies in eval}}
%    \label{fig:costhist}
%\end{figure}

% \begin{figure*}[tbp]

%     \centering
%     \includegraphics[width=\textwidth]{figures/output_relative_to_skystore.pdf}
%     \label{fig:32trace-2region}
%     \vspace{-2em}
%     \caption{32 Trace, 2 Region Experiments (Relative To SkyStore) \shu{Put a line, but put what is higher cost above, and lower cost below (to make it easier to visualize)}}
% \end{figure*}

% We use the JuiceFS benchmark to measure \sys's system overhead compared to naively using the provider's tool. We run the performance test on the object store and compare the latency for operations with and without \sys. The benchmark consists of put, get, list, head, and delete operations over 10K objects, each of size 128 KB, and measures the average latency per object. The result in Fig. \ref{fig:proxy-overhead} shows that the overhead of using \sys compared to using cloud provider's API is minimal: for put and get operations, the overhead is less than 10\%. Furthermore, \sys can even speed up the list and head operations by up to 3.4$\times$ because of the efficiency of the control plane. 

% \begin{figure}
%     % \centering
%     \includegraphics[width=.85\linewidth]{figures/juicefs.pdf}
%     \caption{\sys System Performance v.s. AWS APIs: client, server and object store on region \textit{aws:us-east-2}}.
%     \label{fig:proxy-overhead}
%     \vspace{-2em}
% \end{figure}


% OLD: TWO REGION BASE AND CACHE SETTING 
% We first explore how \sys policy behaves under a 2-region base and cache setting and show that our technique has merit as a standalone caching policy. In this setup, all PUTs are located in the base region, and all GETs occur in a separate cache region. We only evaluate storage and network costs from the cache regions and ignore the storage cost of the base region, as it is constant across all policies. The evaluation is run with an average $\teven$ of 24 hours for our 7-day trace, calculated using the average network transfer cost of 22 AWS regions and storage cost close to standard storage prices in the cloud. 


% Figure~\ref{fig:2sites} shows the cost efficiency of \sys policy compared to the other baselines evaluated across 31 traces. The cost-saving percentages show how much \sys policy can save compared to each alternative, with negative values indicating cases where other methods are more cost-effective. Generally, \sys adapts well to varying workloads (e.g., on average, 10.1\%-57.6\% cost savings), closely matching or surpassing the most cost-efficient baseline method for each trace. 

% While \sys performs robustly on all workloads, alternative policies may work well on specific traces but perform poorly on other request patterns. For example, the Always Evict policy works well on traces with few repeated reads or high one-hit-wonder ratios (e.g., 40-65\% one-hit objects for Trace 014 and 051, >90\% on Trace 069 and 070). In these cases, Always Evict is 1.3\%-8.9\% better than \sys because \sys reactively caches data on the read location and takes about a day to collect metadata and adapt to workloads with many one-hit-wonders. In contrast, for traces with heavy repeated reads (e.g., Trace 065), the Always Evict policy will evict and re-fetch data across regions repeatedly, resulting in 71$\times$ higher cost compared to \sys. On the other hand, the 
% Always Store policy shows the opposite results compared to Always Evict; it performs best on heavy repeated read workloads (e.g., -3.3\% on Trace 065) and worst on one-hit-wonder workloads (e.g., 4.3$\times$ more expensive on Trace 069). 

% A Fixed TTL method like TTL=1hr slightly outperforms \sys on some workloads where repeated reads are close together within the 1-hour timeframe. For example, it is 7-10\% more cost-efficient than \sys on Traces 009, 011, 018, 020, and 036. However, it incurs very high costs on traces with longer duration repeated reads, such as Trace 047 for which it is 3.6$\times$ more expensive than our solution. For the cases where TTL=1hr does perform better, we verify that \sys indeed learns a 1-hour TTL. However, it does so only after a warm-up phase; thus, the \% cost increase comes from the overhead of its warm-up period. Compared to the other fixed TTL methods like TTL=12hr, \sys ranges from 1\% more expensive on Trace 072 and up to 31.7\% cheaper on Trace 070. Compared to TTL=$\teven$, where $\teven$ is 24 hours in this setup, \sys achieves -3.38\% (Trace 065) to 47.4\% cost savings (Trace 070).  \sys achieves -13\% (Trace 055) to 78\% (Trace 072) saving (17.41\% on average) compared to TTL-CC. TTL-CC sometimes performs poorly because it models the GET times as a Poisson distribution and this does not occur in many real traces. Lastly, compared to EWMA, \sys achieves -10.16\% (Trace 011) to 78.3\% (Trace 065) savings, averaging 25.8\%. EWMA collects statistics on a per-object basis and predicts the next access time per object. This approach can sometimes work well, but oftentimes is misleading and does not reflect the overall workload pattern. Table\ref{table:avg_std} shows the average and standard deviation of the ratio between other policies and \sys approach. Overall, TTL=12hr performs the best and the Always Evict policy performs the worst.

% Figure~\ref{fig:opt} shows that \sys, on average, performs within 15\% of the CGP policy, which is the cost-optimal in this setup. However, in specific cases, such as Trace 043 and Trace 056, \sys underperforms the optimal by 30-32\%. This discrepancy arises because \sys aggregates access statistics for all objects in the bucket, whereas CGP has an oracle knowledge at a more granular per-object level. For instance, the times between GETs in Trace 043 and 056 vary significantly across objects — 42.8\%, 31.3\%, 19.7\%, and 5.5\% of objects have GET recency of more than three days, between one and three days, one hour to one day, and less than an hour, respectively. Conversely, in traces like 069 and 070, where nearly all objects have similar access recency (i.e., >99\% objects are accessed within an hour), \sys cost performance is only 1-2\% lower than the optimal. 
% OLD: TWO REGION BASE AND CACHE SETTING 



% \subsection{7-Region across Clouds (Fixed Base)} 
% Our evaluation extends to a multi-region and multi-cloud setting with a fixed base mode. We direct all PUT operations to one specific base region and GETs across 6 additional regions, evenly split between AWS, Azure, and GCP (Section~\ref{sec:eval-workload}). The derived $\teven$ values range from 4 hours to 2.2 days, calculated using the smallest value within each cloud and the largest value across clouds. Figure~\ref{fig:32trace-7region} and Table \ref{table:avg_std} demonstrate that \sys consistently performs well across traces, achieving an average of 11.2\% to 69.5\% cost savings over other baselines.

% Interestingly, policy effectiveness differs with the increased number of regions. Originally, the Always Evict policy is 2.67$\times$ worse than Always Store in 2 regions, but it outperforms the other by 1.8$\times$ in 7 regions. This is because read operations are now spread over more regions, so it is less likely repeated reads on the same object will occur in the same region.
% % due to the spread of read operations per objects into more regions. 
% Take Trace 013 as an example where 99\% of objects have 2-10 GETs; when these GETs are spread across the 7 regions, most regions see only a few GETs, which makes Always Evict more beneficial due to its minimal storage cost. On the other hand, the Always Store policy still performs reasonably well for traces like 036, which has heavy reads. Second, we see lower cost savings from Table~\ref{table:avg_std} on average when comparing 2-region results with 7-region ones, except TTL-CC, which performs particularly poorly in in the multi-cloud setting. This is expected because GETs are dispersed across regions, so the base network cost for fetching objects initially becomes higher. %, thus offsetting the differentiation between baselines.  

% % Second, \sys average cost saving numbers from Table~\ref{table:avg_std} are generally lower in 7-region compared to the 2-region setting in Section~\ref{sec:twosite}. This is also expected as the GETs get distributed across regions and repeated accesses at the cache regions becomes smaller, the base cost for fetching objects initially becomes higher, thus offset the differentiation between baselines. Also, the cost heterogeneity becomes larger in multi-cloud, which can exacerbate this issue. 

% % Trace 13 can be taken as an example, where 99\% of the objects have 2-10 GETs. 
% % For example, 99\% of objects in Trace 013 contain between 2-10 reads. When we create our 7 region traces, these reads are distributed across regions, making few GETs in each region. Thus, on average, the Always Evict policy performs better than Always Store, as it is not worth storing data with only a few accesses at the cache regions. 

% Lastly, the Trace 014 result shown in Figure~\ref{fig:32trace-7region} is an outlier case where \sys performs 25\% worse than a policy like Always Evict or TTL=1hr. This trace comes with many one-hit-wonder accesses, and 90\% of GETs appear in the first 36 hours. While we verify that \sys does identify the best TTL (which is close to the Always Evict policy, the best policy in this setting), \sys does so only after a large percentage of GETs had already occurred. Hence, it fails to keep costs low for this period of time. After a long enough warm-up phase, our results are better. The same reasoning applies to why \sys fails in 085 and 095 traces. We see similar behaviors when generalizing the fixed base mode to 9-region, shown in Appendix C. 

% Lastly, one outlier of \sys appears in Trace 014, where - in this trace, 90\% of the GETs occur in the first 36 hours. While \sys does identify the best TTL here, which is Always Evict, since there are hardly any repeated reads). However, it does so only after a large percent of the GETS had already occurred. Hence, it fails to keep up. After enough of a warm-up phase, our results become even better. Same reasonings apply for Trace 013 and Trace 095. Table~\ref{table:avg_std} lists the average saving of our method in this setting. The savings compared to TTL=12hr are over 11\%, then TTL=1hr, and then $\teven$. In this complex setting, TTL-CC did not fare well. We run the fixed base mode for 9-region traces as well and draw similar conclusions, as in Appendix\ref{}.


% Also, 
% This is because the cost for the initial get of an object is the same for all methods, and only subsequent gets make the difference. In the 7-region traces, there are many more initial gets and far fewer subsequent ones, leaving less potential for differentiation between methods. Also, higher network costs exacerbate this issue for multi-clouds. 

% The cost savings \sys achieves change from 57.6\% from the 2-region base and cache setup to 67.5\% because the network cost of the Always Evict policy is even more expensive, considering data now can be located in another cloud. \shu{Write about example of 047, reads are spreaded and always store always evict behavior; write about 013 (have few GETs, and when it becomes multi-region --> all the reads, 99\% between 2-10 reads), 036 (over 1) the majority of objects have between 10-100 reads, does not get affected}

% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=\textwidth]{figures/byte_hit_ratio_9_region_no_base.pdf}
%     \vspace{-2em}
%     \caption{\textbf{\sys Byte Hit Ratio (\%) on 9-Region, Free Placement (FP):} \sys policy on average within 10\% of the byte hit ratio of the  Always Store policy.}
%     \label{fig:32trace-9region-byte-hit}
% \end{figure*}



% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=\textwidth]{figures/savings_7_region_base_without_storage.pdf}
%     \vspace{-2em}
%     \caption{\textbf{\sys Cost Savings (\%) on 7-Region, Fixed Base (FB)}: \sys achieves on average 11.2\% - 69.5\% cost savings over 30 traces and 6 other baselines.}
%     \label{fig:32trace-7region}
% \end{figure*}



% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=\textwidth]{figures/savings_9_region_no_base.pdf}
    
%     % \vspace{-2em}
%     \caption{\textbf{\sys Cost Savings (\%) on 9-Region, Free Placement (FP)}: \sys achieves on average 2.0\%-59.4\% cost savings over over 30 traces and 6 other baselines.}
%     \label{fig:32trace-9region}
% \end{figure*}

% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Policy} & \multicolumn{2}{c}{\textbf{2-Region (FB)}} & \multicolumn{2}{c}{\textbf{7-Region (FB)}} & \multicolumn{2}{c}{\textbf{9-Region (FP)}} \\
% \cmidrule{2-7}
% & \textbf{Avg} & \textbf{Std Dev} & \textbf{Avg} & \textbf{Std Dev} & \textbf{Avg} & \textbf{Std Dev} \\
% \midrule
% \textit{Always Evict} & 7.85 & 16.19 & 3.28 & 5.55 & 2.46 & 3.89 \\
% \textit{Always Store} & 2.94 & 1.28 & 6.09 & 8.89 & 1.49 & 0.28 \\
% \textit{TTL-CC} & 1.34 & 0.67 & 2.37 & 4.22 & 1.64 & 2.04 \\
% \textit{TTL=12hr} & 1.22 & 0.15 & 1.13 & 0.15 & 1.02 & 0.05 \\
% \textit{TTL=1hr} & 1.25 & 0.60 & 1.16 & 0.52 & 1.08 & 0.30 \\
% \textit{Teven} & 1.46 & 0.30 & 1.42 & 0.33 & 1.08 & 0.12 \\
% \textit{EWMA} & 1.49 & 0.66 & N/A & N/A & N/A & N/A \\
% \textit{SPANStore} & N/A & N/A & N/A & N/A & 1.35 & 0.24 \\
% \bottomrule \\
% \end{tabular}%
% \caption{Average and standard deviation of existing baselines, measured as the average ratio between baseline v.s. \sys total cost across traces. FB denotes the free base mode, and FP denotes the free placement mode.}
% \vspace{-2em}
% \label{table:avg_std}
% \end{table}



